Delegating to Multiple Agents

We consider a multi-agent delegation mechanism without money. In our model, given a set of agents, each agent has a fixed number of solutions which is exogenous to the mechanism, and privately sends a signal, e.g., a subset of solutions, to the principal. Then, the principal selects a final solution based on the agents' signals. In stark contrast to single-agent setting by Kleinberg and Kleinberg (EC'18) with an approximate Bayesian mechanism, we show that there exists efficient approximate prior-independent mechanisms with both information and performance gain, thanks to the competitive tension between the agents. Interestingly, however, the amount of such a compelling power significantly varies with respect to the information available to the agents, and the degree of correlation between the principal's and the agent's utility. Technically, we conduct a comprehensive study on the multi-agent delegation problem and derive several results on the approximation factors of Bayesian/prior-independent mechanisms in complete/incomplete information settings. As a special case of independent interest, we obtain comparative statics regarding the number of agents which implies the dominance of the multi-agent setting ($n \ge 2$) over the single-agent setting ($n=1$) in terms of the principal's utility. We further extend our problem by considering an examination cost of the mechanism and derive some analogous results in the complete information setting.

==> Delegating to Multiple Agents (1)/abstract.tex <==
We consider a \emph{multi-agent delegation} mechanism without money.
% which is the first to study the multi-agent extension of Kleinberg and Kleinberg (EC'18).
In our model, given a set of agents, each agent has a fixed number of solutions which is exogenous to the mechanism, and privately sends a signal, \eg a subset of solutions, to the principal.
Then, the principal selects a final solution based on the agents' signals.
% Our model captures a variety of real-world scenarios, spanning classical economical applications to modern intelligent system.
In stark contrast to single-agent setting by Kleinberg and Kleinberg (EC'18) with an approximate \emph{Bayesian mechanism}, we show that there exists efficient approximate \emph{prior-independent mechanisms} with both information and performance gain, thanks to the competitive tension between the agents.
Interestingly, however, the amount of such a compelling power significantly varies with respect to the information available to the agents, and the degree of correlation between the principal's and the agent's utility.
Technically, we conduct a comprehensive study on the multi-agent delegation problem and derive several results on the approximation factors of Bayesian/prior-independent mechanisms in complete/incomplete information settings.
As a special case of independent interest, we obtain comparative statics regarding the number of agents which implies the dominance of the multi-agent setting ($n \ge 2$) over the single-agent setting ($n=1$) in terms of the principal's utility.
We further extend our problem by considering an examination cost of the mechanism and derive some analogous results in the complete information setting.
% To highlight several technical results,
% \begin{enumerate}
%     \item In the complete information setting, we show that there exists a prior-independent mechanism such that the principal's expected utility is bounded below by the \emph{first-best solution} of the \emph{second-best agent} (in principal's view). We quantify this approximation factor by analyzing its upper and lower bound under various regimes, which further enables us to construct an asymptotically optimal prior-independent mechanism with respect to $n$ and $k$ (number of solution per agent) under certain regimes. In words, the power of multi-agent delegation is significant. At the heart of this analysis, we provide new technical results regarding the order statistics of i.i.d. random variables, which might be of independent interest.
%     \item In the incomplete information setting, we show that under symmetric agents with uniform distribution $U[0,1]$ and independent utility assumption, there exists a prior-independent mechanism for which there is a $(1-e^{-n^2/2(n-1)^2})$-approximate \emph{Bayes Nash equilibrium} such that the principal's expected utility becomes optimal, where $1-e^{-n^2/2(n-1)^2}$ converges to $1-\nicefrac{1}{\sqrt{e}} \cong 0.3935$ as the number of agents $n$ increases. 
%     Using a similar technique, we analyze that there exists a \emph{Bayes correlated equilibrium} with a multiplicative approximation factor of $e^{n^2/2(n-1)^2} \cong \sqrt{e}$.
%     \item We further show that the assumptions of symmetric agents and independent utility in (2) are necessary.
%     That is, without these assumptions, we can construct a problem instance such that there exists a \emph{Bayes Nash equilibrium} in which the agents propose the worst solution in terms of the principal's utility, which possibly leads to arbitrarily bad principal's expected utility.
%     Thus, the gains from delegating to multiple agents becomes drastically restrictive.
% \end{enumerate}

==> Delegating to Multiple Agents (1)/bayes_correlated.tex <==

\section{Bayes Correlated equilibrium}\label{sec:correlated_equi}
In this section, we discuss that the mechanism presented in Theorem~\ref{thm:bayes_oblivious} also has an efficient Bayes correlated equilibrium.
To be more specific, we are interested in the notion of Bayes correlated equilibrium \cite{bergemann2016bayes}.
Suppose that there exists a mediator who is able to access the realization of all the solutions observed by the agents.
Given the realization of all the solutions $\omb = (\omb_i)_{i \in [n]}$ observed by the agents, the mediator recommends a strategy $\psi_i: \Om^* \mapsto \Sigma_i$ for each agent $i \in [n]$.
It is important to note that the mediator recommends the strategy based on observing all the agents' solutions.
Given the recommended strategy $\psi_i$ and observed solution $\omb_i$, agent $i$ plays a strategy $\sigma_i(\omb_i, \psi_i): \Omega^* \times \Sigma_i \mapsto \Omega_i$.
The procedure of recommending strategies is specified as a part of the mechanism $M$, and we denote by $f_{M, \sigma, \psi}(\omb)$ the interim allocation function, \ie the selected winner, of the mechanism $M$ given $\psi(\omb)$ and $\sigma(\omb, \psi).$

Then, given $\psi_i(\omb)$ and $\omb_i$, agent $i$'s expected utility of playing $\sigma_i$ is
\begin{align*}
	u_i(\sigma_i(\psi_i, \omb_i), \sigma_{-i})
	=
	\Ex{\int_{\omb_{-i}} y_i(f_{M,(\sigma_i(\psi_i(\omb), \omb_i), \sigma_{-i})})f_{-i}(\omb_{-i})d\omb_{-i}},
\end{align*}
and agent $i$'s total expected utility of playing $\sigma_i$ is 
\begin{align*}
	u_i (\sigma_i, \sigma_{-i}) = \Exu{\omb_i}{u_i(\sigma_i(\psi_i, \omb_i), \sigma_{-i})}.
\end{align*}
We now define a Bayes correlated equilibrium as follows.
\begin{definition}[Bayes correlated equilibrium]
	We say that $\psi_i$ induces a \emph{Bayes correlated equilibrium} (BCE) if for any $i \in [n]$,
	\begin{align*}
		u_i(\psi_i, \sigma_{-i}) \ge u_i(\sigma'_i, \sigma_{-i}),	
	\end{align*}
	for any other strategy $\sigma'_i$, \ie there exists no incentive to deviate from the mediator's recommendation.
\end{definition}
Compared to BNE, due to the existence of the additional signals provided by the mediator who can observe all the solutions, both the principal and agents may enjoy the increased utility.
%We note that our definition of BCE is slightly different from that of \citet{bergemann2016bayes}, as we allow the mediator to recommends null strategy and there exists no restriction in playing strategies in this case.
In the following theorem, we prove that there exists a PIM such that it achieves asymptotically constant multiplicative approximation factor for some BCEs.
We provide the proof in Appendix~\ref{pf_thm:bce}
\begin{theorem}\label{thm:bce}
	Consider a symmetric and independent setting such that the distributions of the both principal's and agent's utility follow $U[0,1]$.
	Then, there exists an $\parans{\exp\parans{\frac{n^2}{2(n-1)^2}},0}$-approximate PIM and corresponding BCE.
\end{theorem}

==> Delegating to Multiple Agents (1)/bck/bayes_recover.tex <==
% \begin{proof}
% 	The overall proof is exactly same as that of Theorem \ref{thm:recover}.
% 	In the proof of Theorem \ref{thm:recover}, we only used Assumption~\ref{as:pareto},
% 	and the fact that principal selects the best proposed solution as the winner.
% 	As both of those asuumptions still hold in incomplete information settings, we can follow the same proof to get the same result.
% 	However, we provide the proof for completeness. \keivan{should we really put the proof here? it is exactly same.}

	% Consider a problem instance of multi-agent settings where $n$ agents propose solutions.
	% In order to find solutions, Agent $i$ samples $k_i$ times from distribution $D_i$.
	% We construct a single-agent problem instance
	% where the only agent samples $k_i$ times from each distribution $D_i$, $\sum_{i=1}^{n} k_i$ samples on aggregate.
	% According to \citet{kleinberg2018delegated}, there exists an SPM with proper eligible set $R$ under the constructed settings such that
	% principal's expected utility is at least $\frac{1}{2}\Ex{X_{(1)}}$.
	% We use the same eligible $R$ in designed SPM for all agents in multi-agent settings.
	% We claim that for any realization of solutions $\omb = \cup_{i=1}^{n} \omb_i$,
	% principal's utility in multi-agent setting is at least that of single-agent setting which further implies that
	% using same eligible set $R$, principal's expected utiltiy in multi-agent settings is at least $\frac{1}{2}\Ex{X_{(1)}}$.
	% \keivan{Should I elaborate on single-agent utility function?}

	% Consider a realization of solutions $\omb$. Let $\omega$ be the winner in single-agent setting.
	% If $\omega = \perp$, then all observed solutions are not eligible.
	% Formally, for all $i$ in $\left[n\right]$, and $j$ in $\left[k_{i}\right]$:
	% $\omega_{i, j} \notin R$. In this case, there is not any eligible solution in multi-agent setting as well which
	% indicates that prinicpal utiltiy in both settings is zero.
	% On the other hand, if $\omega \neq \perp$, let $\omega^*$ be the winner in multi-agent setting, we claim that $x(\omega^*) \geq x(\omega)$.
	% Denote by $i$ the agent who has sampled $\omega$. Denote by $\sigma_i$ the solution proposed by agent $i$ in multi-agent setting.
	% As both $\sigma_i, \omega \in R$, and $\omega$ is the eligible solution which maximizes agent utility in single-agent setting then 
	% $y_i(\omega) \geq y_i(\sigma_i)$. As a result, according to Assumption~\ref{as:pareto}, $x(\sigma_i) \geq x(\omega)$.
	% There are two cases

	% \begin{itemize}
	% 	\item
	% 	$\omega^*$ is sampled by $i$, i.e. $\omega^* = \sigma_i$. As shown above $x(\omega^*) = x(\sigma_i) \geq x(\omega)$.
	% 	\item
	% 	$\omega^*$ is sampled by another agent $j \neq i$.
	% 	As principal selects the best proposed solutions among all agents, $x(\omega^*) \geq x(\sigma_i)$.
	% 	Using the inequality $x(\sigma_i) \geq x(\omega)$ we further conclude that $x(\omega^*) \geq x(\omega)$.
	% \end{itemize}

	% This finishes the proof.

	% OLD PROOF
	% As in the proof of Theorem \ref{thm:recover}, we focus on proving (1) and we will argue that the proof naturally transfers to the other settings as well.
	% Consider a problem instance of the multi-agent setting.
	% Restrict our attention to agent $i$, and consider a problem instance of the single-agent setting such that the principal delegates to only agent $i$.
	% Then, by \citet{kleinberg2018delegated}, there exists an SPM under the constructed single-agent setting such that the principal's expected utility is at least $\frac{1}{2}\Ex{X_{i,(1)}}$.
	% Denote this mechanism by $M'_i$ and let its eligible set be $R_i$.
	% We can define such $R_i$ for each agent $i \in [n]$.
	% Given the observed solution $\omb_i$ of agent $i$, let the agent's strategy be $\sigma'_i \in \Omega^{k_i}$ under the single-agent setting with $M'$.
	
	% Now, under the multi-agent setting, consider an MSPM with eligible sets $R_i$ and a deterministic tie-breaking rule with transitivity.
	% Suppose that the solutions are realized to be $\omb = (\omb_1, \ldots, \omb_n)$ and consider any corresponding equilibrium strategies $\sigma = (\sigma_1,\ldots, \sigma_n)$.
	% We want to show that each agent $i$, given the observed solutions $\omb_i$, play a strategy $\sigma_i$ such that $x(\sigma_i) \ge x(\sigma'_i)$.
	% Suppose not, i.e. $x(\sigma_i)<x(\sigma'_i)$ for some $i \in [n]$.
	% If agent $i$ does not have eligible solutions, it contradicts the fact that $x(\sigma_i) < x(\sigma'_i)$.
	% Hence, agent $i$ has at least one eligible solution $\sigma'_i$.
	% Obviously, $\sigma \in R_i$ since if not the agent's utility in playing $\sigma_i$ is simply zero, and then proposing $\sigma'_i$ would yield a larger utility.
	% Then, by the definition of $\sigma'_i$, $y(\sigma'_i) \ge y(\sigma_i)$ and $x(\sigma'_i) > x(\sigma_i)$.
	% This contradicts Assumption~\ref{as:pareto} since $\sigma'_i$ dominates $\sigma_i$.
	% Therefore we conclude that $x(\sigma_i) \ge x(\sigma'_i)$.
	% Since the principal eventually selects the best candidate that maximizes her utility, we have
	% \begin{align*}
	% 	\Ex{\Ex{\max_{i \in [n]} x(\sigma_i) \given \omb_i}}
	% 	\ge
	% 	\Ex{\Ex{\max_{i \in [n]}x(\sigma'_i) \given \omb_i}}
	% 	\ge
	% 	\frac{1}{2}\Ex{X_{\max}}.
	% \end{align*}
	% Similarly, we can derive the same arguments for (2) and (3), and we finish the proof.
% \end{proof}

% In proving Theorem \ref{thm:recover_bayes}, we only analyze the principal's expected utility given a BNE, but we do not characterize the BNEs at all.
% This is in stark contrast to the complete information setting, since in Theorem~\ref{theorem:multi-agent-unlimited-budget}, we reveal that proposing the solution that maximizes the principal's utility is an equilibrium strategy except for the agent with the best solution, even under the MSPM without any eligible sets.

==> Delegating to Multiple Agents (1)/bck/cost_quantify.tex <==

\subsection{Informed mechanism}
\todo{single agent recovery is still possible? - not quite sure for now}

\todo{General lower bound? - when super agent, then regardless of $B$, examining super agent first then prophet lower bound.}


In case of symmetric agents, we observe that Theorem~\ref{thm:informed} still holds even with unit budget.
\begin{corollary}
	Consider symmetric agents endowed with distribution $D$ with support on $[0,1]$ such that its c.d.f. $F(x)$ satisfies $F(x) \le x^{\alpha}$ for any $x \in [0,1]$ for some $\alpha >0$. Then, there exists an oblivious mechanism with arbitrary examination budget such that under any BNE, the delegation gap is at most $1 - \parans{\frac{\alpha nk}{\alpha nk+1}}^{\frac{1}{\alpha nk}}$, which converges to $0$.
\end{corollary}
Noting that the proof of Theorem \ref{thm:informed} can be easily applied to examination cost setting with arbitrary budget, we omit the proof.

\subsection{Oblivious mechanism}
We present several explicit upper bound on the delegation gap for oblivious mechanism.
Our results will be based on the following corollary which is straightforward to obtain from Theorem \ref{theorem:multi-agent-limited-budget}.
\begin{corollary}
If the principal does not define an eligible set, then in the multi-agent setting with budget $2 \leq B \leq n - 1$, the RSPM has a delegation gap of at most
\begin{align*}
\Ex{X_{(1)}} - \Ex{X_{(n-B+2)}}.
\end{align*}
\end{corollary}

\todo{negative results on general setting}

We now consider symmetric agents.
First, in case of arbitrary distribution supported on $[0,1]$, we present the following theorem.
\begin{theorem}
	If agents are symmetric and the domain of their utility function lies in $[0,1]$, then there exists an oblivious mechanism in which the delegation gap is upper bounded by  \todo{Simplify... A figure on this w.r.t. $B$ for several $n$ may help?}.
\end{theorem}
\begin{proof}
	Suppose that we run the RSPM.
	By our assumption on symmetry and since each agent independently samples solutions, $X_{i,(1)}$ for $i \in [n]$ are identical and independent.
	Then, we use the following lemma introduced by \citet{lopez2011upper}.
	\begin{lemma}[\citet{lopez2011upper}]\label{lm:lopez_2}
		Let $X_1,\ldots, X_n$ be i.i.d. random variables supported on $[0,1]$. Given an integer $k$ such that $1 \le l < k \le n-1$, let $Y_k$ and $Y_l$ be $k$-th and $l$-th order statistics of $X_1,\ldots, X_n$. 
		Define
		\begin{align*}
			p_{k,l}= \parans{1 + \parans{\frac{\binom{n-1}{l-1}}{\binom{n-1}{k-1}}}^{\frac{1}{l-k}}}^{-1}.
		\end{align*}
		Then, the following holds.
		\begin{align*}
			\Ex{Y_{l} - Y_{k}} \le np_{k,l}^{k-1}(1-p_{k,l})^{n-l}\parans{\binom{n-1}{k-1}(1-p_{k,l})^{l-k} - \binom{n-1}{l-1}p^{l-k}}
		\end{align*}
	\end{lemma}
	Plugging $l = n$ and $k=B-1$ in the above lemma, we obtain
	\begin{align*}
		\Ex{X_{(1)} - X_{(n-B+2)}}
		\le 	
		\parans{1 + \parans{\frac{1}{\binom{n-1}{B-2}}}^{\frac{1}{n-B+1}}}^{-1},
	\end{align*}
	and it completes the proof.
\end{proof}

\begin{theorem}
	If agents are symmetric and $X_{i,j} \sim D$ such that $D$ has MHR, then there exists an oblivious mechanism in which the delegation gap is upper bounded by $\sqrt{2Var(D_{\max})}$ where $D_{\max}$ is distribution of $X_{i,(1)}$.
	In case of $D = U[0,1]$, we have delegation gap of at most $(n-B+1)\sqrt{2 \cdot \frac{k}{(k+1)^2(k+2)}} \approx \frac{\sqrt{2}(n-B+1)}{k}$.
\end{theorem}
\begin{proof}
	\todo{Elaborate more on}
	Note that
	\begin{align}
		\Ex{X_{(1)} - X_{(n-B+2)}}
		&=
		\Ex{X_{(1)} - X_{(2)}} + \Ex{X_{(2)} - X_{(3)}} + \ldots + \Ex{X_{(n-B+1)} - X_{(n-B+2)}}.\label{ineq:010151137}
	\end{align}
	We now prove that for any $k = 2,\ldots, n-1$,
	\begin{align*}
		\Ex{X_{(k)} - X_{(k+1)}}
		\le 
		\Ex{|A-B|},
	\end{align*}
	where $A$ and $B$ are two i.i.d. random variables of which the endowed distribution is equivalent to that of $X_{i,(1)}$.
	This is indeed true because
	\begin{align*}
		\Ex{X_{n-k+1:n} - X_{n-k:n}}
		&\le
		\Ex{X_{2:n-k+1} - X_{1:n-k+1}}
		\\
		&\le
		\Ex{X_{2:2} - X_{1:2}}
		\\
		&=
		\Ex{|A-B|},
	\end{align*}
	where the first inequality follows from the first part of Lemma~\ref{lm:order_stat_diff}, and the second one follows from the second part.
	Hence, applying Theorem~\ref{thm:mhr_upperbound} in \eqref{ineq:010151137}, we finish the proof.
\end{proof}




\begin{theorem}
	If agents are symmetric and $X_{i,j} \sim D$ such that $D$ has monotone increasing p.d.f. then there exists an oblivious mechanism in which the delegation gap is upper bounded by $\frac{n-B+1}{n+1}\sqrt{2Var(D_{\max})}  +$ where $D_{\max}$ is distribution of $X_{i,(1)}$.
	In case of $D = U[0,1]$, we have delegation gap of at most $\frac{n-B+1}{n+1}\sqrt{2 \cdot \frac{k}{(k+1)^2(k+2)}} \approx \frac{3\sqrt{2}(n-B+1)}{k(n+1)}$.
\end{theorem}
\begin{proof}
	\todo{Similar to the proof above}
\end{proof}




% \subsection{Toward better mechanism}
% Now we study whether there exists a mechanism that outperforms the randomized single-proposal mechanism in the multi-agent case.

% \paragraph{Warm-up: randomized $k$-proposal mechanism}
% We start with a $k$-proposal mechanism, in which the agents can submit up to $k$ candidates, with a simple selection rule: randomly sort the candidates, examine the first $B$ candidates, and then commit to the best candidate.
% This mechanism obviously has an examination cost of $B$.

% Intuitively, this mechanism works very poor as observed by the following conjecture.
% \begin{conjecture}

%In randomized $k$-proposal mechanism with unit budget, the delegation gap can monotonely increase with respect to $k$, and thus is lower bounded by the delegation gap of single-proposal mechanism.

% \keivan{In this case, agent $i$ will propose top $k$ eligible points w.r.t to her own utility $y_i$. Therefore, change in delegation gap depends on whether those top $k$ points give better utility to the principal or not.}

% \suho{Provide a counterexample that this works poorly}
% In a unit-budget randomized $k$-proposal mechanism with arbitrary eligible sets, the delegation gap is monotone increasing with respect to $k$, and thus is lower bounded by the delegation gap of RSPM with the same eligible sets.
% \end{conjecture}
%\begin{proof}[Intuition]
%	The intuition behind this conjecture is that given fixed budget $B$, when $k$ increases then the chance that set of $B$ chosen solutions by principal covers some solutions of a same agent increases. It implies that the agent may rely on the fact that in some cases competition is only over his proposed solutions which motivates him to propose solutions to maximize his own utility instead of principal utility.
%\end{proof}

% \begin{conjecture}
% In a $B$-budget randomized $k$-proposal mechanism with arbitrary eligible sets, the delegation gap can monotony increase with respect to $k$, and thus is lower bounded by the delegation gap of RSPM with the same eligible sets.
% \end{conjecture}

% \keivan{The intuition behind this conjecture is that given fixed budget $B$, when $k$ increases then the chance that set of $B$ chosen solutions by principal covers some solutions of a same agent increases. It implies that the agent may rely on the fact that in some cases competition is only over his proposed solutions which motivates him to propose solutions to maximize his own utility instead of principal utility.}
%\paragraph{Improved mechanism}
%We have some options that we do not fully exploit in our randomized single-proposal mechanism.
%Firstly, we did not customize eligible set for each agent. Secondly, we did not optimize the examination order over the agents.




% \section{Further directions}


% \begin{question}[Improved mechanism - customizing eligible set]
% In our RSPM, the examination set is randomly permuted and then we examine up to $B$ candidates, and we mainly consider a homogeneous eligible set.
% How much can we improve by considering heterogeneous eligible sets for the agents?
% Consider an extreme scenario in which each agent $i$ has a distribution with support on $\{1, 2^i\}$ with probability $1/2$ for both the elements, in terms of the principal's utility, and suppose that both elements have a random utility of $1$ or $2$ for the agent independently from the principal's utility.
% In this case, if we set agent-wise threshold $\tau_i = 2^i$, this seems to work superior to any homogeneous eligible set, though needs to be checked thoroughly.
% As this kind of exploiting agent-wise thresholds seems to be somewhat similar to multiple threshold algorithms in prophet inequality literature, it would be interesting if we can find some relations between general RSPM and multiple thresholds algorithms in the prophet inequalities literature.
% Furthermore, as the principal is allowed to select up to some given multiple candidates, it would be also interesting if we may find some relations between some mechanisms and the multi-unit prophet inequality, though it is not clear at this point.
% \end{question}

% \begin{question}[Improved mechanism - examination order]
% Obviously, the randomized examination is somewhat silly, since if we know that some agents have superior distribution, the principal might be better to examine them first.
% This problem reduces to designing an optimal order of examination for our mechanisms.
% Consider the example we considered in Question 4. 
% In this case, we can further optimize the examination order by examining the agents with large indexes first, as they are always expected to have larger values when the thresholds are set properly.
% Suppose that there exists no eligible set and $k_i = 1$. 
% Under the RSPM each agent essentially proposes only one solution.
% In which order should we examine the candidates in this case?
% More generally, the question of deciding examination order may (or may not) be similar to the problem of deciding optimal ordering in prophet inequalities~\cite{agrawal2020optimal}.
% It would be interesting to explore whether some relations indeed exist, though not seem to be straightforward.
% \end{question}



% \begin{question}[Further possible extensions]
% Further extensions that might be interesting to explore.
% It seems we should definitely think about the incomplete information setting for sake of completeness, but the others might be beyond the scope of this research.
% \begin{enumerate}
%     \item Incomplete information setting
%     \item Multiple distributions for each agent (similarly from~\citet{kleinberg2018delegated}
%     \item binary model with sampling cost model, which corresponds to delegated search on Weitzman's box problem as in~\citet{kleinberg2018delegated}
%     \item Online proposal and examination setting (when agents sequentially propose and the principal should irrevocably decide)
%     \item Learning agents (when each agent does not know the quality of own solutions but rather learns over multiple interaction between the mechanism)
% \end{enumerate}
% \end{question}


% \begin{conjecture}
% For any budget $B$, there exists a mechanism in which the delegation gap is always smaller than randomized single-proposal mechanism.
% Some ideas: use personalized eligible set, use a smarter selection rule
% \end{conjecture}

==> Delegating to Multiple Agents (1)/bck/cost_recover.tex <==

\todo{Mention that if $B \ge n$, all the results from the no cost section holds as we consider MSPM with some eligible sets.}
\begin{corollary}
In the multi-agent setting, for any mechanism $M$ with budget $B \ge n$ and corresponding Nash equilibrium $\sigma$, there exists a RSPM $M'$ with budget $n$ such that for any Nash equilibrium strategies $\sigma'$, for any $\om \in F_{M,\sigma}(\omb)$ and any $\om' \in F_{M',\sigma'}(\omb)$, we have $x(\om) \le x(\om')$ for any observed solutions $\omb \in \Omega^*$.\todo{prove for self-containedness}
\end{corollary}

==> Delegating to Multiple Agents (1)/bck/randomized_not_working.tex <==
\section{Randomized tie-breaking rule does not work}\label{app_sec:random_tie}
\suho{I think this section will be removed}
We recall that Theorem~\ref{theorem:multi-agent-unlimited-budget} only holds for the \emph{deterministic} tie-breaking rule.
The intuition behind it is that if the principal exploits a randomized tie-breaking rule, it may reduce the power of competition in certain cases since the agents may settle with a bad solution in terms of the principal, as it still gives the agents higher utility with small probability due to the randomized tie-breaking rule, yet another solution which might induce higher probability to be selected by the principal may yield too low utility for the agents. 
However for the deterministic tie-breaking rule, as the principal naturally prefers some agents, less preferred agents tend to submit the candidate more in a competitive manner in order to be selected by the principal, and again, this recursively makes preferred agents behave more in favor of the principal.
More formally, in the following theorem, we prove that the random tie-breaking rule can be arbitrarily bad, which implies that the deterministic tie-breaking rule is essential.
\begin{theorem}
    Consider a MSPM with no eligible sets and a randomized tie-breaking rule that uniform-randomly selects the candidate.
    Then, for any $\alpha \ge 1$, there exists a problem instance such that the mechanism have a bad equilibrium in which the delegation gap can be larger than $\alpha \cdot \Ex{X_{(1)} - X_{(2)}}$.
\end{theorem}
\begin{proof}
    \todo{Fix this w.r.t. i.i.d. sampling}
	Given a solution space $\Omega = \{a,b,c\}$, consider $n=3$ agents with the same utility function $y$ such that $y(a) > 3y(b)$ and $y(b) > y(c)$.
	The principal's utility function is given by $x(\cdot)$ such that $x(a) < x(b) < x(c)$.
	Note that the detailed quantities will be determined later.
	Agent $1$ and $2$ always sample both $a$ and $b$, and agent $3$ also always samples both $a$ and $c$. 
	In this case, although $X_{(1)} - X_{(2)} = x(c) - x(b)$, if all the agents $1$, $2$ and $3$ determine to submit $a$, they can get $y(a)\cdot 1/3 > \max(y(b),y(c))$, and thus this forms an equilibrium.
	In this equilibrium, the delegation gap is $(x(c) - x(a))$, and hence by constructing the function $x(\cdot)$ to satisfy $x(c) - x(a) \ge \alpha (x(c) - x(b))$, we can conclude the proof.
	Note that this is always po ssible since we can take arbitrarily small $x(a) \le \alpha x(b) - (\alpha-1)x(c)$ as RHS is a positive number.
\end{proof}

==> Delegating to Multiple Agents (1)/bulow_klemperer.tex <==

\section{Bulow-Klemperer-style result for prior-independent mechanism}\label{sec:BKS}
In constructing efficient PIM, one standard way would be to construct PIM from BM by applying the Bulow-Klemperer-style result by \citet{bulow1994auctions}, which considers a fictitious BM with $n+1$ agents to find a good upper bound on the efficiency of PIM with $n$ agents.
More precisely, they first show the existence of PIM (auction in their case) which always allocates the item to some bidders and then prove that such PIM is optimal among the mechanism that always allocates the item.
Then, for any Bayesian mechanism $M$ with an arbitrary reserve price, one can consider a fictitious auction with $n+1$ agents such that it runs $M$ with the first $n$ agents, and if it does not allocate the item, then it allocates the item to $n+1$-th agent.
Given the observations above, one can conclude that the PIM with $n$ agents defined above outperforms arbitrary BM with $n+1$ agents, and thus we can derive the approximation factor of PIM based on BM.
This technique, however, does not work in our case as we cannot easily argue that MSPM that admits all the solutions induces the optimal utility for any mechanism that always adopts the winner.
This is because we can consider a PIM that always admits all the solutions for some agents, but enforce some nontrivial (which does not always accept any solution) eligible sets for other agents. 
Indeed, this mechanism may outperform MSPM that admits all solutions, since it may motivate the other agents with nontrivial eligible sets to propose more in favor of the principal, while maintaining the mechanism to always delegate to some agents.

==> Delegating to Multiple Agents (1)/compare.tex <==
\section{Comparing multi-agent and single-agent delegation}\label{sec:compare_mul_sin}
% In Theorem~\ref{thm:recover}, we show that one can always recover the guarantees from the single-agent delegation setting for informed mechanism by setting proper eligible sets.
% However, in terms of comparison between the multiple-agent and the single-agent setting, the argument we used in the proof of Theorem Theorem~\ref{thm:recover} does not seem to be a reasonable way to compare both settings.
To give a brief intuition in how one can reasonably compares the multi-agent and single-agent setting in terms of the principal, we start with an example.
\begin{example}\label{ex:cs}
    Consider a task requester in the online labor market, \eg crowdsourcing platform.
    The task requester wants to solve a task by finding a single best solution for the task, and she is capable of recruiting five online workers.
    Due to the intrinsic volatility of the online platform, each worker is equipped with a similar level of skill, and is expected to exert a similar level of effort per some unit of payment.
    As such, each worker has the same \emph{certainty equivalent} in coming up with a single solution, saying $\$10$.
    Because of the anonymity of the online labor market, each worker does not exactly obey the instruction of the task therein to answer the task, but instead propose a solution of his own interest, \ie misaligned payoffs.
    The task requester has a budget of $\$100$, and faces two options of (i) delegating to a single agent and (ii) delegating to five agents.
    The first option is to solely depend on a single worker, and the worker will sample $10$ solutions and commit to one of them.
    By exploiting the second option, five workers will observe two solutions each and commit to one of them.
    Given the assumptions above, it is likely that the expected quality of a single solution will be similar, i.e. workers are symmetric.
    Which option should the principal take?
    As observed in our previous results, delegating to multiple workers is expected to be generally better, but to any extent?
% That is, delegating to one agent and requiring him to sample a single solution with a certain level of effort costs $\$10$.
% The principal wants to maximize own expected utility given the budget constraint of $\$100$, and suppose that she has two options: (1) delegating to a single-agent and asking him to sample ten solutions, and (2) delegating to five agents and asking him to sample two solutions. In what follows, we investigate to answer this question in quantitative manner.
\end{example}
In what follows, we answer this question in  quantitative manner.
More formally, we provide comparative statics given the reasonable comparison between the single-agent and multi-agent setting, wherein our derivation of reasonable comparison follows from the intuition described in the example above.
Note that we obtain the result of similar flavor in Theorem~\ref{thm:recover}, but it only accommodates a reduction from a multi-agent instance to single-agent instance entirely to provide an approximation ratio of the multi-agent setting.
In this section however, we cement this result by showing that given any single-agent instance with arbitrary mechanism, we can construct a reasonable multi-agent instance such that there exists a multi-agent mechanism with principal's utility at least that under the original single-agent instance.
This result implies given any single-agent delegation problem instance, the principal can instead delegate to a reasonable set of multiple agents and obtain a superior utility. 
To this end, we first introduce how we construct a multi-agent instance from a single-agent instance.
\begin{definition}[Multi-agent correspondence]
Consider a single-agent problem with a distribution $D$, a number of solutions $k$, the agent's utility function $y$, and the principal's utility function $x$.
Consider a multi-agent problem with $n \ge 2$ agents in which the principal has the same utility function $x$ and each agent $i$ has a distribution $D_{i,j} = D$ for $j \in [k_i]$, a number of solutions $k_i$ such that $\sum_{i=1}^nk_i = k$, and the utility function $y_i = y$. We denote this multi-agent problem by multi-agent correspondence of the single-agent problem.
%\begin{enumerate}
%	\item there exists an agent $i$ with parameters $k_i = k$, $D_i =D$, and $y_i = y$. We denote this multi-agent problem a \emph{strong} $n$-agent correspondence of the single-agent problem.
%	\item each agent $i$ has a distribution $D_i = D$, a number of solutions $k_i$ such that $\sum_{i=1}^nk_i = k$, and the utility function $y_i = y$. We denote this multi-agent problem a \emph{weak} $n$-agent correspondence of the single-agent problem.
%\end{enumerate}
\end{definition}
%The strong $n$-agent correspondence refers to a strong version of benchmark in which the agent in the single-agent problem becomes one of the agents in the multi-agent problem.
%Intuitively, we expect this strong benchmark to be have better outcome in terms of the principal's utility, since the principal delegates to a strictly better pool of agents.
The above construction of multi-agent instance is reasonable.
This is because to see whether delegating to the multi-agent indeed brings advantages, it is fair to compare under the assumption that the agents exert the same total amount of effort in the task in both the single-agent and the multi-agent problem.
Since the number of solutions can be translated as the amount of effort exerted in the task, our definition of the multi-agent correspondence would play a reasonable role in comparing the single-agent and the multi-agent problem.
We present the proof in Appendix~\ref{pf_theorem:multi-agent-correspondence}

\begin{theorem}\label{theorem:multi-agent-correspondence}
Given a single-agent problem $P$, denote its multi-agent correspondence $P'$.
For any mechanism $M$ under $P$, there exists an MSPM under $P'$ such that the principal's utility of the MSPM under $P'$ is at least that of  $M$ under $P$.
\end{theorem}
%However in some sense, to see whether delegating to multi-agent indeed brings advantages, it is fair to compare under the assumption that the agents exert the same total amount of effort in the task in both the single-agent and multi-agent problem.
%We first present a result on the strong benchmark.
%\begin{theorem}
%Given a single-agent problem $P$, denote its strong $n$-agent correspondence $P'$.
%For any SPM with an eligible set in $P$, there exists a unit-budget RSPM with a homogeneous eligible set in $P'$ such that the principal's expected utility of the RSPM under any Nash equilibrium in $P'$ is at least that of the $SPM$ in $P$.	
%\end{theorem}
%\begin{theorem}
%Given a single-agent problem $P$, denote its weak $n$-agent correspondence $P'$.
%For any SPM with an eligible set in $P$, there exists a RSPM with a homogeneous eligible set and budget $B=n$ in $P'$ such that the principal's expected utility of the RSPM under any Nash equilibrium in $P'$ is at least that of the $SPM$ in $P$.
%\end{theorem}


The main take-away is that the principal can actually increase (at least not decrease) her utility by recruiting more agents with similar utilities to delegate the task, although this does not quantify whether the multi-agent delegation largely improves upon the single-agent setting.
\begin{remark}
    As we discussed in Section~\ref{sec:cost}, delegating to multiple agents induce a trade-off in examining the candidates in terms of the principal's resource, \eg time.
    Meanwhile, delegating to multiple agents already has its advantage in time consumption in the sense that it would take much smaller time for the entire process to be finished in the multi-agent delegation as each agent's task solving process is independent from each other and thus can be parallelized.
    We discuss more in the following example.
\end{remark}
\begin{example}
    Back to Example~\ref{ex:cs}, it is indeed the case the task requester can simultaneously request five workers to solve the task and save her time.
    Assuming that obtaining a single solution takes around five minutes.
    Roughly speaking, single-agent delegation with $10$ solutions requires $50$ minutes, whereas delegating to five agents with two solutions would take $10$ minutes.
    Afterward, the principal will examine the task.
    Suppose that the principal requires $t$ minutes to examine a single solution.
    In the single-agent scenario, overall time consumption is $50+t$.
    Note that $t$ is added back as the principal indeed has to examine the solution even though it is only one as the use of Bayesian mechanism (and thus decide whether or not to accept it) is essential in the single-agent setting.
    Meanwhile, the five agents scenario require $10+5t$.
    For any $t \le 10 = 5\cdot 2$, \ie when the principal can examine the solutions faster than twice of the time that each agent needs to find one solution, delegating to five agents still carries its own benefit even under the total examination.
    This will be even more true when the production function of the worker is concave, \ie, when they need more time to find a solution as they've already found some solutions.
    In short, multi-agent delegation may have both time and efficiency gains to some extents. 
\end{example}
% delegating to multi-agent still has benefits in the sense that 
% \begin{example}
% Consider the research proposal selection process we introduced in Section \ref{sec:intro}.
% Suppose that the grant agency wants to select a single research direction, and assume each investigators take one day to come up with a single research direction.
% The agency wants the agents to find at least $100$ research directions in total, and expect to select one of them.
% If the agency asks $10$ investigators to find $10$ research directions and propose one among them, it approximately requires $10$ days.
% On the other hand if the agency asks a single agent to find $100$ research directions, it would probably require almost $100$ days, which is indeed inefficient in terms of both the principal and the agent.
% On the top of the time efficiency presented in the example above, the competitive tension in the multi-agent delegated search increases the principal's actual utility as well.
% This again emphasizes the benefit of delegating to multiple agents.
% \end{example}

% If the agency asks $10$ investigators to sample $10$ research directions and propose one among them, it approximately requires 

% if we ask $10$ investigators to sample $10$ research directions (this can be interpreted as time window as well) and propose at most one solution each, rather than the scenario that we ask a single agent to find $100$ solutions and propose at most $10$ solutions.

==> Delegating to Multiple Agents (1)/conclusion.tex <==
\section{Conclusion}
In this paper, we present a thorough study on efficient delegation mechanisms against multiple agents, spanning the analysis of Bayesian/prior-independent mechanisms in complete/incomplete information settings 
%
%
%In this paper, we introduce a novel problem of delegation against multiple agents.
%To the best of our knowledge, this is the first to study the multi-agent extension by \citet{kleinberg2018delegated}.
%We conduct a comprehensive study on the multi-agent delegation mechanism, spanning the analysis of Bayesian/prior-independent mechanisms in both the complete/incomplete information settings.
We mainly reveal that the competitive tension arising from the multiple agents enables us to obtain efficient prior-independent mechanisms, in stark contrast to the Bayesian single-agent mechanism by \citet{kleinberg2018delegated}.
Furthermore, the gain from competition largely depends on the information available to the agents and the correlation between the agent's and the principal's utility, \eg it significantly degrades in the incomplete information setting with strongly negatively correlated utility.
Closing the gap between the approximation factors in various regimes and analyzing exact Bayes Nash equilibriums along with its efficiency in the incomplete information setting remains as major open problems.
In perspective of model, exploring the impact of examination costs more in details, endogenizing agents' costs to search/choose solutions, and studying the strategic tension arise from a repeated interaction would be interesting directions as well.

\begin{acks}
The work is partially supported by DARPA QuICC, NSF AF:Small \#2218678, and NSF AF:Small \# 2114269. 
\end{acks}

==> Delegating to Multiple Agents (1)/contribution.tex <==
\section{Overview of results}\label{sec:overview}
Before presenting the summary of our results, we briefly discuss our problem setup and some preliminaries.
We refer to Section~\ref{sec:setup} for a more formal problem setup.
In \emph{multi-agent delegation} problem,
there exists a principal who wants to find a solution for a task by
designing a mechanism that delegates the task to $n$ agents.
Each agent $i$ observes $k_i$ solutions by sampling from his own distributions, where both the number of solutions and the distributions are \emph{exogenous} to the mechanism.
These exogenous parameters can be interpreted as the intrinsic level of effort and skill of the agent.
Afterward, each agent proposes a subset of observed solutions (signal) to the principal.
Eventually, the mechanism selects a single solution, \emph{winner}, from the proposed ones.
% Agents are supposed to find solutions, in order to do so,
% they sample from their own distributions.
% Each agent may find a different number of solutions
% which indicates the level of effort that an agent commits to the problem that is exogenous from the mechanism.
% After finding solutions, each agent sends a subset of his sampled solutions to the principal
% and the mechanism designed by the principal selects a {\em winner} solution
% based on those subsets.  
If the solution $\omega$ is selected as the winner,
the principal receives the utility of $x(\omega)$.
If $\omega$ is proposed by agent $i$, he gets the utility of $y_i(\omega)$ while other agents realize the utility of zero.
Given the mechanism, each agent $i$ determines a (possibly mixed) strategy $\sigma_i$ to maximize own utility, which maps the observed solutions and information regarding others' solutions to the signal, and plays an action based on the strategy.
Importantly, we impose no restriction on the utility function $x(\cdot)$ and $y_i(\cdot)$, \ie they might be misaligned, which brings an interesting trade-off in designing the mechanism.
% The mechanism can reject all the solutions, which results in the utility of zero for both the principal and the agents.

We introduce technical notations to summarize our results.
Denote by $\omb_i = \{\om_{i,1}, \om_{i,2}, \ldots \om_{i,k_i}\}$  the agent $i$'s observed solutions for $i \in [n]$.\footnote{We use $[n]$ to denote $\{1,2,\ldots, n\}$ for $n \in \N$ throughout the paper.}
Define $X_{i,j} = x(\om_{i,j})$ for $i \in [n]$ and $j \in [k_i]$.
Sort $X_{i,j}$ for $j \in [k_i]$ in decreasing order, and denote by $X_{i,(1)} \ge X_{i,(2)} \ge \ldots \ge X_{i,(k_i)}$.
We denote by $X_{i,(1)}$ the first-best solution of agent $i$.
Again, sort $X_{i,(1)}$ for $i \in [n]$ in decreasing order, and obtain $X_{(1)} \ge X_{(2)} \ge \ldots \ge X_{(n)}$.
Let the owner of $X_{(i)}$ be the $i$-th best agent.
We often overwrite $X_{(1)}$ by $X_{\max}$.
Our benchmark of the mechanism is $\Ex{X_{(1)}}$, \ie the case when the principal can select the best one by directly accessing all the observed solutions.
% Let's enumerate agents from $1$ to $n$ and denote by
% $k_i$, the number of solutions that agent $i$ samples,
% and by $\omb_{i} = \{\omega_{i, 1}, …, \omega_{i, k_i}\}$,
% the multi-set of solutions sampled by agent $i$.
% Define $X_{i, j} = x(\omega_{i, j})$ for all agent $i \in \left[n\right]$ and each $j \in \left[k_i\right]$.
% Furthermore, we denote by $X_{i, (j)}$ the $j$-th highest solution in $\omb_i$
% in terms of $x(\cdot)$ so that $X_{i, (1)} \geq X_{i, (2)} \geq ... \geq X_{i, (k_i})$.
% Finally, we use $X_{(k)}$ to show the $k$-th highest solutions among the best solutions of agents.
% Formally, we have $X_{(1)} \geq X_{(2)} \geq ... \geq X_{(n)}$,
% and $\{X_{(1)}, X_{(2)}, ..., X_{(n)}\} = \{X_{1, (1)}, X_{2, (1)}, ..., X_{n, (1)}\}$ \keivan{not true! I need to define $X_{\max}$ somewhere}.
% In the ideal setting where the principal could directly investigate all the sampled solutions,
% she would select the solution corresponding to the utility of $X_{(1)}$.
% As a result, the principal's expected utility would be $\Ex{X_{(1)}}$.
% So, in order to evaluate a mechanism, we should compare the principal's expected utility under that mechanism to $\Ex{X_{(1)}}$.
Let $f_{M,\sigma}$ be an interim allocation function which specifies the outcome under the mechanism $M$ and some strategies $\sigma$, given a realization of the solutions.
Then, given some strategies $\sigma$ of the agents, we say that mechanism $M$ is $(\rho, \gamma)$-approximate if 
\begin{align*}
\rho \Ex{f_{M,\sigma}} + \gamma \geq \Ex{X_{(1)}}.
\end{align*}
We denote by $\rho$ and $\gamma$ the multiplicative and additive approximation factors, respectively.
We say that $M$ has multiplicative \emph{price of anarchy} ($\poa_m$) of $\rho$ if it is $(\rho,0)$-approximate under \emph{any Nash equilibrium} of agents' strategies, and it has multiplicative \emph{price of stability} ($\pos_m$) of $\rho$ if there exists \emph{a Nash equilibrium} such that $M$ is $(\rho,0)$-approximate. We similarly define $\poa_a$ and $\pos_a$ to denote the price of anarchy/stability for $(1,\gamma)$-approximation, \ie  additive approximation factor.\footnote{See Definition~\ref{def:apx-mech} and \ref{def:poa-pos} for more details.}


% \suho{how about "... to the problem that is exogenous from the mechanism". My point is, since there exists a line of economics literature that makes this choice of effort level to be a strategic choice as well (contract theory based delegation), we need to emphasize that we assumed that this is an exogenous parameter that is given as a part of problem instance.} \keivan{I see your point, I changed it.}

\subsection{Contributions and techniques}
We here summarize our key results and the major techniques therein.
Basically, we analyze two types of mechanisms: (1) Bayesian mechanism (BM) with knowledge of the prior distributions, and (2) prior-independent mechanism (PIM) which does not know the distributions in advance.
We further consider complete and incomplete information settings.
In the complete information setting, each agent knows the others' observed solutions while in the incomplete information setting, he only knows the distributions from which the others sample, but not the realized solutions.

We begin by showing that any mechanism can be reduced to a \emph{multi-agent single-proposal} mechanism (MSPM, Definition~\ref{def:mspm}) in Theorem \ref{thm:multiagent_revel}.
% MSPM is an extension of single-proposal mechanism by~\citet{kleinberg2018delegated}, and the formal definition can be found in Definition~\ref{def:mspm}.
% In MSPM, the principal announces an eligible set for each agent.
% Each agent is required to propose only a single solution, which we refer to as \emph{candidate}.
% Then, the principal filters the candidates which do not belong to the corresponding eligible sets and selects the candidate that maximizes her own utility function.
Essentially, this theorem implies that we can narrow down our scope of interest to the space of the MSPMs.
We note that the MSPM can be either BM or PIM depending on whether the mechanism uses the knowledge on the distributions or not.
All the positive results we present below will be built upon MSPMs.

\paragraph{General result in the complete information setting}
We start with the general result on MSPM.
\begin{customthm}{\ref{theorem:multi-agent-unlimited-budget}}
\label{thm:1.1_informal}
    In the complete information setting, for any $\tau \ge 0$, there exists a MSPM with $\poa_a$ of
	\begin{align*}
		\Ex{X_{(1)} - X_{(2)}\IND[X_{(2)}\ge \tau] - \tau \IND[X_{(1)} \ge \tau > X_{(2)}]}
        .
	\end{align*}
\end{customthm}
Intuitively, the first-best agent needs to guarantee that he will be selected by the principal while maximizing his own utility.
This motivates him to propose a solution that yields the principal's utility at least that of the first-best solution of the second-best agent.
The proof is built upon such simple intuition, however, it is still tricky to characterize arbitrary (possibly mixed) Nash equilibrium of the agents, and the formal proof can be found in Appendix~\ref{pf_theorem:multi-agent-unlimited-budget}.
This result implies that the additive approximation factor is characterized by the difference between $X_{(1)}$ and $X_{(2)}$, \ie the difference of first-best solution between the first-best and second-best agents.
On top of it, the principal can also smartly define the threshold $\tau$ using the prior information, and further improve the quality of the candidates, although it may decrease the probability of the acceptance.

\paragraph{BM in the complete information setting}
From the general result, we obtain the following result on BM which recovers the single-agent guarantee in \citet{kleinberg2018delegated}.
% first show that we can recover the guarantees achieved by the single-agent setting presented in \citet{kleinberg2018delegated}, by using BM.
\begin{customthm}{\ref{thm:recover} and \ref{thm:lowerbound_comp_worst}}\label{thm:recover_informal}
        In the complete information setting, there exists a BM with $\poa_m$ of $2$.
    In addition, this multiplicative approximation factor is tight, \ie there exists a problem instance that no BM can achieve $\pos_m < 2-\eps$.
\end{customthm}


\begin{table}[]
\centering
\resizebox{11cm}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Information}                                                                 & \textbf{Bound} & \textbf{General}   & \textbf{Symmetric $\alpha$-decaying}
\\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ Complete\end{tabular}}}   & Lower     &$\pos_m \ge 2$ \quad ( Thm \ref{thm:lowerbound_comp_worst}) & open 
\\ \cline{2-4} 
& Upper&$\poa_m \le 2$ \quad (Thm \ref{thm:recover})& $\poa_m \le \parans{\frac{\alpha nk}{\alpha nk+1}}^{\frac{-1}{\alpha nk}}$  (Thm \ref{thm:informed}) \\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ Incomplete\end{tabular}}} & Lower & $\pos_m \ge 2$ \quad (Cor \ref{thm:recover_bayes})& open 
\\ \cline{2-4} & Upper & $\poa_m \le 2$ \quad (Cor \ref{thm:recover_bayes})& $\poa_m \le \parans{\frac{\alpha nk}{\alpha nk+1}}^{\frac{-1}{\alpha nk}}$  (Cor \ref{thm:recover_bayes}) \\ \hline
\end{tabular}
}
% \vspace{0.1cm}
\caption{Summary of results on Bayesian mechanism.  \emph{Symmetric} refers to the symmetric agents and \emph{$\alpha$-decaying} denotes the distributions such that its c.d.f. $F$ satisfies $F(x) \le x^{\alpha}$ for some $\alpha > 0$. Lower bounds for the symmetric setting remain as open problems.}
\vspace{-5mm}
\label{table:1}
\end{table}


The upper bound follows from the reduction from multi-agent setting to single-agent setting, where we in fact obtain stronger comparative statics such that the multi-agent delegation is always superior to the single-agent delegation.
We discuss a more detailed comparison between the single-agent and multi-agent settings in Appendix~\ref{sec:compare_mul_sin}.
The lower bound is obtained by introducing a concept of \emph{super-agent} equipped with the standard worst-case instance in prophet inequalities.
% To prove the theorem above, we mainly use the fact that multi-agent delegated search can be reduced to a single-agent delegated search, presented by \citet{kleinberg2018delegated}.
% The lower bound is obtained by introducing \emph{super-agent} with dominantly qualified solutions, combined with the standard worst-case instance for prophet inequalities.
% The problem instance for lower bound follows from the standard worst case instance for prophet inequalities, and by introducing an existence of 
% its connection to our problem by constructing a worst-case distribution over the agents in which there exists a \emph{super-agent} whose sampled solutions are always strictly dominant over other agents' solutions in terms of the principal's utility.
This worst-case instance implies that there is no merit in delegating the task to multiple agents with highly \emph{asymmetric} levels of skill.

We then naturally consider a \emph{symmetric} case (see Definition \ref{def:symmetric}) when the agents are equipped with the same parameters, \ie they have similar levels of skill and effort.
% This naturally leads us to consider cases in which there do not exist any agents who are dominant over other agents or dominated by others. Roughly speaking, we should analyze multi-agent delegated search in cases where all the agents have similar levels of skill in solving the task. To this end, we restricted our focus to cases in which all the agents are equipped with a single distribution $D = D_{i,j}$ and a same number of solutions.
% We denote this case by \emph{symmetric agents} (for formal definition, please see Definition~\ref{def:symmetric-agent}).
In this case, for a certain class of distributions, we show that the multiplicative approximation factor can be subconstant for BM, \ie converges to $1$ as $n$ (the num. of agents) or $k$ (the num. of solutions per agent) increases.
\begin{customthm}{\ref{thm:informed}}\label{thm:subconstant_informal}
    In the complete information setting, consider the symmetric agents with $X_{i, j} \sim D$ where $D$ is a distribution supported on $[0,1]$ and the cumulative distribution function (c.d.f.) of $F(x)$ satisfies $F(x) \le x^{\alpha}$ for some $\alpha > 0$.
    Then, there exist a BM with $\poa_m$ of $\parans{\frac{\alpha nk}{\alpha nk+1}}^{-\frac{1}{\alpha nk}}$. Hence, the principal's expected utility converges to $\Ex{X_{\max}}$ as $n$ or $k$ increases.
\end{customthm}
To obtain the subconstant bound above, we use threshold-based eligible sets that are tighter than the ones used in the prophet inequalities.
%Combined with the fact that the agents are symmetric, we obtain a subconstant bound followed by an elementary level of analysis.
We present the summary of results for BM in Table~\ref{table:1}.

%
%\kvdelete{I think here we need to motivate more why prior-independent case is more interesting and practical as most of our results are in this setting}
%\ssdelete{I think this motivation needs to be located in introduction, or model section, instead of contributions section. But I agree that this motivation is important - See Information Structure paragraph}

\paragraph{PIM in the complete information setting}
For PIM, we observe that Theorem~\ref{thm:1.1_informal} yields an additive approximation factor of $\Ex{X_{(1)}- X_{(2)}}$ by setting $\tau = 0$ (see Corollary~\ref{cor:infbud_notau}).
This indeed requires no prior knowledge as it accepts any solution.
On the other hand, we argue that this guarantee can be arbitrarily bad if we do not restrict our problem instances to symmetric agents.
\begin{customthm}{\ref{thm:comp_obl_neg}}\label{thm:arbbad_informal}
    In the complete information setting, suppose that principal's utility function lies in $[0,L]$ for some $L>0$.
    Then for any $\eps > 0$, there exists a problem instance such that no PIM can achieve $\pos_a \le L-\eps$.
\end{customthm}
The proof is based on a construction worst-case instance with a super-agent similar to the lower bound under the general setting in BM.

We thus consider the symmetric agents and derive the following result.
\begin{customthm}{\ref{thm:comp_sym_general}}
    In the complete information setting, consider symmetric agents with the principal's utility function lies in $[0,L]$ for some $L>0$.
    Then, there exists a PIM with $\poa_a$ of $(1-\frac{1}{n})^{n-1}$.
    % This upper bound is tight, \ie no mechanism can achieve 
    % $\pos_a \le (1-\frac{1}{n})^{n-1} - \eps$ for any $\eps >0$.
%    $\pos_a \le \eps$ when $\eps < (1-\frac{1}{n})^{n-1}$.
\end{customthm}
Note that $(1-\frac{1}{n})^{n-1} \le 1/2$ for all $n \ge 2$, and decreases to $\nicefrac{1}{e}$ as $n$ increases.
This constant approximation is a big improvement over the arbitrarily bad approximation in the general setting.


Next, we improve the approximation factors of PIM to be subconstant with respect to some canonical family of distributions.
At the heart of this analysis, we come up with several new results (see Lemma \ref{lm:order_stat_diff}, \ref{lm:mhr_preserving}, \ref{lm:order_stat_diff_restricted}, and \ref{lm:id_preserving}) in order statistics\footnote{Given $n$ i.i.d. samples, $r$-th order statistics refer to the $r$-th smallest value among the i.i.d. samples.}, which might be of independent interest.
Detailed discussions are presented in Section \ref{sec:comp_pim}.
\begin{customthm}{\ref{thm:mhr_upperbound} and \ref{thm:decaying_upperbound}}
    In the complete information setting, consider symmetric agents such that $X_{i, j} \sim D$ where $D$ is a distribution with a probability distribution function (p.d.f.) of $f(x)$.
    Let $D_{\max}$ be the distribution of $X_{i,(1)}$ for any $i \in [n]$. 
    Denote by $\var(\cdot)$ the variance of a distribution.
    Then, the following holds.
    \begin{enumerate}
	\item If $D$ has MHR (see Section~\ref{sec:comp_pim} for definition), then there exists a PIM with $\poa_a$ of $\sqrt{\frac{4\var(D_{\max})}{3}}$. In case of $D = U[0,1]$, we have $\sqrt{\frac{4\var(D_{\max})}{3}} = \sqrt{\frac{4k}{3(k+1)^2(k+2)}} \approx \frac{1.155}{k}$.
	\item If $f(x)$ is nondecreasing on $x$, then there exists a PIM with $\poa_a$ of $\frac{\sqrt{12\var(D_{\max})}}{n+1}$. In case of $D = U[0,1]$, we have $\frac{\sqrt{12\var(D_{\max})}}{n+1} = \frac{1}{n+1}\sqrt{\frac{12k}{(k+1)^2(k+2)}} \approx \frac{3.464}{k(n+1)}$.
    \end{enumerate}
\end{customthm}

\paragraph{Incomplete information setting}
In the incomplete information setting, we first discuss that the results on the BM, Theorem~\ref{thm:recover_informal} and Theorem~\ref{thm:subconstant_informal}, still carry over in the incomplete information setting.
In addition, without the assumption of symmetric agents, we still have an arbitrarily bad lower bound in the approximation ratio for any PIM, \ie Theorem~\ref{thm:arbbad_informal} still holds.
This justifies our assumption of symmetric agents in the incomplete information setting as well.
Interestingly, however, assuming the symmetric agents is not sufficient to derive a positive result.
\begin{customthm}{\ref{thm:pim_neg_incomp}}
    In the incomplete information setting, under symmetric agents with $X_{i,j} \sim U[0,1]$, there is a problem instance where no PIM has $\poa_a < \frac{k-1}{k+1} - \sqrt{\frac{\log n}{2k+3}}$.
\end{customthm}
Note that by making $k$ arbitrarily large give $n$, RHS can be arbitrarily close to $1$.
The proof is based on a construction of strongly negatively correlated utility between the principal and the agents, preceded by some algebraic manipulations.
% This result stems from the fact that we can construct a problem instance in which the principal's and the agent's utility functions are strongly negatively correlated. 
Interestingly in this problem instance, each agent's utility decreases by playing for sake of the principal.
Hence, each agent settles with a solution that gives the agent largest ex-post utility (and thus smallest principal's utility), even though it yields a small probability to be selected.
We present the result for uniform distribution for simplicity, but we in fact provide a more general result.

\begin{table}
\centering
\resizebox{14cm}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Information}  & \textbf{Bound} & \textbf{General}  & \textbf{Symmetric (Sym)}   & \textbf{Sym MHR}  & \textbf{Sym Inc}  & \textbf{Sym Ind}            
\\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ Complete\end{tabular}}}   & Lower      & \begin{tabular}[c]{@{}c@{}}$\pos_a \ge L$\\ Thm \ref{thm:comp_obl_neg}\end{tabular} &
Open
% \begin{tabular}[c]{@{}c@{}}$\pos_a \ge \parans{1-\frac{1}{n}}^{n-1}\cong \frac{1}{e}$\\ Thm \ref{thm:comp_sym_general}\end{tabular}
& Open & Open   & Remark \ref{remark:just_table2}  
\\ \cline{2-7} 
& Upper      & Cor \ref{cor:infbud_notau}   & \begin{tabular}[c]{@{}c@{}}$\poa_a \le L\parans{1-\frac{1}{n}}^{n-1}\cong \frac{L}{e}$\\ Thm  \ref{thm:comp_sym_general}\end{tabular}  & \begin{tabular}[c]{@{}c@{}}$\poa_a \le \frac{1.15}{k}$\\ Thm \ref{thm:mhr_upperbound}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\poa_a \le \frac{3.46}{k(n+1)}$\\ Thm \ref{thm:decaying_upperbound}\end{tabular} & Remark \ref{remark:just_table2}  
\\ \hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\\ Incomplete\end{tabular}}} & Lower  & \begin{tabular}[c]{@{}c@{}}$\pos_a \ge L$\\ Cor \ref{thm:pim_lower}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\poa_a \ge \frac{k-1}{k+1} - \sqrt{\frac{\log n}{2k+3}}$\\ Thm \ref{thm:pim_neg_incomp}\end{tabular} & Remark \ref{remark:just_table} & Remark \ref{remark:just_table}& Open \\ \cline{2-7} & Upper      & Remark \ref{remark:just_table3} & Remark \ref{remark:just_table}   & Remark \ref{remark:just_table} & Remark \ref{remark:just_table} & \begin{tabular}[c]{@{}c@{}}$0.39$-$\pos$ is $\opt$\\ Thm \ref{thm:bayes_oblivious} \end{tabular} \\ \hline
\end{tabular}
}
% \vspace{0.1cm}
\caption{Summary of results on prior-independent mechanism. \emph{ MHR} refers to MHR distribution, \emph{ Inc} refers to nondecreasing p.d.f., and \emph{Sym Ind} refers to independent utility setting with the uniform distribution $U[0,1]$.
\emph{Open} denotes that this regime remains an open problem.
For general case lower bound for both settings, and symmetric case upper bound in the complete information setting, we assume that the support of the principal's utility function lies in $[0,L]$. For Sym MHR, Sym Inc, and lower bound in the incomplete information setting under Sym, we present the results for $U[0,1]$ for brevity.}
 \vspace{-6mm}
 \label{table:2}
\end{table}

In this context, we additionally consider an \emph{independent utility} assumption in which the agents' and principal's utilities are independent of each other (see Definition~\ref{def:indep-utility} for more details).
Then we show that there exists a good approximate Bayes Nash equilibrium (BNE) (see Definition \ref{def:apxbne} for more details) such that the principal's expected utility becomes exactly optimal.
%, when the principal's utility over the solution is sampled from a uniform distribution $U[0,1]$.
\begin{customthm}{\ref{thm:bayes_oblivious}}
    In the incomplete information setting, consider symmetric agents and independent utility assumption such that $X_{i,j},Y_{i,j} \sim U[0,1]$.
    Then, there is an optimal PIM with $\beta$-approximate BNE where $\beta = 1-\exp\parans{\frac{-n^2}{2(n-1)^2}}$.
    Note that $\beta$ becomes $0.3935...$ as $n$ grows.
%    The second term in $\beta$ converges to $\nicefrac{1}{\sqrt{e}} = 0.6065...$ as $n$ increases.
\end{customthm}
Different from the complete information setting, deriving and analyzing BNE is far more challenging, especially for our problem setup.
One reason is that the feasible action of an agent depends on the realization of his solution.
In addition, computing the expected payoff of an agent's strategy requires us to compute the expectation over every possible realization of the others' solutions.
Despite these difficulties, we obtain the above result, of which the proof heavily relies on the FKG inequality (Lemma \ref{lm:FKG}) and some properties on the joint density function of two order statistics, preceded by some algebraic manipulations.
% Our proof is based on analyzing the probability that the principal's and the agent's utility is somehow aligned, i.e., an agent maximizes his expected utility by proposing his best solution in terms of principal. We show that this probability is lower bounded by $1-\exp \parans{\frac{-n^2}{2(n-1)^2}}$, which is at least $1-\frac{1}{\sqrt{e}}$.
% some absolute constant that does not depend either on $n$ or $k$ \keivan{correct?}.
% The proof heavily relies on the FKG inequality (Lemma \ref{lm:FKG}) and some properties on the joint density function of two order statistics.
Using a similar but more involved technique, in Appendix~\ref{sec:correlated_equi}, we show that there exists a PIM such that under some \emph{Bayes correlated equilibrium}, it achieves a multiplicative approximation factor of $\exp\parans{\frac{n^2}{2(n-1)^2}} \cong 1.649$ (as $n$ increases).
%$\parans{\exp\parans{\frac{-n^2}{2(n-1)^2}},0}$-approximation.
We present the summary of results on PIM in Table~\ref{table:2}.
We remark on some points regarding the table as follows.
\vspace{-5mm}
\begin{remark}\label{remark:just_table}
    We do not study the upper bound for symmetric agents in the incomplete information setting because the lower bound in this setting can be arbitrarily bad for certain problem instances.
    In addition, we do not consider Sym MHR and Sym INC in the incomplete information setting since the lower bound in the symmetric setting already implies a pessimistic result.
\end{remark}
\vspace{-3mm}
\begin{remark}\label{remark:just_table2}
    Since the complete information setting inherently admits positive results only with the symmetry assumption, we do not consider the symmetric agents and independent utility scenario in the complete information setting.
\end{remark}
\vspace{-3.5mm}
\begin{remark}\label{remark:just_table3}
    The upper bound for the general incomplete information setting is not studied, as one can easily obtain a mechanism with an approximation ratio of $\infty$, \eg a mechanism that selects a solution to maximize the agent's utility.
\end{remark}

\paragraph{Examination cost}
Finally, we study an extension to consider the examination cost of the mechanism.
The examination cost of a mechanism is defined by the number of candidates that the mechanism has to access to choose the winner.
We refer to Definition~\ref{def:exam} for more details.
In this extension, we obtain the following result of a similar flavor to Theorem~\ref{theorem:multi-agent-unlimited-budget}.
\begin{customthm}{\ref{theorem:multi-agent-limited-budget}}
    Define $X_{(n + 1)} = -\infty$.
    For any $\tau \ge 0$, there exists a mechanism with examination cost $2 \le B < n$ such that $\poa_a$ is at most,
    \begin{align*}
    \Ex{X_{(1)}}
    -
    \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau > X_{(B+1)}\right] -  \tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]
    -
    \sum_{e=B+1}^{n} X_{(e-B+2)}\IND\left[X_{(e)} \geq \tau > X_{(e+1)}\right]}.
    \end{align*}
\end{customthm}
This depicts the trade-off between the examination cost and the approximation ratio.
Indeed, $\poa$ increases as $B$ decreases, and plugging $B = n$ carries over to the bound in Theorem~\ref{theorem:multi-agent-unlimited-budget}.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}




% No contingent monetary transfer between the officer and researcher is allowed upon the selection of final solution, however, the researcher's utility becomes positive only when his solution is finally adopted.
% For example, he may be funded some budget to perform the experiments based on the solution, may be prompted, or may receive a good annual performance review.
% In this context, how should the officer restrict the soltuion space fo 

% Such a delegation of task broadly happens in a variety of real-world situations.
% When a decision-maker is faced with a challenging task that cannot be solved by her own, her best plan would be to delegate the task into some experts, and 


% Such a scenario involving the delegation of the task broadly happens in a variety of real-world situations, mostly for which the decision-maker is faced with a challenging problem that cannot be solved by her own.


% In a long line of literature in optimal delegation (cite), 


% Furthermore, this falls into the area of mechanism design without money due to the restriction of no monetary transfer
% To overcome such a challenge, a rich literature has studied the 
% This imparts a structural restriction on the reasonable mechanisms, 


==> Delegating to Multiple Agents (1)/exam_cost.tex <==
\section{Examination cost}\label{sec:cost}
Since we allow multiple agents to propose a solution, on one hand, it helps the principal find a better solution because she can compare more solutions as observed in Section~\ref{section:no_cost} and \ref{section:no_cost_incomp}.
On the other hand, since the principal needs to select which ones to choose among the multiple candidates,
it entails an additional burden to \emph{evaluate} the candidates, compared to
the single-agent setting.

\begin{example}
Suppose that a project manager delegates the task of finding a solution for a project
to multiple teams.
Each team proposes a candidate and then
the manager needs to find the best candidate by
sequentially examining the candidates.
This procedure can be costly for the manager and even
cannot be parallelized since the manager may want to examine the candidates by herself.
\end{example}

To effectively study the trade-off between such a burden in evaluating the candidates and the principal's utility,
we introduce the following notion of the examination cost of a mechanism.

\begin{definition}[Examination]\label{def:exam}
Given a set of solutions $\omb \in \Omega^*$ and corresponding strategies $\sigma$,
suppose that mechanism $M$ can eventually choose a winner among a subset $p \subset \omb$.
The mechanism cannot directly access the subset $p$, and does not have information on their values,
but only knows from whom each candidate in $p$ is proposed.
In order to select the winner,
the mechanism should examine the solution by accessing each candidate in $p$, and this incurs an \emph{examination cost} of $1$.
We call this procedure an examination process.
\end{definition}

It is important to note that the principal may randomize the examination process.
We further denote that a mechanism has \emph{(examination) budget} $B$, if its total cost of examination does not exceed $B$ for any realized set of solutions and any corresponding strategies.
% For example, she may randomly select any candidate and commit to it.
% This process, in reality, may not entail any cost to the principal in examining the outcomes since she can just commit to it without verifying it, however, we assume that such a mechanism also has an examination budget $1$ in order to prevent any confusion arising from it.
% As we are only interested in comparing the efficiency of mechanisms having a fixed examination budget, this assumption indeed does not impose any restriction on our results.

% \begin{definition}[Examination budget]
% We say that mechanism $M$ has an examination budget $B$,
% if its total cost of examination does not exceed $B$
% for any realized set of solutions $\omb \in \Omega^*$ and any corresponding strategies $\sigma$.
% In case $B=1$, we say that $M$ has a unit budget.
% \end{definition}
We aim to study the trade-off between the examination budget $B$ and the approximation factor of a mechanism.
Unlike the previous results in which the MSPM can examine all the candidates proposed by the agents and commit to the best one, if the examination budget is finite, the principal should selectively examine them.
In this context, we present the following variant of MSPM.
\begin{definition}[Randomized single-proposal mechanism]
In a \emph{randomized single-proposal mechanism (RSPM)} with budget $B$, a tie-breaking rule $\rho$, an eligible set $R_i \subset \Omega$ are announced by the principal for each agent $i$.
Each agent proposes up to one solution, and the principal selects $B$ candidates uniformly at random and adopts the one of them to maximize her utility.
\end{definition}
Note that RSPM with budget $B$ always examine at most $B$ candidates.
As it can be observed in the definition of the RSPM, once a candidate $\om \notin R_i$ is submitted by agent $i$, there is no chance of getting accepted by the mechanism.
This implies that there is no incentive for the agent to submit a candidate beyond the eligible set.
In this context, we impose the following mild assumption.
\begin{assumption}[Rationality]\label{as:rationality}
Given a RSPM $M$ with arbitrary tie-breaking rule $\rho$ and eligible sets $R_1,\ldots, R_n$, each agent $i$ for $i \in [n]$ does not play strategy $\sigma_i = \om$ if $\om \notin R_i$.
\end{assumption}
% This assumption is indeed practical since (i) each agent himself would be aware of the quality of the submission, and (ii) the principal may punish such behavior exogenously, for example, the management may reflect a bad annual review to the divisions with these undesired behaviors.

In Section ~\ref{section:no_cost} and \ref{section:no_cost_incomp}, we assume that the principal can examine  all candidates (at most $n$) and takes the best one as the winner, \ie the principal has a sufficient budget $B \ge n$.
%In Section ~\ref{section:no_cost} and \ref{section:no_cost_incomp},
%we assume that the principal has a sufficient budget, i.e.,
%she can examine all candidates (at most $n$) and takes the best one as the winner. 
%Hence, we implicitly assume that $B = n$. 
To study the nontrivial effect of examination cost, we assume that the budget is \emph{not sufficient} to examine all the candidates, \ie $B < n$.
We analyze RPSM in the complete information setting by generalizing Theorem~\ref{theorem:multi-agent-unlimited-budget} in Section~\ref{section:no_cost} to the limited budget case.

\begin{theorem} \label{theorem:multi-agent-limited-budget}
Given any $\tau \ge 0$, let $R$ be an eligible set with threshold $\tau$ such that $R:= \{\omega: x(\omega) \ge \tau, \omega \in \Omega\}$ and $\rho$ be an arbitrary deterministic tie-breaking rule.
Let $X_{(n + 1)} = -\infty$.
Given $2\leq B < n$, RSPM with $\rho$ and
a~homogeneous eligible set $R$ has $\poa_a$ of at most
\begin{align*}
\Ex{X_{(1)}
-
X_{(2)}\IND\left[X_{(2)} \geq \tau > X_{(B+1)}\right] -  \tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]
-
\sum_{e=B+1}^{n} X_{(e-B+2)}\IND\left[X_{(e)} \geq \tau > X_{(e+1)}\right]}.
\end{align*}
% where we abuse $X_{(n + 1)} = -\infty$.
\end{theorem}
Its proof structure follows that of Theorem~\ref{theorem:multi-agent-unlimited-budget}, but is more involved due to the randomness in the mechanism.
Formal proof is deferred to Appendix~\ref{pf_theorem:multi-agent-limited-budget}.
This result depicts the trade-off between the budget and the the efficiency of a mechanism.
Indeed, the upper bound on $\poa$ presented above decreases as $B$ increases, and by plugging $B=n$ we can exactly recover the guarantee provided in Theorem~\ref{theorem:multi-agent-unlimited-budget}.
This is fairly intuitive as if the principal can evaluate more candidates, then she can commit to more efficient solutions.
Similar to Remark~\ref{rm:bm_pim_comp}, RSPM can be either BM or PIM depending on the choice of the eligible sets.
% If it announces eligible sets $\{R_i\}_{i=1}^{n}$ based on the knowledge over the distributions in advance, then it would be a BM mechanism.
% However, if the mechanism does not determine eligible sets, i.e. $R_i = \Om$, then it would be a PIM.
For PIM, we can directly obtain the following result.
\begin{corollary}\label{cor:limbud_notau}
    There exists a PIM having budget $B$ with $\poa_{a}$ of $\Ex{X_{(1)}} - \Ex{X_{(n-B+2)}}$.
    % in which the delegation gap is upper bounded by $\Ex{X_{(1)}} - \Ex{X_{(2)}}$.
\end{corollary}

Importantly, quantifying the additive approximation factor in Corollary~\ref{cor:limbud_notau} is intrinsically more challenging than the previous result
without the examination cost,
since we need to deal with the expected difference of two order statistics which are not consecutive.
One straightforward approach would be to simply sum up the bound for two consecutive ones, but we found this bound to be cumbersome and couldn't find any take-away.
Analyzing or simplifying this gap for arbitrary budget $B$ and deriving analogous results as in Section~\ref{section:no_cost} remains a major open problem.

Although RSPM has the benefit of its simplicity, however, it is not a clever choice as it examines the candidates in uniformly at random. A better approach might be to exploit the prior information on the distributions regarding the quality of candidates, which might be an interesting topic.
% Designing an efficient Bayesian mechanism in a limited budget setting would be a very interesting topic.


==> Delegating to Multiple Agents (1)/experiment.tex <==



\section{Numerical Experiments on the Tightness of Theorem \ref{thm:bayes_oblivious}}\label{app:c}
We here numerically verify that the lower bound on $\Pr{E}$ obtained in the proof of Theorem~\ref{thm:bayes_oblivious}, \ie $\exp\parans{-\frac{n^2}{2(n-1)^2}}$, is almost tight.
Figure~\ref{fig:num-exp-pim} represents $\Pr{E}$ with respect to the value of $n$ for some choices of $k$.
To obtain the true value of probability of the event $E$, we simulate the principal and agents and compute the frequency of the event that each agent's utility is aligned, \ie proposing a solution that maximizes the principal's utility also maximizes the agent's utility, for every agent.
To present some details in the experiment, we consider $n = \{5, 10, 20, 50, 100, 200, 300, 400\}$ and $k = \{10, 20, 100, 150, 1000\}$.
For each pair of $n$ and $k$, we run $30000$ times to compute the probability that the event $E$ happens.
We repeat this procedure $60$ times to obtain the variance for each setting, which is plotted as the shade in the figure.
The main take-away here is that the lower bound and the average value of the quantity $\Pr{E}$ is indeed becoming tight as $n$ increases.
As a side note, one can observe that as $n$ increases the precision error appears in each experiment (shade) becomes wider.
This is because large $n$ introduces more randomness in each experiment which requires more samples to stabilize its average, and thus we believe it not to be a meaningful phenomenon.
\input{figures/figure.tex}

==> Delegating to Multiple Agents (1)/figures/figure.tex <==
% !TEX root = ../main.tex
\begin{figure}[tbp]
\centering
    \hspace{-6mm}
    \includegraphics[width=12cm]{figures/plt-v2.pdf} 
    \caption{
    Probability of the event $E$ defined in~\eqref{ineq:01231307}.
    Lowerbound refers to the lower bound of the event $E$ that we obtained in \eqref{ineq:01062049}, and $n$ and $k$ denotes the number of agents and the number of solutions per agent. We note that $x$-axis is presented in the base of the natural number $e$.
    }
    \label{fig:num-exp-pim}
\end{figure}
  

==> Delegating to Multiple Agents (1)/intro.tex <==
\section{Introduction}\label{sec:intro}
In many real-world situations, a decision-maker (called "principal") is encountered with a difficult task that cannot be solved by herself.\footnote{Throughout the paper we use feminine pronouns to denote the principal and masculine pronouns to denote the agents.}
To cope with it, she delegates the process of finding a solution to several agents who have the ability to solve the task, and then examines agents' proposed solutions to take the best one.
An interesting tension arises when the utility of the agents are not aligned with that of the principal.
% An interesting tension that arises in such a procedure is that the utility of the agents may not be aligned with that of the principal.
Since the agents are self-interested to maximize their own payoff, they may not propose the solutions for sake of the principal. 

As a concrete example, consider a research proposal selection process by a grant agency. In this problem, a {\em principal} (\eg the grant agency) introduces a topic for proposals  and asks each {\em agent} (\eg a principal investigator) to send a private proposal, or a set of proposals, based on a set of his research directions (possibly coming from some distribution) related to the topic introduced by the principal.
Each proposal has some valuation for the agent and some valuation for the principal which can be different (\eg a proposal may be more aligned with a research direction by the agent but less aligned with the principal's interests). 
The goal of the principal is to {\em maximize} own valuation of the finally selected proposal while the goal of each agent is to maximize his utility which is his valuation for a proposal selected by the principal and zero otherwise.

In this example, the principal faces a problem of \emph{mechanism design without money} to incentivize the agents to behave more in favor of her.
In practice, the setting here can be an {\em incomplete information} game in the sense that though an agent knows the topic introduced by the principal and general research topics of the other agents (\ie distributions of possible proposals), he may not know the exact topics that other agents consider for their proposals.
In addition, the principal may have an {\em examination cost} (\eg travel cost for time-consuming site visits) for each proposal which should be accounted for in the proposal selection process as well. 
% In designing an efficient delegation mechanism, the principal may adopt a \emph{Bayesian mechanism} (BM) by exploiting the historical information regarding the solution of the agents (i.e., she knows the distributions from which the agents have submitted proposals in the past),  or should stick with \emph{prior-independent mechanism} (PIM) due to the absence of such information (i.e., she does not have any prior knowledge regarding the agents'  past proposals).
A fundamental question in this example is how should the principal design a mechanism to maximize her own utility function.

%
%\note{previous example}
%For example, consider a scenario in which a chief technical officer (principal) of a company tries to seek the best solution for an annual research project. 
%She does not have enough skill (or time) to explore the task by herself, thus delegates the task to multiple researchers (agents) at a research division in the company.
%The officer requires each division to submit a candidate solution for the project, and she selects the final solution after aggregating and evaluating the submitted candidates.
%The officer is interested in the optimal solution which will bring the highest revenue to the company. However, each researcher tries to seek a solution that is more interesting for his own sake or a solution that may be accepted by a famous venue with high probability.
%As a result, a natural question arises, how should the principal design a delegation mechanism in order to extract more utilities from the self-interested agents?

Initiated by \citet{holmstrom1980theory}, there exists a rich line of literature studying the theory of \emph{delegation without monetary transfer}.
The restriction that the principal cannot commit to a contingent monetary transfer in the mechanism imparts a restrictive structure on feasible mechanisms in which the mechanism simply commits to a set of acceptable solutions, and only decide whether or not to accept the proposed solutions.
\citet{holmstrom1980theory} study the optimality of these simple mechanisms and the characterizations of the regimes for these mechanisms to be optimal.
% have long been studied in the literature on the theory of delegation.
Subsequent works including \citet{alonso2008optimal} and \citet{armstrong2010model} develop the theory of delegation in this context and broaden its scope in fruitful direction.

Recently, with a lens of computer science, \citet{kleinberg2018delegated}  study a problem of designing approximate mechanisms in the \emph{delegated search} problem.\footnote{They study two types of model, one of which is similar to delegated choice without search cost by \cite{armstrong2010model}, and the other is that with search (sampling) cost. Our model can be framed as either of a delegated search problem with exogenous solutions, or delegated choice problem which delegates the choice between given alternatives.}
They consider a simple mechanism so-called a {\em single-proposal} mechanism, which consists of single-round interaction between the principal and the agent.
Remarkably, it achieves a $2$-approximation compared to an ideal scenario in which the principal can directly select the best solution among the entire set of agents' solutions.
Their analysis is based on a novel observation regarding a connection between the dynamics of the single-proposal mechanism and the dynamics of threshold-based algorithms in \emph{prophet inequalities} (see \citet{samuel1984comparison},
\citet{krengel1987prophet},
\citet{hajiaghayi2007automated},
\citet{alaei2012online}, \citet{abolhassani2017beating}, \citet{correa2017posted} for more reference to prophet inequalities).

As we discussed in the above example, there exists a variety of real-world situations, spanning economical applications to modern intelligent systems, such that the principal needs to delegate the task to multiple agents with misaligned payoff.
Surprisingly, however, the problem of delegating to \emph{multiple}  agents in the framework of mechanism design without money has received less attention in the community.
The recent work by \citet{gan2022optimal}, preceded by \citet{alonso2014resource}, study the optimal delegation mechanism with two agents in the context of mechanism design without money, but their model is significantly different from ours, and also is restricted to small number of agents with specific utility functions.\footnote{We provide the detailed discussion in Section~\ref{sec:related_work}.}

In this context, we introduce the \emph{multi-agent delegation} problem, and conduct a comprehensive study on the approximation factors of various mechanisms without monetary transfer.
Technically, we aim to design a multi-agent delegation mechanism that improves upon the guarantees of a single-agent mechanism by \citet{kleinberg2018delegated}.
Surprisingly, different from the single-agent mechanism which assumes the prior knowledge on the agent's distribution to derive a constant approximation factor, \ie \Emph{Bayesian mechanism} (BM), we show that we can construct an efficient mechanism even without those prior knowledge, \ie by \Emph{prior-independent mechanism} (PIM), which is mainly due to the competitive tension arise from the multi-agent extension.
Notably, however, we further observe that the amount of such a compelling power from competition differs with respect to the information available to the agents, and the degree of correlation between the principal's and the agent's utility.
Overall, we comprehensively analyze the approximation factors of BM and PIM in both the \Emph{complete} and \Emph{incomplete information} settings (in terms of the agents' information).
We note that our main technical results lie on the \emph{analysis of approximation factors of PIM}.
To highlight a few of the main results,
\vspace{-0.3mm}
\begin{enumerate}
    \item In the complete information setting, we show that there exists a PIM such that the principal's expected utility is bounded below by the \emph{first-best solution} (in the principal's view) of the \emph{second-best agent}. We further quantify this approximation factor by analyzing the upper and lower bound of the principal's expected utility in various regimes. This tends to asymptotically optimal in certain regimes, \ie the gains from multi-agent delegation is significant. En route to this analysis, we present several technical results regarding the order statistics of i.i.d. random variables, which might be of independent interest.
    \item In the incomplete information setting, we show that under symmetric agents with uniform distribution $U[0,1]$ and the assumption of independent utility, we can construct a PIM in which there exists a $(1-e^{-n^2/2(n-1)^2})$-approximate \emph{Bayes Nash equilibrium} such that the principal's expected utility becomes exactly optimal, where $1-e^{-n^2/2(n-1)^2}$ converges to $1-\nicefrac{1}{\sqrt{e}} \cong 0.3935$ as the number of agents $n$ increases.
    We numerically verify that this guarantee is almost tight. Using a similar technique, we analyze that there exists a \emph{Bayes correlated equilibrium} with a multiplicative approximation factor of $e^{n^2/2(n-1)^2} \cong \sqrt{e}$.
    \item We further show that the assumptions of symmetric agents and independent utility are necessary. More formally, without these assumptions, we can construct a problem instance such that there exists a \emph{Bayesian Nash equilibrium} in which the agents propose their worst solutions for the principal, which may induce arbitrarily bad principal's utility.
\end{enumerate}
\vspace{-0.3mm}
To select the best solution among the solutions from multiple agents, however, the principal suffers a cost of \emph{examining the candidates}.
In this context, we extend our problem setup and further study a trade-off between such an examination cost and an efficiency of mechanisms, and provide an analogous result in the complete information setting.

% \sscomment{To summarize the main \emph{takeaway} of our results, we mainly show that the prior independent mechanism can be made efficient, which was not the case in the single-agent setting. This is due to the fact that the competition partly enforces each agent to behave more in favor of the principal. .}

The remainder of the paper is organized as follows.
In Section~\ref{sec:overview}, we summarize overall results and the techniques therein.
Section~\ref{sec:related_work} provides detailed discussions on the related work.
Section \ref{sec:setup} introduces the formal problem setup.
In Section \ref{section:no_cost} and \ref{section:no_cost_incomp}, we provide the results in the complete and incomplete information setting, respectively.
Finally in Section \ref{sec:cost}, we introduce the examination cost and some results in this extension.


% In this paper, we study approximation mechanisms in the delegated search problem with multiple agents.
% Since the multi-agent extension naturally imposes an additional burden for the principal to evaluate the solutions from multiple agents, which we refer to as an examination cost, we study the trade-off between the principal's burden to examine multiple solutions and the efficiency of the mechanism.
% Firstly, we investigate whether the multi-agent extension indeed brings an advantage over the single-agent delegated search.
% To this end, we define a reasonable method to compare the multi-agent and the single-agent setting, and reveal that for any mechanism $M$ in the single-agent setting, there exists a certain type of mechanism in the multi-agent setting that is superior to $M$ in the single-agent setting.
% More specifically, we consider a simple class of mechanism defined as a randomized single-proposal mechanism and prove its superiority over any mechanism in the single-agent setting.
% We next study the delegation gap of the randomized single-proposal mechanism and parameterize it with respect to the examination cost of the mechanism.
% We further improve this delegation gap by more involved variants of the randomized single-proposal mechanism.
% The results above are derived in the complete information setting, and we present analogous results for the incomplete information setting.


% \note{Finally, highlight that this work belongs to the line of mechanism design without money, and refer several papers on it.}

% \todo{We do some comprehensive studies...}





==> Delegating to Multiple Agents (1)/mechanism_example.tex <==
\section{Further discussion on feasible mechanisms}\label{sec:fur_fea_mec}
Another reasonable choice of mechanism will be to require each agent submitting certain number, say two, of solutions, \ie multi-proposal mechanism.
    Under this mechanism, each agent might select a pair of aggressive solution with large ex-post utility but smaller chance to be selected, and conservative solution with small ex-post utility but larger probability of winning, in order to balance these features of two solutions.
    More abstractly, one may consider a mechanism that requires each agent to signal some statistics of the observed solutions, \eg sample average or the number of eligible solutions, upon the solutions themselves.
    As astute readers may have noticed, in the complete information setting, however, the revelation principle style of result allows us to reduce any mechanism to single-proposal mechanism, so such generalization does not help. This is formalized in Theorem~\ref{thm:multiagent_revel}.
    Note that this reduction does not preclude any randomized mechanism.

==> Delegating to Multiple Agents (1)/mymath.tex <==

%\newtheorem{example}{Example}
% \newtheorem{theorem}{\bf Theorem}
% \newtheorem{definition}{\bf Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{\bf Corollary}
% \newtheorem{proposition}{\bf Proposition}
% \newtheorem{claim}{\bf Claim}
% \newtheorem{observation}{\bf Observation}
% \newtheorem{question}{\bf \color{red} Question}
% \newtheorem{remark}{Remark}
% \newtheorem{fact}{Fact}
% \newtheorem{assumption}{Assummption}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{reduction}[theorem]{Reduction}
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{extension}[theorem]{Extension}
\newtheorem{assumption}[theorem]{Assumption}

\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim*}{Claim}

\theoremstyle{definition}
\newtheorem*{definition*}{Definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{discussion}[theorem]{Discussion}
\newtheorem*{remark*}{Remark}
\newtheorem*{property*}{Property}
\newtheorem{exercise}{Exercise}[section]
\newtheorem*{problem*}{Problem formulation}


\newcommand{\Emph}[1]{\textbf{#1}}



%%%%%%%%%%%% real, integer notation
\newcommand{\real}{{\mathbb R}}
\newcommand{\integer}{{\mathbb Z}}
\newcommand{\paranth}[1]{{\left(#1 \right)}}
\newcommand{\parans}[1]{{\left(#1 \right)}}
\newcommand{\paranm}[1]{{\left\{#1 \right\}}}
\newcommand{\paranl}[1]{{\left[#1 \right]}}


% boldface characters
% macro by mung

\newcommand{\td}{\ensuremath{t_{\text{dl}}}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bbx}{\ensuremath{{\bm x}}}
\newcommand{\bbc}{\ensuremath{{\bm c}}}
\newcommand{\bu}{\ensuremath{{\bm u}}}

\newcommand{\bz}{\ensuremath{{\bm z}}}
\newcommand{\ba}{\ensuremath{{\bm a}}}
\newcommand{\be}{\ensuremath{{\bm e}}}
\newcommand{\br}{\ensuremath{{\bm r}}}
\newcommand{\by}{\ensuremath{{\bm y}}}
\newcommand{\bby}{\ensuremath{{\bm y}}}
\newcommand{\bbq}{\ensuremath{{\bm q}}}


\newcommand{\bp}{\ensuremath{{\bm p}}}
\newcommand{\bh}{\ensuremath{{\bm h}}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bA}{\ensuremath{{\bm A}}}

\newcommand{\bF}{\bm{F}}
\newcommand{\bN}{\ensuremath{{\bm N}}}
\newcommand{\bbf}{\ensuremath{{\bm f}}}
\newcommand{\bG}{\ensuremath{{\bm G}}}
\newcommand{\bQ}{\ensuremath{{\bm Q}}}
\newcommand{\bH}{\ensuremath{{\bm H}}}
\newcommand{\bW}{\ensuremath{{\bm W}}}
\newcommand{\bJ}{\ensuremath{{\bm J}}}
\newcommand{\bg}{\ensuremath{{\bm g}}}
\newcommand{\bs}{\ensuremath{{\bm s}}}

\newcommand{\bbv}{\ensuremath{{\bm v}}}
\newcommand{\bbz}{\ensuremath{{\bm z}}}
\newcommand{\bbu}{\ensuremath{{\bm u}}}
\newcommand{\bbm}{\ensuremath{{\bm m}}}
\newcommand{\bbU}{\ensuremath{{\bm U}}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bbr}{\ensuremath{{\bm r}}}
\newcommand{\bbalpha}{\ensuremath{{\bm \alpha}}}
\newcommand{\brho}{\ensuremath{{\bm \rho}}}


% \newcommand{\bblambda}{\mbox{\boldmath \ensuremath{\lambda}}}
% \newcommand{\blambda}{\mbox{\boldmath \ensuremath{\lambda}}}

% \newcommand{\bmu}{\mbox{\boldmath \ensuremath{\mu}}}
% %\newcommand{\bmu}{\mu}

% \newcommand{\bbeta}{\mbox{\boldmath \ensuremath{\beta}}}
% \newcommand{\btheta}{\mbox{\boldmath \ensuremath{\theta}}}
% \newcommand{\bv}{\ensuremath{{\mathbf v}}}
% %\newcommand{\reals}{\ensuremath{\mathbf{R}}}
\newcommand{\bR}{\bm{R}}
% \newcommand{\bw}{\ensuremath{{\mathbf w}}}
% % \newcommand{\bF}{F}


%%%%%%%%%%%% Sets, calligraphic characters...
\newcommand{\cR}{\ensuremath{\mathcal R}}
\newcommand{\set}[1]{\ensuremath{\mathcal #1}}
\renewcommand{\vec}[1]{\bm{#1}}
\newcommand{\mat}[1]{\bm{#1}}

\newcommand{\node}[1]{\ensuremath{{\tt #1}}}
\newcommand{\nn}[1]{\node{#1}}

\newcommand{\mytitle}[1]{\medskip \noindent{\em #1} \smallskip}
\newcommand{\mytitlehead}[1]{\noindent{\em #1} \smallskip}
\newcommand{\rnote}[1]{{\color{red}#1}} 

\newcommand{\separator}{
  \begin{center}
    \rule{\columnwidth}{0.3mm}
  \end{center}
}
\newenvironment{separation}{ \vspace{-0.3cm}  \separator  \vspace{-0.2cm}}
{  \vspace{-0.4cm}  \separator  \vspace{-0.1cm}}

%%%%%%%%%%%%%%%% other macros %%%%%%%%%%%%%%%%%%
\def\un{\underline}
\def\ov{\overline}
\def\Bl{\Bigl}
\def\Br{\Bigr}
% \def\bl{\bigl}
% \def\br{\bigr}
\def\lf{\left}
\def\ri{\right}
\def\st{\star}

% \def\eg{{\it e.g.}}
% \def\ie{{\it i.e.}}

%\newcommand{\eqdef}{{\triangleq}}

% \newcommand{\bi}{\begin{itemize}}
% \newcommand{\ei}{\end{itemize}}


\newcommand{\bbprob}[1]{\mathbb{P}\lf[ #1 \ri]}
\newcommand{\bprob}[1]{\mathbb{P}\Bl[ #1 \Br]}
\newcommand{\prob}[1]{\mathbb{P}[ #1 ]}
\newcommand{\expect}[1]{\mathbb{E}[ #1 ]}
\newcommand{\bexpect}[1]{\mathbb{E}\Bl[ #1 \Br]}
\newcommand{\bbexpect}[1]{\mathbb{E}\lf[ #1 \ri]}
\newcommand{\vari}[1]{\text{VAR}[ #1 ]}
\newcommand{\bvari}[1]{\text{VAR}\Bl[ #1 \Br]}
% \newcommand\given[1][]{\:#1\vert\:}


\newcommand{\exming}{\ensuremath{\text{ExMin}_g} }
\newcommand{\imp}{\Longrightarrow}
\newcommand{\beq}{\begin{eqnarray*}}
\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\bemn}{\begin{multiline}}
\newcommand{\eemn}{\end{multiline}}

\newcommand{\sqeq}{\addtolength{\thinmuskip}{-4mu}
\addtolength{\medmuskip}{-4mu}\addtolength{\thickmuskip}{-4mu}}

\newcommand{\unsqeq}{\addtolength{\thinmuskip}{+4mu}
\addtolength{\medmuskip}{+4mu}\addtolength{\thickmuskip}{+4mu}}

% floor function
\newcommand{\lfl}{{\lfloor}}
\newcommand{\rfl}{{\rfloor}}
\newcommand{\floor}[1]{{\lfloor #1 \rfloor}}

\newcommand{\grad}[1]{\nabla #1}

% \newcommand{\sqeq}{\addtolength{\thinmuskip}{-4mu}
%   \addtolength{\medmuskip}{-4mu}\addtolength{\thickmuskip}{-4mu}}
% \newcommand{\unsqeq}{\addtolength{\thinmuskip}{+4mu}
%   \addtolength{\medmuskip}{+4mu}\addtolength{\thickmuskip}{+4mu}}

% \newcommand{\bea}{\begin{eqnarray}}
%   \newcommand{\eea}{\end{eqnarray}}
% \newcommand{\beas}{\begin{eqnarray*}}
%   \newcommand{\eeas}{\end{eqnarray*}}
% \newcommand{\bd}{\begin{displaymath}}
%   \newcommand{\ed}{\end{displaymath}}
% \newcommand{\be}{\begin{equation}}
%   \newcommand{\ee}{\end{equation}}
% \newcommand{\vs}{\vspace{0.2in}}
% \newcommand{\hs}{\hspace{0.5in}}
% \newcommand{\el}{\end{flushleft}}
% \newcommand{\bl}{\begin{flushleft}}
% \newcommand{\bc}{\begin{center}}
% \newcommand{\ec}{\end{center}}
% \newcommand{\remove}[1]{}


% \newtheorem{assum}{Assumption}
% % \newtheorem{example}{Example}
% \newtheorem{property}{Property}
% \newtheorem{remark}{Remark}

% \newcommand{\separator}{
%   \begin{center}
%     \rule{\columnwidth}{0.3mm}
%   \end{center}
% }

% \newenvironment{separation}
% { \vspace{-0.3cm}
%   \separator
%   \vspace{-0.25cm}
% }
% {
%   \vspace{-0.5cm}
%   \separator
%   \vspace{-0.15cm}
% }

% \renewcommand{\baselinestretch}{0.98}

\def\A{\mathcal A}
\def\oA{\overline{\mathcal A}}
\def\S{\mathcal S}
\def\D{\mathcal D}
\def\eff{{\rm Eff}}

\def\cU{{\cal U}}
\def\cM{{\cal M}}
\def\cV{{\cal V}}
\def\cA{{\cal A}}
\def\cX{{\cal X}}
\def\cN{{\cal N}}
\def\cJ{{\cal J}}
\def\cK{{\cal K}}
\def\cL{{\cal L}}
\def\cI{{\cal I}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}
\def\cC{{\cal C}}
\def\cR{{\cal R}}
\def\id{{\rm Id}}
\def\st{{\rm st}}
\def\cF{{\cal F}}
\def\cG{{\mathcal G}}
\def\N{\mathbb{N}}
\def\R{\mathbb{R}}
\def\cB{{\cal B}}
\def\cP{{\cal P}}
\def\cS{{\cal S}}
%\def\and{\quad\mbox{and}\quad}
\def\ind{{\bf 1}}

\def\bmg{{\bm{\gamma}}}
\def\bmr{{\bm{\rho}}}
\def\bmq{{\bm{q}}}
\def\bmt{{\bm{\tau}}}
\def\bmn{{\bm{n}}}
\def\bmcapn{{\bm{N}}}
\def\bmrho{{\bm{\rho}}}

\def\igam{\underline{\gamma}(\lambda)}
\def\sgam{\overline{\gamma}(\lambda)}


\def\PP{{\mathrm P}}
\def\EE{{\mathrm E}}
\def\iskip{{\vskip -0.4cm}}
\def\siskip{{\vskip -0.2cm}}

\def\bp{\noindent{\it Proof.}\ }
\def\ep{\hfill $\Box$}


% \newcommand{\set}[1]{\mathcal{#1}}





==> Delegating to Multiple Agents (1)/no_cost.tex <==
% !TEX root =  main.tex
\section{Analysis of the multi-agent single-proposal mechanism}\label{section:no_cost}
In this section, we provide a performance guarantee of MSPM.
Note that for the multi-agent delegation problem, it suffices to find a good mechanism over the space of MSPMs, thanks to Theorem~\ref{thm:multiagent_revel}.
We first present the analysis of delegation gap of MSPM, and then present a comparison between the performance of MSPM in the multi-agent setting and the performance of any mechanism in the single-agent setting.

\subsection{Delegation Gap}
We first prove a generic result regarding an arbitrary threshold-based eligible set and further quantify the corresponding delegation gap for some good choices of the parameters of MSPM.

%We mainly argue that a large examination budget gives us a significant amount of gain in terms of principal's utility.

% To elaborate, we first present how the single-proposal mechanism behaves under the single-agent setting in terms of $X_{i,j}$ and $Y_{i,j}$, which will be useful in comparing the results.
% Generally, the threshold $\tau$ is set to be half of the expectation of $X_{\max} =  \max_{j \in [k]} X_{1,j}$ so that $\tau = 1/2\Ex{X_{\max}}$.
% Then, by the dynamics of the single-proposal mechanism, solution with highest $Y_j$ satisfying $X_{j} \ge \tau$ will be selected.
% Define $\set{E} = \{\om \in \omb : x(\om) \ge \tau \}$, i.e. the subset of solutions contained in the eligible set.

% We use $\mec_{SP}$ to denote the expected utility of single-proposal mechanism.
% More, formally,
% \begin{align*}
% \mec_{SP}  = \Ex{TBD}
% \end{align*}

\begin{theorem} \label{theorem:multi-agent-unlimited-budget}
Given any $\tau \ge 0$, let $R$ be an eligible set with threshold $\tau$ such that $R:= \{\omega: x(\omega) \ge \tau, \omega \in \Omega\}$, and $\rho$ be an arbitrary deterministic tie-breaking rule with transitivity.
In the multi-agent setting, MSPM with $\rho$ and a homogeneous eligible set $R$ has a delegation gap of at most
\begin{align*}
\Ex{X_{(1)}} - \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} - 
\Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.
\end{align*}
\end{theorem}
\begin{proof}[Proof]
We mainly prove that the payoff of randomized single-proposal mechanism $M$ is at least $$\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.$$
% We denote by $c_i$ the agent $i$'s proposed candidate. Since there is an unlimited budget for examination, we can assume that the principal examines all candidates and takes the best candidate which maximizes her utility, i.e. winner is $c_{i^*}$ where $i^* = \argmax_{i} x(c_i)$.

We find a lower bound on the principal's utility in an arbitrary Nash equilibrium. 
%We consider two cases based on whether there exist eligible solutions or not.
Let $\omb = \cup_{i \in [n]}\omb_i$ be the entire set of solutions observed by the agents and $\sigma = (\sigma_1,\ldots, \sigma_n)$ be the equilibrium strategies.
We separately consider two cases (i) for any $\om \in \omb$, $\om \notin R$ and (ii) there exists $\om \in \omb$ such that $\om \in R$.

{\em Case (i).} 
In this case, the utility of all agents is $0$,
and there does not exist a winner. 
Recall that for any Nash equilibrium,
there exists no incentive for any agent to deviate from equilibrium strategies.
%We denote the agent with rank $1$ by $t$. 
%<<<<<<< Updated upstream
%We show that in this case $X_{(1)} < \tau$.
%Suppose not, i.e. $X_{(1)} \geq \tau$. 
%Denote by $\om^*$ the candidate which corresponds to the utility of $X_{(1)}$.
%If agent $t$ proposes $\om^*$, his utility strictly increases from $0$ to $y(\om^*)$, which contradicts that the agents have played equilbirium strategies.
%=======
We claim that $X_{(1)} < \tau$, where it concludes that the principal's utility is simply zero in this case.
Suppose not, i.e. $X_{(1)} \geq \tau$. 
Denote by $\om^*$ the candidate which corresponds to the utility of $X_{(1)}$.
If agent $t$ plays $\om^*$, his utility strictly increases from $0$ to $y(\om^*)$, which contradicts that the agents have played equilibrium strategies.
%>>>>>>> Stashed changes
Hence we conclude that $X_{(1)} < \tau$, and the principal's utility is $0$.

{\em Case (ii).} 
Suppose that the winner is the candidate proposed by agent $i^*$. 
In this case, all agents except agent $i^*$ have a utility of $0$. 
Like the previous case, there is no incentive for agents to change their strategies. 
%<<<<<<< Updated upstream
%Consider agent $i \neq i^*$,
%there is no incentive for the agent to propose his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$. 
%This implies that even if agent $i$ proposes that solution, he still gets a utility of $0$. 
%\suho{I understand these sentences, but it would be more formal if we can mathematically represent them, not by english. For example in the above sentence, we can say that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y(\sigma_i) = 0$. I think the reason that Mohammad commented on our previous version to be less formal is that it argues too much with words.}
%As a result, if he proposes his best-observed solution, that solution is not selected as the winner, which shows that the current winner gives a higher utility to the principal, i.e. $x(c^*) \geq X_{i, (1)}$. 
%\suho{same as above}
%=======
Consider agent $i \neq i^*$, there is no incentive for the agent to propose his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$. 
This implies that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y_i(\sigma_i) = 0$.
%\suho{I understand these sentences, but it would be more formal if we can mathematically represent them, not by english. For example in the above sentence, we can say that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y(\sigma_i) = 0$. I think the reason that Mohammad commented on our previous version to be less formal is that it argues too much with words.}
Since the agents are playing equilibrium strategies $\sigma$, the winner should not be changed with respect to agent $i$'s strategy.
This implies that $x(\sigma_{i^*}) \geq X_{i, (1)}$ for any $i \neq i^*$.
%
%As a result, if he proposes his best-observed solution, that solution is not selected as the winner, which shows that the current winner gives a higher utility to the principal, i.e. $x(c^*) \geq X_{i, (1)}$. 
%\suho{same as above}
%>>>>>>> Stashed changes
Furthermore, we have $x(\sigma_{i^*}) \leq X_{i^*, (1)}$. Since for $n-1$ agents $i$ ($i \neq i^*$) we have $X_{i, (1)} \leq x(\sigma_{i^*})$, and $x(\sigma_{i^*}) \leq X_{i^*, (1)}$ using the definition of $X_{(r)}$ we get
$$
X_{(n)} \leq X_{(n-1)} \leq ... \leq X_{(2)} \leq x(\sigma_{i^*}) \leq X_{(1)}.
$$
Also, in this case, we assume that $\sigma_{i^*}$ is eligible which further implies that $\tau \leq x(\sigma_{i^*}) \leq X_{(1)}$. So we get $\max\left(X_{(2)}, \tau\right) \leq x(\sigma_{i^*}) \leq X_{(1)}$. This inequality shows that
\begin{itemize}
    \item if $X_{(2)} \geq \tau$ then $x(\sigma_{i^*}) \geq X_{(2)}$.
    \item if $X_{(1)} \geq \tau \geq X_{(2)}$ then $x(\sigma_{i^*}) \geq \tau$.
\end{itemize}

Therefore, by combining the results of the case (i), and case (ii) the expected utility of the principal is at least
\begin{align}
	\Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
	\Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.\label{ineq:infbud_tau}
\end{align}


% The proof mainly follows from the following lemma.


% \begin{lemma}
% In multi-agent setting with unlimited budget, the payoff of randomized single-proposal mechanism $M$ is at least $\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}$.
% \begin{proof}[Proof Sketch of Lemma]
% Since there is an unlimited budget for examination, we can assume that the principal takes the best candidate with respect to her own utility.
% There are two cases here:
% \begin{itemize}
%     \item If the best candidate does not satisfy the principal requirements, i.e. none of the proposed candidates are in eligible set $T_\tau$, i.e. $X_{\max} < \tau$; then the principal utility will be $0$.
%     \item If there is at least one candidate which satisfies the principal requirements; then we have $f_{M, \sigma}(\omb) = \argmax_i x(\sigma_i(\om_i))$. If $i^*$ is the agent who owns the winner, then all other agents have a utility of $0$. Consider a Nash equilibrium case where the utility of agents does not increase if they change their candidates (i.e. $\sigma_i(\om_i)$). Since the utility of all agents except agent $i^*$ is $0$, it implies that other agents do not have any strategies to get a positive utility. Since we are considering a Nash equilibrium, if agent $i \left(i \neq i^*\right)$ proposes his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$, then he still gets utility of $0$, which implies that the winner selected by the principal has utility at least $\max_{i \neq i^*} X_{i, (1)}$.
% Therefore, we can conclude that $i^*$ is the agent whose rank is $1$, thus what he proposes should give the principal higher utility than the best proposal of other agents:
% $$
% x(\sigma_{i^*}(\om_{i^*})) \geq X_{(2)} \geq X_{(3)} \geq ... \geq X_{(n)}.
% $$
% Also, if $X_{(2)} < \tau$ then we can have a better bound on the winner since $\sigma_{i^*}(\om_{i^*})$ is eligible then $x(\sigma_{i^*}(\om_{i^*}) \geq \tau$ thus in this case we have:
% $$
% x(\sigma_{i^*}(\om_{i^*})) \geq \tau > X_{(2)} \geq X_{(3)} \geq ... \geq X_{(n)}.
% $$
% \end{itemize}

% Therefore, we can conclude that the utility is bounded by 
% $$
% \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
% \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}
% $$
% \end{proof}
% \end{lemma}
\end{proof}
The main intuition behind this advantage is that the existence of opponents, whose proposed solutions are examined by the principal, makes agents more competitive in sending signals, thus resulting in submitting more qualified solutions to be selected.


A direct corollary of this result is that we can derive the following upper bound on the delegation gap even without the eligible set.
\begin{corollary}\label{cor:infbud_notau}
MSPM with no eligible set and a deterministic tie-breaking rule with transitivity has a delegation gap of at most
\begin{align}
	\Ex{X_{(1)}} - \Ex{X_{(2)}}\label{ineq:infbud_notau}
\end{align}
\end{corollary}
This implies that even without the eligible set, the multi-agent setting brings some advantages for the principal, which is mainly due to the competitive tension arising between the agents.


We highlight that the theorem only holds for the \emph{deterministic} tie-breaking rule.
The intuition behind it is that if the principal exploits a randomized tie-breaking rule, it may reduce the power of competition in certain cases since the agents may settle with a bad solution in terms of the principal, as it still gives the agents some utility due to the randomized tie-breaking rule and another solution which is more preferred to the principal might yield a low utility for the agents.
However for the deterministic tie-breaking rule, as the principal naturally prefers some agents, the other agents tend to be more competitive in order to be selected by the principal, and this recursively makes those preferred agents to behave more in favor of the principal.
More formally, in the following theorem, we prove that random tie-breaking rule can be arbitrarily bad for some problem instances.
\begin{theorem}
    Consider a MSPM with eligible sets $(R_i)_{i \in [n]}$ and a random tie-breaking rule.
    Then, for any $\eps > 0$, there exists a problem instance such that the mechanism have a bad equilibria in which the delegation gap is at least $1/\eps$.
\end{theorem}
\begin{proof}
\todo{prove it.}
\end{proof}


\todo{Recovering single-agent guarantees.}
% \begin{example}
% Given a solution space $\Omega = \{a,b,c\}$, consider $n=4$ agents with the same utility function $y(a) = 100$, $y(b) = 10$ and $y(c) = 1$ and a principal with utility function $x(a) = 1$, $x(b) = 10$ and $x(c) = 100$.
% Each agent samples two solutions.
% Agents $1,2$ sample $a$ or $c$ with equal probability, and agents $4,5$ sample $b$ or $c$ with equal probability.
% Consider a RSPM with a random tie-breaking rule, eligible sets $R_i$ for $i \in [n]$ and unlimited budget.
% Suppose that the agents' solutions are realized to be $\{a,c\}$,$\{a,c\}$,$\{b,c\}$ and $\{b,c\}$.
% \end{example}




%\note{I couldn't find a good description for Theorem 3.3}
\subsection{Comparing multi-agent and single-agent delegation}
% Furthermore, we find a lower-bound on the expected utility of the principal using RSPM. In Theorem \ref{theorem:multi-agent-unlimited-budget}, we formulate the principal's utiltiy when there is an unlimited examination budget, i.e. principal can examine all candidates. Then in Theorem \ref{theorem:multi-agent-limited-budget}, we consider the case that examination budget is limited, and we find a lower-bound on principal's utilty regarding the examination budget.

%We further ask whether there exists any improvement in the delegation gap in the multi-agent setting compared to single-agent setting despite using of the same mechanism.
%We will elaborate more later on how we compare the multi-agent and the single-agent setting.
%Surprisingly, we find that the delegation gap in multi-agent setting can significantly decrease compared to that of single-agent setting.
%This is mainly due to the competition between agents, which was not there in single-agent setting in which any mechanism with an arbitrary budget can be simply reduced to single-proposal mechanism with unit examination budget.

In this section, we show that the multi-agent delegation indeed brings advantages over the single-agent delegation. we compare the principal's utility when delegating to multiple agents with a situation where a single agent is in charge of finding the solutions. 
We observe that delegating to multiple agents indeed has advantages in terms of the principal's utility.
To this end, we first define a reasonable way to compare the principal's utility in the multi-agent setting with that in the single-agent setting.
%Given a single-agent problem, we present two benchmarks in multi-agent problem as follows.
\begin{definition}[Multi-agent correspondence]
Consider a single-agent problem with a distribution $D$, a number of solutions $k$, the agent's utility function $y$, and the principal's utility function $x$.
Consider a multi-agent problem with $n \ge 2$ agents in which the principal has the same utility function $x$ and each agent $i$ has a distribution $D_i = D$, a number of solutions $k_i$ such that $\sum_{i=1}^nk_i = k$, and the utility function $y_i = y$. We denote this multi-agent problem a \emph{weak} $n$-agent correspondence of the single-agent problem.
%\begin{enumerate}
%	\item there exists an agent $i$ with parameters $k_i = k$, $D_i =D$, and $y_i = y$. We denote this multi-agent problem a \emph{strong} $n$-agent correspondence of the single-agent problem.
%	\item each agent $i$ has a distribution $D_i = D$, a number of solutions $k_i$ such that $\sum_{i=1}^nk_i = k$, and the utility function $y_i = y$. We denote this multi-agent problem a \emph{weak} $n$-agent correspondence of the single-agent problem.
%\end{enumerate}
\end{definition}
%The strong $n$-agent correspondence refers to a strong version of benchmark in which the agent in the single-agent problem becomes one of the agents in the multi-agent problem.
%Intuitively, we expect this strong benchmark to be have better outcome in terms of the principal's utility, since the principal delegates to a strictly better pool of agents.
To see whether delegating to the multi-agent indeed brings advantages, it is fair to compare under the assumption that the agents exert the same total amount of effort in the task in both the single-agent and the multi-agent problem.
Since the number of solutions can be translated as the amount of effort exerted in the task, our definition of the multi-agent correspondence would play a reasonable role in comparing the single-agent and the multi-agent problem.

\begin{theorem}\label{theorem:multi-agent-correspondence}
Given a single-agent problem $P$, denote its multi-agent correspondence $P'$.
For any mechanism $M$ under $P$, there exists a MSPM under $P'$ such that the principal's utility of the MSPM under $P'$ is at least that of  $M$ under $P$.
\end{theorem}
%However in some sense, to see whether delegating to multi-agent indeed brings advantages, it is fair to compare under the assumption that the agents exert the same total amount of effort in the task in both the single-agent and multi-agent problem.
%We first present a result on the strong benchmark.
%\begin{theorem}
%Given a single-agent problem $P$, denote its strong $n$-agent correspondence $P'$.
%For any SPM with an eligible set in $P$, there exists a unit-budget RSPM with a homogeneous eligible set in $P'$ such that the principal's expected utility of the RSPM under any Nash equilibrium in $P'$ is at least that of the $SPM$ in $P$.	
%\end{theorem}
%\begin{theorem}
%Given a single-agent problem $P$, denote its weak $n$-agent correspondence $P'$.
%For any SPM with an eligible set in $P$, there exists a RSPM with a homogeneous eligible set and budget $B=n$ in $P'$ such that the principal's expected utility of the RSPM under any Nash equilibrium in $P'$ is at least that of the $SPM$ in $P$.
%\end{theorem}
\begin{proof}
We start by presenting the following lemma from~\cite{kleinberg2018delegated}.
\begin{lemma}[\cite{kleinberg2018delegated}]\label{thm:singleagent_revel}
In the single-agent setting, for any mechanism $M$ and corresponding dominant strategies $\sigma$, there exists a MSPM such that for any equilibrium strategies $\sigma'$, we have $x(f_{M,\sigma}(\omb)) = x(f_{SPM,\sigma'}(\omb))$ for any $\omb \in \Omega^*$.
\end{lemma}
% This corresponds to a celebrated revelation principal~(cite) in mechanism design literature.
% It is important to note that any SPM requires an examination budget of $1$, since it only evaluates a single candidate from a single agent.
% This implies that there is no merit in having a large examination budget against single-agent.
% This is fairly intuitive because, in a single-agent setting, the agent does not have any incentive to signal more than two candidates since he knows that only one of them would be eventually selected.
By the lemma, it suffices to consider the case when $M$ is a SPM.
Let the realized solutions in $P$ be $\omb = \{\om_1, \om_2,\ldots, \ldots \om_k\}$. Consider a partition of $\omb$ as follows
\begin{align*}
	\omb_{1} &= \{\om_1,\ldots, \om_{k_1}\}
	\\
	\omb_{2} &= \{\om_{k_1+1},\ldots, \om_{k_1+k_2}\}
	\\
	&\vdots
	\\
	\omb_{n} &= \{\om_{k_1+\ldots+k_{n-1}+1},\ldots, \om_{k_1+\ldots + k_n=k}\}.
\end{align*}
Suppose that agent $i$'s realization of solutions in $P'$ is $\omb_{i}$ so that the outcomes of $P$ and $P'$ are coupled. 
This coupling is indeed possible because the probability that agent $i$'s solutions are realized to be $\omb_i = \{\om_{i_1},\ldots, \om_{i_{k_i}}\}$ is exactly equal to the marginal probability that $\om$'s $i$-th partition is realized to be $\omb_i = \{\om_{i_1},\ldots, \om_{i_{k_i}}\}$.
Consider a SPM with an eligible set $R$ under $P$, and corresponding equilibrium strategies $\sigma$.
Denote by $x$ and $y$ the principal and the agent's utility function under $P$ respectively.
Given the solutions realized as above, SPM will select the solution which maximizes $y(\om_j)$ for $j \in [k]$ such that $\om_j \in R$, i.e. $\om_1^* = \argmax_{j \in [n], \om_j \in R} y(\om_j)$.
Let this solution be $\om_1^*$.
Now consider a MSPM with arbitrary tie-breaking rule and the same eligible set $R$ under $P'$, and suppose that the agents play equilibrium strategies $\sigma'$.
Let $\om_2^*$ be the corresponding winner in this case.
% Let $A$ be a set of solutions that can be selected as a winner in the MSPM under $P'$.
% Note that $A$ might include multiple solutions since the examination process is randomized in RSPM.
% For any $\om_2^* \in A$, 
We want to show that $x(\om_2^*) \ge x(\om_1^*)$  for any realization of solutions $\omb$.
Suppose not.
It is obvious that both $x(\om_1^*)$ and $x(\om_2^*)$ belong to the eligible set $R$.
If $\om_1^*$ and $\om_2^*$ belongs to the same partition $\omb_i$, it means that agent $i$ has both the solutions $\om_1^*$ and $\om_2^*$.
By our definition on $\om_1^*$ such that $\om_1^* = \argmax_{j \in [n], \om_j \in R} y(\om_j)$, submitting $\om_1^*$ is gives the better or the same utility for agent $i$.
If $y(\om_1^*) > y(\om_2^*)$, then simply submitting $\om_1^*$ gives a strictly better utility for agent $i$, and it contradicts that $\sigma'$ is equilibrium strategy.
If $y(\om_1^*) = y(\om_2^*)$, then $x(\om_1^*) \le x(\om_2^*)$ by Assumption~\ref{as:pareto}.
Hence, $x(\om_1^*) \le x(\om_2^*)$ in both cases.
Now suppose that $\om_1^*$ and $\om_2^*$ belongs to the different partitions $\omb_i$ and $\omb_j$.
Suppose that agent $i$'s equilibrium strategy satisfies $\sigma'_i \neq \om_1^*$.
If playing $\omb_i$ is strictly better for agent $i$, it contradicts that $\sigma'_i$ is an equilibrium strategy.
Hence $y(\om_1^*) = y(\sigma_i')$. Again by Assumption~\ref{as:pareto}, since agent $i$ plays $\sigma_i'$, we have $x(\sigma'_i) \ge x(\om_1^*)$.
Note that the principal should observe both $\sigma_i'$ and $\om_2^*$, and commits to $\om_2^*$.
This implies that $x(\om_2^*) \ge x(\sigma') \ge x(\om_1^*)$, and we finish the proof.
\end{proof}

A main implication of the theorem is that the principal can actually increase her utility by recruiting more agents with similar utilities to delegate the task and examining only a single solution from each agent.
Although this does not quantify whether the multi-agent delegation largely improves upon the single-agent setting, delegating to multi-agent still has benefits in the sense that it would take much smaller time (or resource) in terms of the agents if we ask $10$ agents to find $10$ solutions and propose at most one solution each, rather than the scenario that we ask a single agent to find $100$ solutions and propose at most $10$ solutions.



% \begin{question}[Quantifying the delegation gap]\label{quest:2}
% Quantify some reasonable upper bounds on \eqref{ineq:infbud_tau} and ~\eqref{ineq:infbud_notau} with respect to distribution $D_i$ and $k_i$ for $i \in [n]$ will be interesting.
% Following the proof technique of prophet inequalities, it seems to be doable to initially prove that we have $2$-approximation.
% Upton this, if we can derive a big improvement over $2$ or $e/(e-1)$ for some regimes, then it will be interesting.
% We may firstly consider a simplistic setting of two agents and $D_i = D$, maybe uniform distribution, and $k_i = k$, and further extend it.
% For example, if $k_i=1$ and $x(D_i) = U[a,b]$ for some positive $a,b > 0$, then it seems to be straightforward to check that the delegation gap is upper bounded by $\mO(1/n)$, using some order statistics (although we do not precisely define $x(D_i)$, we use it to denote the distribution of $x(\om)$).

% Negative results for some characterizations on $k_i,D_i$ might be also interesting. We can say something like if the distributions are something like this, then multi-agent delegation does not improve much, so just better off settling with a single agent.

% Finally, we may try to derive a lower bound on the delegation gap for any mechanism.
% \end{question}

==> Delegating to Multiple Agents (1)/no_cost_comp.tex <==
% !TEX root =  main.tex
\section{Complete information}\label{section:no_cost}
% In this section, we consider a scenario in which the agents can access each others' observed solutions, i.e., each agent not only knows his solutions but also knows what other agents have sampled. 
% This implies that each agent $i$ determines his strategy based on all observed solutions $\omb = \cup_{i=1}^{n} \omb_i$. Formally, agent $i$'s strategy $\sigma_i: \Omega^* \mapsto \Sigma_i$ is a function of all observed solutions to a signal which is typically a subset of his solutions.
% According to Theorem~\ref{thm:multiagent_revel}, it suffices to find a good mechanism over the space of MSPMs.
% Therefore, we analyze the performance of MSPM in both Bayesian and prior-independent settings.  
In the complete information setting, we first present a generic result regarding MSPM with arbitrary threshold-based eligible sets.
%We mainly argue that a large examination budget gives us a significant amount of gain in terms of principal's utility.
% To elaborate, we first present how the single-proposal mechanism behaves under the single-agent setting in terms of $X_{i,j}$ and $Y_{i,j}$, which will be useful in comparing the results.
% Generally, the threshold $\tau$ is set to be half of the expectation of $X_{\max} =  \max_{j \in [k]} X_{1,j}$ so that $\tau = 1/2\Ex{X_{\max}}$.
% Then, by the dynamics of the single-proposal mechanism, solution with highest $Y_j$ satisfying $X_{j} \ge \tau$ will be selected.
% Define $\set{E} = \{\om \in \omb : x(\om) \ge \tau \}$, i.e. the subset of solutions contained in the eligible set.

% We use $\mec_{SP}$ to denote the expected utility of single-proposal mechanism.
% More, formally,
% \begin{align*}
% \mec_{SP}  = \Ex{TBD}
% \end{align*}

\begin{theorem}\label{theorem:multi-agent-unlimited-budget}
Given any $\tau \ge 0$, let $R$ be an eligible set with threshold $\tau$ such that
$R:= \{\omega: x(\omega) \ge \tau, \omega \in \Omega\}$, and $\rho$ be
an arbitrary deterministic
% \footnote{Deterministic here means by the mechanism prespecifies a total ordering on the agents.}
% \footnote{We note that the deterministic tie-breaking rule is necessary. Indeed in Appendix \ref{app_sec:random_tie}, we prove that randomized tie-breaking rule may induce arbitrarily bad delegation gap.} 
tie-breaking rule.
Then, the MSPM with $\rho$ and a homogeneous eligible set $R$ has $\poa_a$ of at most
\begin{align*}
\Ex{X_{(1)}} - \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} - 
\Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.
\end{align*}
\end{theorem}
We present the proof in Appendix \ref{pf_theorem:multi-agent-unlimited-budget}.
To interpret the bound above, suppose that we set $\tau = 0$.
Then it implies that the principal can obtain the utility of first-best solution of the second-best agent.
In addition, by properly defining the eligible set, \ie $\tau$ in this case, she can further improve the potential quality of the candidates, although it might possibly decrease the probability that each agent samples eligible solutions.
Intuitively, the existence of the other agents make each agent more competitive in sending signals, thus motivating them to submit more qualified solution.
% This result implies that 
% without even announcing eligible sets, the principal can expect to receive a candidate that gives her the utility of at least the first-best solution (in terms of principal) of the second-best agent. 
% Furthermore, she can improve the quality of candidates by defining eligible sets, however, it decreases the probability that an eligible solution is observed by any of the agents. 

% The main intuition behind this analysis is that the existence of opponents whose proposed solutions are examined by the principal
% makes agents more competitive in sending signals,
% thus resulting in submitting more qualified solutions to be selected.
\begin{remark}
The role of deterministic tie-breaking rule is essential. 
Indeed if the principal exploits a randomized tie-breaking rule, it may reduce the power of competition in certain cases since the agents may settle with a bad solution in terms of the principal, as it still gives the agents higher utility with some small but still positive probability due to the randomized tie-breaking rule.
\end{remark}

% yet another solution which might induce higher probability to be selected by the principal may yield too low utility for the agents. 
% However for the deterministic tie-breaking rule, as the principal naturally prefers some agents, less preferred agents tend to submit the candidate more in a competitive manner in order to be selected by the principal, and again, this recursively makes preferred agents behave more in favor of the principal.

% \suho{what about briefly discuss why we need deterministic tie-breaking rule? (We will not present Appendix A, but we may borrow some sentences therein)}
As per Remark~\ref{rm:bm_pim_comp}, the mechanism presented in Theorem~\ref{theorem:multi-agent-unlimited-budget} can be either BM or PIM.
% Importantly, the mechanism presented in Theorem~\ref{theorem:multi-agent-unlimited-budget} can be either BM or PIM.
% If it specifies the eligible sets $R_i$ based on the information on the distribution in advance, then it would be a BM mechanism.
% On the other hand, if the mechanism does not determine eligible sets, i.e. $R_i = \Om$, then it would be a PIM.
In what follows, we obtain guarantees for BM and PIM independently by quantifying the approximation factor in Theorem~\ref{theorem:multi-agent-unlimited-budget}.

\subsection{Bayesian mechanism}
For BM, we first show that we can exactly recover the guarantees under the single-agent setting provided in \citet{kleinberg2018delegated} by setting proper eligible sets.
\begin{theorem}\label{thm:recover}
    There exists a BM with $\poa_m \le 2$.
	% For each of the following problem instances, there exists a corresponding mechanism that guarantees the stated principal's expected utility.
    % \begin{enumerate}
    % 	\item There exists an $(2,0)$-approximate informed mechanism.
    % 	\item There exists an $(\frac{e}{e-1},0)$-approximate informed mechanism if the utilities are independent, each of which is drawn from an atomless distribution.
    % 	\item There exists an $((\alpha - \mO(\log n/n))^{-1},0)$-approximate informed mechanism if the utilities are independent, each of which is drawn from an atomless distribution, and if the principal can observe the utility of the agents, where $\alpha = 0.745\ldots$ is the solution of $\int_0^1 (t - \ln t + 1 - 1/t)^{-1}dt = 1$.
    % \end{enumerate}
\end{theorem}
% \begin{remark}
% 	We highlight that in the proof of Theorem \ref{thm:recover}, we in fact prove a stronger statement as elaborated below.
% 	Consider any SPM with an eligible set $R$.
% 	Then, exists an MSPM such that given observed solutions $\omb$ and any corresponding equilibrium strategies $\sigma = (\sigma_1, \ldots, \sigma_n)$, the utility $x(\sigma_i)$ is at least that of the SPM with eligible set $R$ given the observed solutions $\omb_i$, under the single-agent setting in which the principal only delegates to agent $i$.
% \end{remark}
The proof can be found in Appendix \ref{pf_thm:recover}.
To obtain the result above,
we reduce the multi-agent delegation problem to a single-agent one and then
use the results by \citet{kleinberg2018delegated} regarding the upper bound on the multiplicative approximation factor.
% In the proof of Theorem \ref{thm:recover}, we in fact derive a stronger result of comparative statistics such that there always is a multi-agent mechanism which yields higher (or equal) principal's utility compared to any mechanism in the corresponding single-agent setting, formal
% We formally present this result as follows.
\begin{remark}
    In the proof of Theorem \ref{thm:recover}, we in fact derive a stronger result such that there always is a multi-agent mechanism which yields higher (or equal) principal's utility compared to any mechanism in the corresponding single-agent setting.
    We complement this result in Appendix~\ref{sec:compare_mul_sin} by proving that for any single-agent problem instance, we can construct a multi-agent instance with higher (or equal) principal's utility.
\end{remark}
The tightness of the bound in Theorem~\ref{thm:recover} is also obtained as follows.
\begin{theorem}\label{thm:lowerbound_comp_worst}
        For any $\eps>0$, there exists a problem instance such that no BM achieves $\pos_m < 2-\eps$.
\end{theorem}
To construct a matching lower bound, we introduce a \emph{super-agent} of superior solutions.
The super-agent always induce solutions each of which is dominant over any solution by other agents.
The principal thus always select one of the super-agent's solution, which in turn reduces the multi-agent setting to the single-agent setting.
% In order to obtain the lower bound, we introduce the notion of the \emph{super-agent} whose observed solutions are always better than others,
% thus, his proposed solutions are always selected as the winner.
% This reduces the multi-agent setting to a single-agent one where only the super agent exists.
Then we borrow the standard worst-case problem instance of the prophet inequalities to construct a matching lower bound.
The formal proof is provided in Appendix \ref{pf_thm:lowerbound_comp_worst}.
In words, if the principal faces a superior agent who overwhelms all the other agents, there is no merit in delegating to multiple agents, other than the superior one.
%
%\begin{remark}
%This implies that if the principal faces a situation in which there exists a superior agent who overwhelms all the other agents, there is no merit in delegating the task to multiple agents.
%Indeed, if one agent's solution can dominate all the other's solutions for any case, it is intuitive that we don't need to consider those other agents at all since we are interested in only one best solution.
%\end{remark}

This naturally bring us to consider a symmetric assumption defined as follows.
\begin{definition}[Symmetric agents]\label{def:symmetric} 
    \label{def:symmetric-agent}
	If $k_i = k$ for $i \in [n]$, and $D_{i, j} = D$ for $i \in [n], j \in [k]$ we say that the agents are symmetric.
\end{definition}
This assumption implies that the agents have a similar level of effort and skill, and importantly, all the agents can possibly become the owner of the winner.
% In this context, we consider a regime in which the agents have a similar level of effort and ability that are exogenous to the mechanism, i.e. when all of the agents are  capable of observing high-qualified solutions that can become the winner.
\begin{example}
In the example of research proposal selection process we presented in Section~\ref{sec:intro}, the grant agency (principal) may announce a shortlist of the investigators (agents) with a similar level of research abilities, \eg by comparing their publication records.
Indeed, the grant agency will not include an investigator who is expected to be not qualified than the others in the shortlist.
\end{example}
%\suho{please provide some examples on it. as above, I think explanation in the main section should be more informative than contribution section.}
%\kvcomment{is it better now? I just added more sentences.}

The symmetry assumption effectively sparks a fire in the competitive tension between the agents due to their similar level of quality.
Formally, in the following theorem, we obtain an upper bound on the additive approximation factor of a Bayesian mechanism under the symmetric agents.
We refer to Appendix \ref{pf_thm:informed} for the proof.
\begin{theorem}\label{thm:informed}
	Consider symmetric agents such that $X_{i, j} \sim D$ where $D$ is supported on $[0,1]$ and its c.d.f. $F(x)$ satisfies $F(x) \le x^{\alpha}$ for any $x \in [0,1]$ for some $\alpha >0$. 
    Then, there exists a BM with $\poa_m \le \parans{\frac{\alpha nk}{\alpha nk+1}}^{\nicefrac{-1}{\alpha nk}}$, where $ \parans{\frac{\alpha nk}{\alpha nk+1}}^{\nicefrac{-1}{\alpha nk}}$ converges to $1$ as $\alpha n k$ increases.
 % Then, there exists an oblivious mechanism such that under any NE, it is $\parans{\parans{\frac{\alpha nk}{\alpha nk+1}}^{\frac{1}{\alpha nk}},0}$-approximation, which converges to $(1,0)$-approximation.
\end{theorem}

In order to obtain the above result, we introduce a tighter threshold $\tau$ compared to the ones studied in the canonical prophet inequalities algorithm.
Combined with the guarantee of MSPM in Theorem~\ref{theorem:multi-agent-unlimited-budget}, followed by some elementary calculations, we derive the subconstant bound above, where the principal attains the optimal utility as $n$ and $k$ increase.
This is in stark contrast to the general setting under which the principal can obtain only a constant factor of the optimal utility.
% we define eligible sets for agents by putting an appropriate value for $\tau$ and use the upper bound on the additive approximation of MSPM provided in  Theorem~\ref{theorem:multi-agent-unlimited-budget}. Note that as $n$ and $k$ increase, the additive approximation factor in the theorem statement goes to $0$, i.e., the principal gets almost optimal utility. 
% This implies that under the assumption on $F(x)$,
% BM enables the principal to get optimal utility in stark contrast to the single-agent delegated search.
%The representative distributions that satisfy $F(x) \le x^{\alpha}$.

\subsection{Prior-independent mechanism}\label{sec:comp_pim}
Now we turn our attention to the class of PIM.
\footnote{Standard approach to analyze prior-independent mechanism would be to use Bulow-Klemperer-style result by \citet{bulow1994auctions}, but this does not apply for our case. We discuss more in details in Appendix~\ref{sec:BKS}.}
By plugging $\tau = 0$ in Theorem~\ref{theorem:multi-agent-unlimited-budget}, we directly obtain the following corollary, where we omit the proof as it is trivial to derive.
\begin{corollary}\label{cor:infbud_notau}
    There exists a PIM with $\poa_{a}$ of at most $\Ex{X_{(1)}} - \Ex{X_{(2)}}$.
    % in which the delegation gap is upper bounded by $\Ex{X_{(1)}} - \Ex{X_{(2)}}$.
\end{corollary}
% \suho{Maybe we can make a remark that this is indeed tight for any PIM. Then, for Theorem 3.7, we can argue that the bound is tight regarding worst case over the distributions.}
This corollary mainly implies that even without the eligible set, the multi-agent setting brings some advantages for the principal, which is mainly due to the competitive tension between the agents.
As the readers may have noticed, this additive approximation factor is equivalent to the expected difference between the $n$-th (highest) order statistics and $n-1$-th order statistics of the random variables $\left(X_{i,(1)}\right)_{i \in [n]}$, which is again the highest order statistics of each agent.

% We now provide several quantitative results regarding the additive approximation factor of PIM 
% provided in Corollary~\ref{cor:infbud_notau}.
Although there exists a vast amount of papers studying order statistics of similar flavor in the literature, the expected gap $\Ex{X_{(1)} - X_{(2)}}$, \ie the expected difference of the highest order statistics between the first-best and second-best agents, has not been studied before to the extent of our knowledge.
In this context, we provide some analysis under which the additive factor is nicely bounded, using some characterizations on the order statistics.

Before presenting our positive results, we present the following negative result, which dictates that one should consider a reasonable assumption on the distribution to obtain positive results.
\begin{theorem}\label{thm:comp_obl_neg}
    Suppose that both the principal's utility functions are supported on $[0,L]$ for some $L >0$.
    For any $\eps > 0$, there exists a problem instance such that $\pos_a \ge L-\eps$.
    
    % For any PIM, its additive price of anarchy can be arbitrarily large, \ie for any $L > 0$, there exists a problem instance such that $\poa_a \ge L$.
    % In addition, this lower bound is essentially tight in the sense that MSPM with no eligible set achieves it.
    % For any $\eps > 0$, there exists a problem instance such that no oblivious mechanism can achieve $(1, \eps)$-approximation, i.e. the lower bound on the delegation gap is essentially $(1,\infty)$, which 
\end{theorem}
We provide the proof in Appendix \ref{pf_thm:comp_obl_neg}.
Similar to the case of BM, we consider the symmetric agents.
% this again justifies that a certain restriction on the problem instances is necessary in order to derive a meaningful guarantee in the approximation factor.
% To formally argue that any PIM cannot commit to any nontrivial eligible set, we prove that any PIM with some nontrivial eligible sets can have arbitrarily bad approximtion ratio under some instances.
% Correspondingly, we consider the symmetric agents.
In this case, we can derive the following upper bound on the additive approximation factor regardless of the underlying distributions.
We present the proof in Appendix \ref{pf_thm:comp_sym_general}.
\begin{theorem}\label{thm:comp_sym_general}
    Under the symmetric agents, suppose that the principal's utility functions are supported on $[0,L]$. Then there exists a PIM with $\pos_a$ of $L(1-\nicefrac{1}{n})^{n-1}$, where $(1-\nicefrac{1}{n})^{n-1} \le 1/2$ for all $n \ge 2$, and it decreases to $\nicefrac{1}{e}$ as $n$ increases.
\end{theorem}
We also note that this upper bound $L(1-\nicefrac{1}{n})^{n-1}$ is tight for $\Ex{X_{(1)} - X_{(2)}}$, \ie we can construct a problem instance with exactly having $\Ex{X_{(1)} - X_{(2)}} = L(1-\nicefrac{1}{n})^{n-1}$.
% and the matching worst-case instance consists of agents with Bernoulli r.v.s of parameter $1-(1-\nicefrac{1}{n})^{\nicefrac{1}{k}}$, \ie which rapidly decreases w.r.t. $n$ and $k$.
Note that this approximation ratio is a big improvement over the general setting under which the additive approximation factor can be arbitrarily bad.


% =============START OF TEMP=============
% Given a distribution $D$ with probability density function (p.d.f.) $f$ and cumulative distribution function (c.d.f.) $F$, we say that $D$ has \emph{monotone hazard rate} (MHR) if $h(x) = f(x)/(1-F(x))$ is a monotone increasing function on $x$.
% If $h'(x) = f(x)/F(x)$ is a monotone decreasing function, then we say $D$ has \emph{monotone reverse hazard rate} (MRHR).
% Given these notions, we prove that the expected gap between two consecutive order statistics is a monotone decreasing function on $n$.
% \suho{Move it to footnote, and explain it only in the main section.}
% \begin{lemma}[Informal restatement of Lemma \ref{lm:order_stat_diff} and Lemma \ref{lm:order_stat_diff_restricted}]\label{lm:ord_stat_informal}
% 	Given an integer $n$, let $X_1, \ldots, X_n$ be i.i.d. random variables with a distribution $D$ whose p.d.f. is $f(x)$, and $X_{1:n} \le \ldots \le X_{n:n}$ be corresponding order statistics.
% 	Define $\Delta_{k,n} = \Ex{X_{n-k+1:n} - X_{n-k:n}}$ and $\delta_{k,n} = \Ex{X_{k+1:n} - X_{k:n}}$. Then for any $k \le n-1$, the following holds.
% 	\begin{enumerate}
% 		\item If $D$ has MHR, then $\Delta_{k,n}$ is nonincreasing on $n$.
% 		\item If $D$ has MRHR, then $\delta_{k,n}$ is nonincreasing function on $n$.
% 		\item If $f(x)$ is nondecreasing on $x$, then $(n+1)\Delta_{k,n} \le n\Delta_{k,n-1}$
% 		\item If $f(x)$ is nonincreasing on $x$, then $(n+1)\delta_{k,n} \le n\delta_{k,n-1}$.
% 	\end{enumerate}
% \end{lemma}
% \suho{I think it would be better to move this interpretation of the lemmas into the main section, and do not mention anything about the exact lemma statement here (wait, would it be really better? not quite sure :) ). Maybe we can just say that we prove Theorem 2.8 based on two novel lemmas, which might be of independent interest. (Mainly due to limited space)}
% Note that (3) implies (1) and (4) implies (2) respectively.
% Our proof builds upon the technique used in \citet{watt2021concavity} and \citet{li2005note}.
% Our result on (1) and (2) generalizes the result of \citet{li2005note} which only deals with the gap between highest (lowest) and second-highest (lowest) order statistics.
% Although this result seems to be obvious at first glance, this does not always hold for arbitrary distributions.
% Indeed, we provide a counter-example such that (1) does not hold for a non-MHR distribution.
% For a more restricted family of distribution presented in (3) and (4), we obtain stronger results such that the expected gap between $n$ and $n-1$ strictly decreases with a multiplicative factor of $\frac{n}{n+1}$.

% We also prove the following lemma which states that the corresponding properties presented in Lemma \ref{lm:ord_stat_informal} are preserved under order statistics relevant operations over it.
% \begin{lemma}[Informal restatement of Lemma \ref{lm:mhr_preserving} and Lemma \ref{lm:id_preserving}]
% 	Let $X_1,\ldots, X_n$ be i.i.d. random variables with a distribution $D$ whose p.d.f. is $f$.
% 	Then, the following hols.
% 	\begin{enumerate}
% 		\item If $D$ has MHR, then $r$-th order statistics has MHR distribution for any $r\in [n]$.
% 		\item If $D$ has MRHR, then $r$-th order statistics has MRHR distribution for any $r\in [n]$. 
% 		\item If $f(x)$ is nondecreasing on $x$, then the largest order statistics is also nondecreasing on $x$.
% 		\item If $f(x)$ is nonincreasing on $x$, then the smallest order statistics is also nonincreasing on $x$.
% 	\end{enumerate}	
% \end{lemma}
% =============END OF TEMP=============



Moreover, if we consider a specific scenario where the principal's utility is endowed with a certain class of distributions, we show that the approximation factor can become arbitrarily small as the number of solutions per agent ($k$) increases.
At the heart of this result, we prove several new properties on the order statistics, which might be of independent interest.
First, we show that the expected difference between any top $k$-th and $k+1$-th order statistics is a nonincreasing function on $n$ for any distributions with \emph{monotone hazard rates} (MHR).
Note that a distribution $D$ with p.d.f. $f(x)$ and c.d.f. $F(x)$ has a monotone hazard rate if $h(x) = f(x)/(1-F(x))$ is nondecreasing on $x$.
Using a similar technique, we also show that the expected difference between any $k$-th and $k+1$-th lowest order statistics is also a nonincreasing function on $n$, for any distribution with \emph{monotone reverse hazard rate}, where a distribution has MRHR if $h'(x) = f(x)/F(x)$ is nonincreasing on $x$ .

In case of the difference between the first and the second order statistics, or the $n-1$-th and the $n$-th order statistics under the distribution with MHR, \citet{li2005note} shows that they indeed are nonincreasing on $n$ with applications to the expected rent of the (reverse) auction.
To the best of our knowledge, we first provide a generalized and strengthened result of theirs.
Our proof builds upon the techniques by \citet{watt2021concavity} which proves the convexity of $k$-th order statistics with respect to $n$.
We present the precise statement below, and its proof is provided in Appendix \ref{pf_lm:order_stat_diff}.
\begin{lemma}\label{lm:order_stat_diff}
	   Let $X_1, \ldots, X_n$ be i.i.d. random variables equipped with a continuous distribution $D$.
		Let $X_{1:n} \le \ldots \le X_{n:n}$ be corresponding order statistics.
		Define $\Delta_{k,n} = \Ex{X_{n-k+1:n} - X_{n-k:n}}$, \ie the difference between the $k$-th largest and $k+1$-th largest order statistics, and $\delta_{k,n} = \Ex{X_{k+1:n} - X_{k:n}}$.
		Then, for any $k \le n-1$, the following holds.
		\begin{enumerate}
			\item If $D$ has MHR, then $\Delta_{k,n}$ is a nonincreasing function on $n$.
			\item If $D$ has MRHR, then $\delta_{k,n}$ is a nonincreasing function on $n$.
		\end{enumerate}
	\end{lemma}
 \begin{remark}
The fact that these quantities are nonincreasing on $n$ is fairly intuitive at first glance since as more samples are drawn their order statistics will lie more compactly within a fixed interval, however, this is not true in hindsight for certain cases. For example, in case of Bernoulli distribution with $p=1/2$, it is straightforward to check that $\Delta_{k,n} = \Pr{\sum_{i=1}^n X_i = n-(n-k+1)+1 = k}= \binom{n}{k}2^{-n}$. Hence, $\Delta_{k,n} \ge \Delta_{k,n+1}$ is equivalent to $\frac{n+1}{n-k+1} \le 2$, which holds only for $k \le \frac{n+1}{2}$.
\end{remark}
 
Next, we prove that any $k$-th order statistics of i.i.d. random variables with MHR distribution has MHR distribution, which also has not been studied before to the extent of our knowledge. We defer the proof in Appendix \ref{pf_lm:mhr_preserving}.
\begin{lemma}\label{lm:mhr_preserving}
		Let $X_1, \ldots, X_n$ be i.i.d. random variables equipped with a MHR distribution, then its $r$-th order statistics has MHR distribution for any $r \in [n]$.
	\end{lemma}

Using the two lemmas described above, we prove that under MHR distribution, PIM can achieve subconstant additive approximation factor as follows. We present the proof in Appendix \ref{pf_thm:mhr_upperbound}.
\begin{theorem}\label{thm:mhr_upperbound}
    Under symmetric agents with $X_{i,j} \sim D$ such that $D$ has MHR,  there exists a PIM with $\poa_a \le \sqrt{\frac{4}{3}\var(D_{\max})}$ where $D_{\max}$ is the distribution of $X_{i,(1)}$ and $\var(\cdot)$ denotes the variance of the distribution.
    In case of $D = U[0,1]$, the approximation factor becomes approximately $\frac{1.155}{k}$.
\end{theorem}

We note that for uniform distribution, the subconstant approximation factor above guarantees the negative dependency on the number of solutions $k$.
Thus, it improves largely upon the constant factor approximation of Theorem~\ref{thm:comp_sym_general}, and the constant factor approximation ratio of $2$ for the Bayesian mechanism in \citet{kleinberg2018delegated}.

Furthermore, if we consider a more restrictive class of problem instances, we prove that one can obtain both negative dependencies on $n$ and $k$, \ie the $\poa$ converges to $1$ whenever $n$ or $k$ increases.
Similar to the MHR distribution case, our proof heavily relies on the following lemmas.
\begin{lemma}\label{lm:order_stat_diff_restricted}
        Define variables the same as Lemma~\ref{lm:order_stat_diff}.
	Then, for any $k \le n-1$, the following holds.
		\begin{enumerate}
			\item If $f(x)$ is nondecreasing on $x$, then $(n+1)\Delta_{k,n} \le n\Delta_{k,n-1}$.
			\item If $f(x)$ is nonincreasing on $x$, then $(n+1)\delta_{k,n} \le n\delta_{k,n-1}$.
		\end{enumerate}
\end{lemma}

\begin{lemma}\label{lm:id_preserving}
        Let $X_1, \ldots, X_n$ be i.i.d. random variables  with p.d.f. $f$.
	Then, the following holds.
	\begin{enumerate}
		\item If $f(x)$ is nondecreasing, then the p.d.f. of the largest order statistics is  nondecreasing on $x$.
		\item If $f(x)$ is nonincreasing, then the p.d.f. of the smallest order statistics is  nonincreasing on $x$.
	\end{enumerate}
\end{lemma}

We highlight that Lemma \ref{lm:order_stat_diff_restricted} implies that the expected difference between two consecutive order statistics is strictly decreasing over $n$ with the factor of $\nicefrac{n}{n+1}$.
Using the above lemmas, we obtain the following theorem, where the proof is presented in Appendix \ref{pf_thm:decaying_upperbound}.
\begin{theorem}\label{thm:decaying_upperbound}
        Under symmetric agents with $X_{i,j} \sim D$ such that $D$ has nondecreasing p.d.f. $f(x)$, there exists a PIM with $\poa_a \le \frac{1}{n+1}\sqrt{12\var(D_{\max})}$.
	In case of $D = U[0,1]$, the approximation factor becomes approximately $\frac{3.464}{k(n+1)}$.
\end{theorem}
This strictly improves upon the approximation factor of Theorem \ref{thm:mhr_upperbound}, since the approximation factor has positive effects on both $k$ and $n$.
This highlights that delegating to multiple agents indeed brings significant advantages over the single-agent case, under which the best one may hope for is to construct constant factor approximation ratio even with Bayesian mechanism.
Notably, the approximation factor decreases to zero as $n$ or $k$ increases, \ie the principal's utility converges to $\Ex{X_{\max}}$.
% The above theorem gives us a better approximation bound which is a function of both $n$ and $k$, i.e., as any of $n$ or $k$ increases, the approximation factor decreases to zero, i.e. the principal's utility converges to $\Ex{X_{\max}}$.
It remains a major open problem to see whether the guarantees above are tight or not.



%If the distributions are further specified, 
%For example, in case of symmetric agents with uniform distributions, we can guarantee the following approximation ratio.
%\begin{corollary}
%Suppose that $k_i = k$ for all $i \in [n]$.
%Then, the principal's utility is at least
%Suppose that the distribution of $x(\om)$ for $\om \sim D_i$ follows the uniform distribution $U[0,1]$ and $k_i = k$ for $i \in [n]$. Then, there exists a mechanism in which the principal's expected utility is at least $(1-o(1/n))\Ex{X_{\max}}$.
%\end{corollary}





% \begin{example}
% Given a solution space $\Omega = \{a,b,c\}$, consider $n=4$ agents with the same utility function $y(a) = 100$, $y(b) = 10$ and $y(c) = 1$ and a principal with utility function $x(a) = 1$, $x(b) = 10$ and $x(c) = 100$.
% Each agent samples two solutions.
% Agents $1,2$ sample $a$ or $c$ with equal probability, and agents $4,5$ sample $b$ or $c$ with equal probability.
% Consider a RSPM with a random tie-breaking rule, eligible sets $R_i$ for $i \in [n]$ and unlimited budget.
% Suppose that the agents' solutions are realized to be $\{a,c\}$,$\{a,c\}$,$\{b,c\}$ and $\{b,c\}$.
% \end{example}





% \begin{question}[Quantifying the delegation gap]\label{quest:2}
% Quantify some reasonable upper bounds on \eqref{ineq:infbud_tau} and ~\eqref{ineq:infbud_notau} with respect to distribution $D_i$ and $k_i$ for $i \in [n]$ will be interesting.
% Following the proof technique of prophet inequalities, it seems to be doable to initially prove that we have $2$-approximation.
% Upton this, if we can derive a big improvement over $2$ or $e/(e-1)$ for some regimes, then it will be interesting.
% We may firstly consider a simplistic setting of two agents and $D_i = D$, maybe uniform distribution, and $k_i = k$, and further extend it.
% For example, if $k_i=1$ and $x(D_i) = U[a,b]$ for some positive $a,b > 0$, then it seems to be straightforward to check that the delegation gap is upper bounded by $\mO(1/n)$, using some order statistics (although we do not precisely define $x(D_i)$, we use it to denote the distribution of $x(\om)$).

% Negative results for some characterizations on $k_i,D_i$ might be also interesting. We can say something like if the distributions are something like this, then multi-agent delegation does not improve much, so just better off settling with a single agent.

% Finally, we may try to derive a lower bound on the delegation gap for any mechanism.
% \end{question}

==> Delegating to Multiple Agents (1)/no_cost_incomp.tex <==
\section{Incomplete information}\label{section:no_cost_incomp}
% In this section, we consider a scenario in which the agents only have partial information on each other's solutions.
% Unlike in the previous section, each agent cannot access the observed solutions of the other agents but is only aware of the distributions and the number of solutions that the other agents are associated with.
% This corresponds to the Bayesian game between the agents in the literature.
Recall that in the incomplete information setting, each agent $i$ decides his own action at the interim stage of the Bayesian game, \ie when he observes his own solutions.
% each agent $i$ first samples his own solutions $\omb_i = \{\om_{i,1}, \ldots, \om_{i,k_i}\}$ and determines his own strategy based on the belief on the other agents' types, i.e. each agent decides own action at the interim stage of the Bayesian game.
More formally, agent $i$'s strategy $\sigma_i: \Omega^* \mapsto \Sigma_i$ is a function from the observed solutions to a signal, which is typically a subset of solutions.
We denote by $\sigma_i(\omb_i)$ the agent's action given the observed solution $\omb_i$.
Given $\omb_i$ and others' strategies $\sigma_{-i}$, agent $i$'s strategy $\sigma_i(\omb_i)$ induces the following expected utility.
\begin{align*}
	u_i(\sigma_i(\omb_i), \sigma_{-i})
	=
	\Ex{y_i(f_{M,(\sigma_i(\omb_i), \sigma_{-i})})}
	=
	\int_{\omb_{-i}}\Ex{y_i(f_{M,(\sigma_i(\omb_i), \sigma_{-i}(\omb_{-i}))})}f_{-i}(\omb_{-i})d\omb_{-i},
\end{align*}
where $f_{-i}(\omb_{-i})$ denotes the p.d.f. of observing $\omb_{-i}$.
Namely, each agent accounts for the probability that certain solutions are observed by the other agents, confirms their corresponding strategies, and computes his own utility based on them.
This process is captured by the integral in the last equation.
Note that the expectation inside the integral accounts for the random bits of the mechanism, which does not appear in deterministic mechanisms.

Then, given the others' strategies $\sigma_{-i}$, agent $i$'s expected utility of playing $\sigma_i$ can be written as
\begin{align*}
	u_i(\sigma_i, \sigma_{-i})
	=
	\Exu{\omb_i}{u_i(\sigma_i(\omb_i), \sigma_{-i})}	
	= \int_{\omb_i} u_i(\sigma_i(\omb_i), \sigma_{-i})f_{i}(\omb_i)d\omb_i.
\end{align*}
%Given an event $A$ regarding the realization of the principal's and agents' utilities, 
%we further define a conditional expected utility as follows.
%\begin{align*}
%	u_i(\sigma_i,\sigma_{-i}|\omb_i, \omb_{-i}, A)
%	=
%	\Ex{y_i(f_{M,(\sigma_i, \sigma_{-i}|\omb_i, \omb_{-i})}) \given \omb \in A}
%\end{align*} 

%For simplicity, we denote by $x_i(\sigma)$ the expected utility of the principal given the strategies $\sigma = (\sigma_1, \ldots, \sigma_n)$.
Finally, a Bayesian Nash equilibrium can be defined as follows.
\begin{definition}[Bayesian Nash Equilibrium]
	Under the incomplete information setting, given a mechanism $M$, a set of strategies $(\sigma_1,\sigma_2,\ldots, \sigma_n)$ is defined to be a Bayesian Nash equilibrium (BNE), if for any $i \in [n]$, $\sigma_i$ satisfies the following for any other strategy $\sigma'_i$ of agent $i$.
	\begin{align*}
		u_i(\sigma_i, \sigma_{-i}) \ge u_i(\sigma'_i, \sigma_{-i}).
	\end{align*}
	% for any other strategy $\sigma'_i$ of agent $i$.
\end{definition}
Our main objective is to construct a mechanism that induces a large principal's expected utility under its BNE.
In the case of incomplete information, the analysis of the approximation ratio becomes more involved as all the computations of the expected payoff of some strategies entail probabilistic arguments regarding the realization of the others' solutions.
Moreover, since the \emph{feasible} strategy depends on the realization of the solutions for each agent, its analysis significantly differs from the standard Bayesian games such as the first-price auction or the all-pay auction.
Due to this fact, even under the symmetric agents, the standard technique of computing symmetric BNE in the first-price auction, \eg which involves the use of the Envelope theorem \cite{milgrom2002envelope}, does not apply to our setting.
Despite these analytical challenges, we succeed in obtaining several positive results in terms of the PIM.

Before presenting our main result on PIM, we first study the class of the Bayesian mechanism.
In the case of BM, it is straightforward to see that all the results in the complete information setting hold in the incomplete information setting as well.
\begin{corollary}\label{thm:recover_bayes}
	Theorem~\ref{thm:recover}, \ref{thm:lowerbound_comp_worst}, and \ref{thm:informed} still holds for the incomplete information setting.
\end{corollary}
We skip the proofs as exactly the same arguments of the corresponding proofs in the complete information setting directly carry over to the incomplete information setting.


% Furthemore, similarly from the complete information setting, if we do not restrict the problem instances at all, the worst-case lower bound of the approximation ratio is equivalent to the single-agent setting.
% \begin{theorem}
% 	Theorem~\ref{thm:lowerbound_comp_worst} still holds for the incomplete information setting.
% \end{theorem}
% \begin{proof}
% 	We can exactly follow the same proof of Theorem~\ref{thm:lowerbound_comp_worst}
% 	since definition of super agent still works under incomplete information setting.
% \end{proof}
% Now we consider symmetric agents.
% Similarly from Theorem~\ref{thm:informed}, we observe that there exists a BM with a good approximation ratio which decreases as $n,k$ increases, and converges to $1$, i.e. $\Ex{X_{\max}}$.
% \begin{theorem}
% 	Consider symmetric agents endowed with distribution $D$ with support on $[0,1]$ such that its c.d.f. $F(x)$ satisfies $F(x) \le x^{\alpha}$ for any $x \in [0,1]$ for some $\alpha >0$. Then, there exists an oblivious mechanism such that under any BNE, the delegation gap is at most $1 - \parans{\frac{\alpha nk}{\alpha nk+1}}^{\frac{1}{\alpha nk}}$, which converges to $0$.
% \end{theorem}
% We omit the proof since the proof of Theorem~\ref{thm:informed} directly applies to this case as well.
In the case of PIM, similar to the complete information setting, we can directly argue that the additive approximation factor can be arbitrarily bad.
% we start with the following negative result which states that without any restriction on the problem instance, the principal may experience arbitrarily bad expected utility compared to $\Ex{X_{\max}}$ in the worst-case scenario, where 
We omit the proof as it is exactly the same as the proof of Theorem \ref{thm:comp_obl_neg}.
\begin{corollary}\label{thm:pim_lower}
    Theorem \ref{thm:comp_obl_neg} still holds for the incomplete information setting.
\end{corollary}

This again naturally leads us to focus on the symmetric agents.
Interestingly however, in the following theorem, we show that even under the symmetric agents, for any PIM, there exists a problem instance such that proposing a solution that minimizes the principal's utility constructs a BNE, and thus we can construct a problem instance such that the approximation factor can be arbitrarily bad.
We defer the proof in Appendix \ref{pf_thm:pim_neg_incomp}.
\begin{theorem}\label{thm:pim_neg_incomp}
        Under the symmetric agents, there exists no PIM such that $\poa_a < \Ex{X_{(1)} - \max_i X_{i,(k)}}$.
        % for any PIM, its additive price of anarchy is at least $\Ex{X_{(1)} - \max_i X_{i,(k)}}$.
        For the uniform distribution $x(D_{i,j}) \sim U[0,1]$, there exists no PIM such that $\poa_a < \frac{k-1}{k+1} - \sqrt{\frac{\log n}{2k+3}}$,
        \ie the additive approximation factor of any PIM can be arbitrarily bad as $k$ increases given $n$.
\end{theorem}



%\begin{example}
%    \todo{Some generalizations of this result?}
%	Consider two symmetric agents with independent utility functions such that $x(\cdot)$ is sampled from a discrete set $\{0.5,1\}$ with equal probability and $y(\cdot)$ is sampled from a discrete set $\{0.01, 1\}$ with equal probability.
%	Suppose that both agents sample two solutions, and we run an MSPM with no eligible sets with a deterministic tie-breaking rule that prefers agent $1$.
%	Suppose that agent $1$ observes solutions $\{\om_1, \om_2\}$ such that $(x(\om_1),y(\om_1)) = (0.5,1)$ and $(x(\om_2),y(\om_2)) = (1,0.01)$.
%	Suppose that agent $2$ plays a strategy that proposes a solution maximizing the principal's utility.
%	By proposing $\om_1$, the expected utility of agent $1$ is $\frac{1}{4}\cdot 1 + \frac{3}{4} \cdot 0 = 0.25$, and by proposing $\om_2$, the expected utility of agent $1$ is $1 \cdot 0.01 = 0.01$.
%	This implies that proposing $\om_1$, which gives the principal a smaller utility, is the better strategy for agent $1$ based on the randomness over the other agent's solutions, even if the agent knows that the other will play to maximize the principal's utility.
%\end{example}
Compared to the subconstant approximation ratio of Theorem~\ref{thm:mhr_upperbound} and~\ref{thm:decaying_upperbound} in the complete information setting, Theorem~\ref{thm:pim_neg_incomp} implies rather pessimistic consequence such that its worst-case guarantees may become arbitrarily bad, alike to the efficiency of prior-independent mechanism in the single-agent setting.
Thus, the gain from multi-agent delegation becomes highly restrictive.


This negative result mainly arises from the fact that each agent has a utility function which is negatively correlated with the principal's utility, and they have limited information regarding each other's solutions.
This induces the agents to propose more in a selfish manner, compared to the complete information setting.

This phenomenon resembles the \emph{bid shading} effect in the BNEs of the first-price auction, in which the bidders tend to bid less than their valuations in equilibriums.
Due to the lack of information on the other's strategy, each agent may tend to submit a candidate which brings more ex-post utility even though it has a smaller chance of being selected.
Similarly from the first-price auction, this is mainly to prevent the case in which he submits more in favor of the principal  when the others' solutions were revealed to be less competitive in terms of being selected.
Combined with this effect and the fact that the agent's utility is strongly negatively correlated with the principal's utility, each agent tends to submit a solution that minimizes the principal's utility.

In this context, one natural question is whether we can recover a better approximation ratio in more restricted problem instances.
To this end, we consider the following assumption.
\begin{definition}[Independent utility]
    \label{def:indep-utility}
    A problem instance satisfies independence if $D_i$ is a product measure over $D_{i,x}$ and $D_{i,y_i}$, \ie $D_i = D_{i,x} \times D_{i,y_i}$, such that each of $x(\cdot)$ and $y_i(\cdot)$ are associated with the distributions $D_{i,x}$ and $D_{i,y_i}$ respectively, and $D_i$ is independent for $i \in [n]$.
\end{definition}
Note that with independent utility assumption, we can overcome the bad problem instance presented in the proof of Theorem \ref{thm:pim_neg_incomp}, as the principal and the agents do not longer have negatively correlated utility, but are rather not correlated at all.
Although we only obtain a positive result under the independent utility assumption due to the analytical tractability, we hope that one may extend our analysis into the case where the principal and the agents have positively correlated utility (or mild amount of negative correlation), and we leave it as a major open problem.

Due to the intrinsic difficulties in analyzing BNE, we consider a more general solution concept of approximate equilibrium defined as follows.
\begin{definition}[Approximate BNE]\label{def:apxbne}
	Given a mechanism $M$, a set of strategies $\sigma = (\sigma_1, \ldots, \sigma_n)$ is $\eps$-approximate BNE if for any $i \in [n]$, $\sigma_i$ satisfies the following for any other strategy $\sigma'_i$ of agent $i$.
	\begin{align*}
		u_i(\sigma_i, \sigma_{-i}) \ge u_i(\sigma'_i, \sigma_{-i}) - \eps,
	\end{align*}
	% for any other strategy $\sigma'_i$ of agent $i$.
\end{definition}
Our definition of $\pos$ and $\poa$ naturally carries over to the approximate equilibrium.
We eventually present our main result in the incomplete information setting.
Our main result in the incomplete information setting is as follows.
% When we consider symmetric agents, in which the principal's utility for each solution follows uniform distribution $U[0,1]$, and the independent utility assumption, we show that there exists a PIM such that the approximation factor is exactly \emph{optimal} for some constant-factor approximate BNE.
\begin{theorem}\label{thm:bayes_oblivious}
        Under the symmetric agents and independent utility with $X_{i,j} = X \sim U[0,1]$, there exists a PIM such that there exists $\eps$-approximate BNE that results in the optimal utility, \ie $\Ex{X_{\max}}$,  where $\eps = 1-e^{-\frac{n^2}{2(n-1)^2}}$.
        Note that $1 - e^{-\frac{n^2}{2(n-1)^2}}$ converges to $1-\nicefrac{1}{\sqrt{e}} \cong 0.3935$ as $n$ increases.
\end{theorem}
The proof can be found in Appendix \ref{pf_thm:bayes_oblivious}.
Remarkably, this implies that the principal can recover the optimal utility if the agents agree to sacrifice only a constant portion of their utility.
This is indeed possible due to the independence assumption and the fact that the agent does not have the exact information on the others' solutions.

Our proof is based on analyzing the probability of the event that the principal's and the agent's utility is somehow aligned, \ie an agent maximizes his expected utility by proposing his best solution in terms of principal. We show that this probability is lower bounded by $\exp \parans{\frac{-n^2}{2(n-1)^2}}$,\footnote{In Appendix \ref{app:c}, we numerically verify that our lower bound is almost tight.} which converges to $\nicefrac{1}{\sqrt{e}}$ as $n$ increases.
% some absolute constant that does not depend either on $n$ or $k$ \keivan{correct?}.
The proof heavily relies on the FKG inequality (Lemma \ref{lm:FKG}) and some properties on the joint density function of two order statistics.
\begin{remark}
    In appendix \ref{sec:correlated_equi}, we also prove that using a similar but more involved technique, we can derive that there exists a PIM such that under some \emph{Bayes correlated equilibrium}, it achieves $\parans{\exp\parans{\frac{n^2}{2(n-1)^2}},0}$-approximation, \ie constant approximation ratio for sufficiently large $n$.
\end{remark}

\begin{remark}
Note that in some cases it might be complicated or even computationally intractable for each agent to compute a best-response given the others' strategies since he needs to account for every possible realization of the solutions for the others.
In this context, it would be reasonable for the agents to follow the mechanism's recommendation to propose a solution that maximizes the principal's utility, even though it may slightly decrease their utility up to some constant factors.
\end{remark}






% \begin{proof}
%     We first define the following notion of conditional Bayesian-Nash equilibrium.
%     \begin{definition}[Conditional BNE]
% 	Under the incomplete information setting, given a mechanism $M$, a set of strategies $(\sigma_1,\sigma_2,\ldots, \sigma_n)$ is defined to be a conditional Bayesian Nash equilibrium (BNE) given a condition $W$, if $\sigma_i$ satisfies
% 	\begin{align*}
% 		\Ex{y_i(f_{M, (\sigma_i,\sigma_{-i})}) \given W} \ge \Ex{y_i(f_{M, (\sigma'_i, \sigma_{-i})})\given W},
% 	\end{align*}
% 	where $\Ex{y_i(f_{M, (\sigma_i,\sigma_{-i})})}$ is computed based on \eqref{eq:12161312}.
%     \end{definition}

% Then, define sth like follows
% \begin{definition}[Approximately BNIC]
% 	We say that a S-SPM mechanism $M$ is $\eps$-approximately BNIC if there exists a $W$ such that $M$ has a conditional BNE w.r.t. $W$ such that $\Pr{W} \ge \eps$.
% \end{definition}
% \begin{proposition}
% 	If $M$ is $\eps$-approxiamtely BNIC w.r.t. $W$ and have delegation gap $\rho$ conditioned on $W$, then we have $(\eps, \rho)$-delegation gap.
% \end{proposition}
% 	Observe that agent $i$'s utility on playing $\sigma_i$ is
% 	\begin{align*}
% 		u_i(\om | \omb_i) 
% 		&=
% 		y(\om)q(\om)
% 		\\
% 		&=
% 		\sum_{\omb_{-i}}y(\om)\Pr{f(\om) \ge f(\om_j),\forall j \neq i}p(\omb_{-i})	
% 	\end{align*}	
% 	Define $W = \{\omb: x(\om)^{k(n-1)}y(\om) \ge x(\om')^{k(n-1)}y(\om'),\forall \om,\om' \in \omb, \iff x(\om) \ge x(\om'), \forall \om,\om'\in \omb\}$.
% 	1. Compute this probability, (seems to be a constant, but not quite sure though).
% 	2. Under this event, maximizing $x(\om)$ is BNE, as the above utility becomes $y(\om)\cdot x(\om)^{k(n-1)}$.
% 	3. Then, we have BNIC under $W$.
% 	4. Approximation ratio is $1$, i.e. optimal in this case.
% 	5. Hence, $(\Omega(1), 1)$-delegation gap.
% \end{proof}






%\begin{theorem}
%	Consider an independent symmetric setting where $D_i = U[0,1] \times U[0,1]$ for any agent $i \in [n]$ for $n \ge 2$ and $k=1$.
%	Then, there exists a mechanism and a corresponding BNE of which the delegation gap is upper bounded by $2^{1/(n-1)}$.
%\end{theorem}
%\begin{proof}
%	We consider a specific form a single-proposal mechanism in which there exists no eligible set, and the principal selects a solution which maximizes $f(x(\om), y(\om))$ for some given real-valued function $f$.
%	Let $F$ be the c.d.f. of $f(\om)$.
%	We focus on a symmetric equilibrium in which all the agents play the same strategies given the observed set of solutions.
%	Let $q_i(\om)$ be the probability that $\om$ is selected as the winner by the mechanism once it is proposed by agent $i$.
%	At any symmetric BNE, it is obvious that $q_i(\om) = q_j(\om)$ for any $i,j \in [n]$.
%	Let $q_i(\cdot) = q(\cdot)$ for simplicity.
%	Given $\om_{-i}$, if agent $i$'s $\om$ is selected as the winner, then it is trivial that agent $i$'s $\om'$ such that $x(\om') \ge x(\om)$ will be also selected by the mechanism.
%	This implies that $q(\om) \ge q(\om')$ if $x(\om) \ge x(\om')$ for any $\om, \om' \in \Omega$.
%	
%	We first focus on $k=2$.
%	
%	
%	
%	We first prove that proposing a solution that maximizes $f(\om)$ is a BNE.
%	
%	The expected utility of agent $i$ proposing $\om \in \omb_i$ can be computed as
%	\begin{align*}
%		u_i(\om | \omb_i) 
%		&=
%		y(\om)q(\om)
%		\\
%		&=
%		\sum_{\omb_{-i}}y(\om)\Pr{f(\om) \ge f(\om_j),\forall j \neq i}p(\omb_{-i})
%		\\
%		&\ge 
%		F(f(\om))y(\om)
%		\\
%		&=
%		x(\om)^{k(n-1)}y(\om).
%	\end{align*}
%	Moreover, we have
%	\begin{align*}
%		u_i(\om | \omb_i) 
%		&=
%		y(\om)\Pr{x(\om) \ge x(\sigma_j),\forall j \neq i}
%		\\
%		&\le
%		y(\om)\Pr{\forall j \neq i, \exists \om' \in \omb_j :x(\om) \ge x(\om')}
%		\\
%		&\le
%		y(\om)(1- (1-x(\om))^{k})^{n-1} \le y(\om)(kx(\om))^{n-1},
%	\end{align*}
%	where the last inequality follows from $(1-x)^k \ge 1-kx$
%	This implies that
%	\begin{align*}
%		x(\om)^{k(n-1)}
%		\le 
%		q(\om)	 
%		\le (1-(1-x(\om))^k)^{n-1}
%	\end{align*}
%	Each agent $i$ selects a solution that maximizes
%	\begin{align*}
%		\sigma_i = \argmax_{\om\in \omb_i} y(\om)q(\om).
%	\end{align*}
%	Such an optimal strategy satisfies
%	\begin{align*}
%		y(\sigma_i)(kx(\sigma))^{n-1}
%		\ge 
%		y(\sigma_i)q(\sigma_i) 
%		\ge 
%		y(\om)x(\om)^{k(n-1)},
%	\end{align*}
%	for any $\om \in \omb_i$.
%	Let $s$ be the agent who possesses the optimal solution in terms of the principal.
%	Then, we have
%	\begin{align*}
%		y(\sigma_s)(kx(\sigma_s))^{n-1}
%		&\ge
%		y(\om)x(\om)^{(k-1)(n-1)}\cdot x(\om_i^*)^{n-1}
%		\\
%		&= 
%		y(\om)x(\om)^{(k-1)(n-1)}\cdot x(\om^*)^{n-1}
%	\end{align*}
%	for any $\om \in \omb_s$, $\om_s^* = \argmax_{\om \in \omb_s}x(\om)$ and $\om^* = \argmax_{\om \in \omb}x(\om)$.
%	Hence we have
%	\begin{align*}
%		k \cdot \Ex{\max_{i \in n}x(\sigma_i)}	
%		&\ge 
%		\Ex{x(\sigma_s)}
%		\\
%		&\ge 
%		\Ex{(\frac{y(\om)}{y(\sigma_s)})^{\frac{1}{n-1}}x(\om)^{k-1}x(\om^*)}
%		\\
%		&\ge
%		\Ex{y(\om)^{\frac{1}{n-1}}x(\om)^{k-1}x(\om^*)}
%		\\
%		&=
%		\Ex{y(\om)^{\frac{1}{n-1}}}\Ex{x(\om)^{k-1}}\Ex{x(\om^*)}
%	\end{align*}
%
%
%
%	Note that delegation gap $c$ is the minimal $c\ge 1$ satisfying
%	\begin{align*}
%		c\cdot \Ex{\max_{i \in [n]}x(\sigma_i^*)} 
%		\ge 
%		\Ex{\max_{\om \in \omb} x(\om)}.
%	\end{align*}
%	For any $\om \in \omb_i$ the proposed candidate of agent $i$ satisfies
%	\begin{align*}
%		x(\sigma_i^*) 
%		\ge 
%		x(\om)y(\om)^{1/(n-1)}/y(\sigma_i^*)^{1/(n-1)}
%		\ge
%		x(\om)y(\om)^{1/(n-1)}.
%	\end{align*}
%	This implies that
%	\begin{align*}
%		\Ex{\max_{i \in [n]}x(\sigma_i^*)}
%		&\ge
%		\Ex{\max_{\om \in \omb}y(\om)^{1/(n-1)}x(\om)}
%		\\
%		&\ge 
%		\Ex{y(\om)^{1/(n-1)}\max_{\om \in \omb}x(\om)}
%		\\
%		&=
%		\Ex{\max_{\om \in \omb}x(\om)}\cdot \Ex{y(\om)^{1/(n-1)}}
%		\\
%		&= \Ex{\max_{\om \in \omb}x(\om)}\cdot \Ex{U[0,1]^{1/(n-1)}}
%		\\
%		&\ge \Ex{\max_{\om \in \omb}x(\om)}\cdot \Ex{U[0,1]}^{1/(n-1)} = \Ex{\max_{\om \in \omb}x(\om)} \cdot \frac{1}{2^{1/(n-1)}},
%	\end{align*}
%	where the last inequality follows from Jensen's inequality.
%	If $Y_{i,1} \sim U[0,1]$, we have delegation gap of $2^{1/(n-1)}$.
%	This is $2$ for $n=2$, and $2^{1/2}= 1.414$ for $n=3$, and converges to $1$ as $n$ increases.
%\end{proof}


% Now we aim to balance the trade-off between BNIC and efficiency of the mechanism.
% \note{We can consider a score function of forms sth like $f(\om) = x(\om)y(\om)$, which will nicely balance between the principal's and agent's utility.}

% Let $F_f(\om) = \sum_{\omb_{-i}}\Pr{f(\om) \ge f(\om_j),\forall j \neq i}p(\omb_{-i})$.
% Denote $f(\om) = f(x(\om),y(\om))$ then $F_f(\om) = g(f(x,y))$.
% Then, utility is $u_i(\om) = g(f(x,y))y$.
% If we find a $f,F_f$ such that maximizing $u_i(\om) = g(f(x,y))y$ is maximizing $f(x,y)$, then we have BNIC with respect to $f$.
% Then, the principal's utility will be characterized by $\Ex{x(\om) \given \om = \argmax_{\om \in \omb}f(\om)}$.
% For example, if we have $f = xy$, then we have $\Ex{x(
% \om) \given \om = \argmax_{\om \in \omb}x(\om)y(\om)}$, and as $xy$ has positive correlation with $x$, this will (possibly) have some constant approximations to $\Ex{X_{\max}}$.

% We focus on the fact that we have full freedom in designing the eligible set.
% For example, we can design eligible sets $R_i$ like
% \begin{align*}
% 	R_i 
% 	&= 
% 	\{\om: x(\om) \ge y(\om)\}
% 	\\
% 	R_i 
% 	&=
% 	\{\om: x(\om)^2 \ge y(\om), x(\om) \ge \tau\}
% 	.
% \end{align*}
% How does the resulting outcome of the mechanism change?

==> Delegating to Multiple Agents (1)/note.tex <==

\section{Note}


\subsection{Heterogeneous cost}

\begin{question}[Heterogeneous examination cost]
We suppose that the examination cost of a single solution is fixed at $1$.
Instead, consider a scenario in which each solution has a heterogeneous cost $c(\om)$
If this solution $\omega$ is proposed as a candidate and examined by the principal, it incurs an examination cost of $c(\om)$.
The principal's objective can be (1) maximizing utility given an examination budget $B$ or (2) maximizing utility minus total examination cost.
For (1), the problem formulation seems somewhat to be relevant to the stochastic knapsack (though not exactly the same) but the difference is that the problem parameters are the proposed candidates, and thus strategically determined.
For (2), it seems to be very relevant to Weitzman's box problem, but the difference is that again, the parameters are strategically decided.
However, in order to derive some interesting results, I think it would be reasonable to compare with another benchmark, rather than the strong benchmark of the delegation gap.
This is because, if we still compare with the case in which the principal can just select the optimal solution among the entire solutions, then what we can only say is whether we can recover the results on the no-cost scenario.
Maybe we can consider a benchmark who has more budgets and can access all the solutions, but does not also know the realization of the solutions, and so is sampling probabilistically.
We may further consider a scenario in which the cost is randomly determined, not publicly available to the principal in advance, but only the distribution is informed.
\end{question}


\paragraph{Plan}
\begin{enumerate}
\item Think about better mechanism
\end{enumerate}



\begin{question}
How does this problem setup differs from procurement auction precisely?
Refer: (..)
\end{question}
Common: (i) adverse selection (information asymmetry), (ii) The player with less information designs a mechanism, (iii) the player with more information sends a signal.

Difference: (i) No monetary transfer

\begin{question}
How does this problem setup differs from crowdsourcing contest precisely?
Refer: (Optimal crowdsourcing contests, GEB 19)
\end{question}
Difference: (i) no monetary transfer, (ii) exogenous samples of agents, i.e. they do not strategize over effort (this does not hold for costly sampling box model)

\suho{In order to position this paper properly, take a careful look at (i) Optimal crowdsourcing contests SODA 12 / GEB 19, literature on procurement auction, and literature on signaling game, and legislative game}

\section{Further Possible Extensions}

\paragraph{Complete information setting}
\begin{enumerate}
    \item Multiple distribution for each agent
    \item Binary model with sampling cost (which corresponds to Weitzman's box problem)
\end{enumerate}


\paragraph{Online extension}


\paragraph{Multi-choice extension}


\begin{question}
does revelation principal (lemma 1~\cite{kleinberg2018delegated}) still holds for multi agent case?
My intuition is that this depends on the information assumption.
In complete information case, I think we can reduce any mechanism to single proposal deterministic mechanism.
\end{question}

Then we can ask what is the characterization of the optimal delegation mechanism.
\begin{question}
What is the optimal delegation mechanism?	
\end{question}


Next, we are interested in the characterization of the scenario in which the competition helps
\begin{question}
In which cases the competition helps compared to the case when the task is only delegated to a single agent.
When compared to single best agent (in terms of the principal), then it corresponds to sth like price of stability, and if compared to single worst agent, then it corresponds to sth like the price of anarchy.
\end{question}

\begin{question}
Delegation gap 
If competition helps or harms, how much the delegation gap increases or decreases?	
\end{question}



\begin{question}
In which situation (characterization of realized samples), competition helps/harms? How much it helps/ harms?
\end{question}
i.e. when does the utility of the principal increase / decrease compared to the scenario when a single agent picks all the $n$ samples by herself?
In here, the single agent might be the best agent (in terms of the principal, thus something like price of stability) or the worst agent (in terms of the principal, thus something like price of anarchy).
If it improves the principal's utility, how much the delegation gap improved compared to $1/2$ of \cite{kleinberg2018delegated}?


\subsection{Incomplete Information}

\paragraph{Improved mechanism}\note{Temporary section...just a bunch of ideas below}
\begin{definition}[Score-based single-proposal mechanism]
    In a score-based single-proposal mechanism (S-SPM), eligible set $R_i$ is announced for each agent.
    Each agent submits a single candidate in the eligible set and the candidate that maximizes a pre-commited score function $f:\Omega \mapsto \R$ is selected as the winner.
\end{definition}
We further define a notion of incentive compatibility.
\begin{definition}[Bayesian-Nash incentive compatibility]
	We say that a S-SPM mechanism $M$ is Bayesian-Nash incentive compatible (BNIC) with respect to the score function $f(\cdot)$ if submitting a solution that maximizes $f(\om)$ constructs a Bayesian-Nash equilibrium of the delegation game.
	We simply say that the mechanism is BNIC if it is BNIC w.r.t. score function $f(\om) = x(\om)$.
\end{definition}
If we can find a BNIC mechanism, then it is the best scenario for the principal, as it can naturally achieve the optimal delegation gap as the agents' strategic decisions are fully aligned with the principal's utility.
This indeed can be achieved under a very specific regime of independent and symmetric settings, described as follows.
\begin{proposition}
	Under the independent and symmetric setting, if $y(\cdot)$ is a linear transformation of $x(\cdot)$, then S-SPM mechanism $M$ with score function $f(\om) = x(\om)$ is BNIC.
\end{proposition}

The above example considers a specific scenario in which the principal's and the agents' utilities are fully aligned.


To guarantee a certain ratio of approximation while guaranteeing the incentive compatibility of the S-SPM, the principal has to sacrifice a bit of utility in designing the score function.
At one extreme, the principal can design a BNIC mechanism by sacrificing all the efficiency of the mechanism.
\begin{proposition}
	Under the independent and symmetric setting, consider a S-SPM mechanism $M$ with score function $f(\om) = y(\om)$.
	Then, $M$ is BNIC.
	However, it's delegation gap can be arbitrarily bad.
\end{proposition}
\suho{More work can be done in this direction. Key point is to design a good score function and eligible sets, in order to incentivize the agents to behave in favor of the principal.
For example, consider a score function $f(\om)= y(\om)x(\om)$ and eligible set $R_i = \{\om : x(\om) \ge y(\om)\}$. Although this will not induce a BNIC mechanism, this somehow efficiently balance the principal's utility and agent's utility so that maximizing score function is good for both the agents and the principal.}





\subsection{Learning setting}
Consider a more practical scenario in which each agent $i$ also does not know the exact values of the own samples $\bar{\omega}_i$, and neither does the principal. (and also does not know the distribution sampled from)
\footnote{Another interpretation: at each round, agent $i$ draws a unknown sample from one of unknown $D_i^{(1)},\ldots, D_i^{(l_i)}$}
Each agent correspondingly registers a set of samples at each round and the mechanism specifies which ones to select as the final outcome at the round.
Only the final outcome's reward is revealed at the end of the round.
\footnote{Another variant would be when each agent has a finite budget and decide whether to sample more solutions with costly effort of $c_i$, or commit with current samples $W_i$.}

Since the value of the solutions are not given in hindsight, threshold based mechanisms like single-proposal mechanism does not apply in this case.
Instead, the principal should design a good sequential decision rule, i.e. the bandit algorithm, to incentivize the agents in preferrable manner.

\begin{question}
What happens in single agent setting?
If agent learns well, he will eventually submit a single solution that maximizes own payoff.
Then, if the principal also learns well, he may apply single proposal mechanism to reject agent's solution after some rounds.

\end{question}

\begin{question}
What happens in single agent setting?
\end{question}



One interesting feature in this repeated setting is that the agents might abuse the exploration of the principal's algorithm as in \cite{shin2022multi}.
For example, if the agent becomes certain that his samples are suboptimal to the principal, he may...



\begin{question}
One interesting question in this setting will be even when all the payoffs are aligned, e.g. all $y_i$ are affine transformation of $x$, the agents might 
\end{question}

\subsection{Multiple selection}
When the principal selects multiple outcomes as final solutions?
For example in 





% \subsection{Further questions that we might work on}
% \begin{definition}[Randomized $k$-proposal mechanism]
% In randomized $k$-proposal mechanism, an eligible set $R \subset \Omega$ is announced by the principal, each agent proposes up to $k$ outcomes, and the principal finally uniform randomly chooses an outcome among the proposed candidates.
% \end{definition}

% \begin{conjecture}
% \suho{not proved, but intuitive}
% Randomized $k$-proposal mechanism admits dominant strategy equilibrium.	
% \end{conjecture}


% \begin{conjecture}
% \suho{not proved, but intuitive}
% Any mechanism $M$ with budget $1$ can be reduced to randomized $k$-proposal mechanism.	
% \end{conjecture}


% \begin{conjecture}
% \suho{not proved, but pretty intuitive}
% Randomized $k$-proposal mechanism achieves $(opt,1)$, i.e. it has optimal delegation gap under any mechanism with budget $1$.
% \end{conjecture}




% \begin{conjecture}
% \suho{not proved}
% There exists a online $f(c)$-proposal mechanism which achieves $(opt_c, c)$-approximation for any $c \in \{1,2,\ldots, \sum_{i=1}^n n_i\}$.
% \end{conjecture}




==> Delegating to Multiple Agents (1)/related_work.tex <==
\section{Related work}\label{sec:related_work}
Initiated by \citet{holmstrom1980theory}, a rich line of literature has studied the delegation mechanism without monetary transfer.
\citet{holmstrom1980theory} considers a setting in which a single agent is delegated to solve an optimization problem over a compact interval, and characterizes conditions under which an optimal solution of the principal exists. \citet{alonso2008optimal} fulfill the results by providing a general characterization of the solution.
\citet{armstrong2010model} study a discrete model in which an agent samples a set of solutions from a distribution and optimizes over the sampled set, which is the most similar problem setup to ours.


While most literature in the theory of delegation aims at characterizing regimes in which the optimal mechanism exists or the structure of it, \citet{kleinberg2018delegated}  study the loss of efficiency from delegating the task into an agent with misaligned payoff. They consider two models, one of which is similar to delegated project choice of \citet{armstrong2010model}.
In this model, the agent samples a fixed number of solutions from a distribution and proposes some of the solutions to the principal in a strategic manner.
% They quantify the gap between a delegated search mechanism and an ideal scenario .
Surprisingly, they show that a simple mechanism enjoys a $2$-approximation ratio compared to the ideal scenario in which the principal can directly choose the optimal solution, based on a connection to the prophet inequalities.
%Their proof is based on a novel observation regarding a connection to the canonical threshold algorithms prophet inequalities.
%The major difference from our paper is that they only consider a single-agent setting, as widely assumed in the delegation literature.

Several works have been devoted to the delegation mechanism without money in the presence of multiple agents.
One of the most relevant problem setting would be \emph{legislative game} with asymmetric information by~\citet{gilligan1989asymmetric}, \citet{krishna2001asymmetric}, \citet{martimort2008informational} and \citet{fuchs2022listen}.
They consider a model in which two self-interested agents with information advantage observe \emph{a state of nature} and independently send a private signal to the principal.
The principal aims to extract truthful information on the state of nature to maximize own utility that depends on it.
Recent works by \citet{alonso2014resource} and \citet{gan2022optimal} extend these settings by considering multiple actions for the principal.
Importantly however, all of their models are significantly different from our model.
In our model, the information asymmetry between the principal and the agents arises from "moral hazard" versus "adverse selection" of the previous works, as per \citet{ulbricht2016optimal}.\footnote{Notably, \citet{ulbricht2016optimal} study both effect of moral hazard and adverse selection in the delegation mechanism but with a monetary transfer. Likewise, there exists a fruitful line of literature dealing with contract-based delegation, \eg \citet{krishna2008contracting} and \citet{lewis2012theory}, but we will not discuss in detail on the delegation mechanism with money.}
In moral hazard, the principal cannot directly observe all the alternatives, but can only access a subset of them based on the signals, whereas in adverse selection, a state of nature is revealed only to the agent but affects the principal's utility  as well.


% \citet{alonso2014resource} firstly study the optimal delegation mechanism without money against three agents.
% They consider the information asymmetry between the principal and the agents such that the principal does not know the state of the nature, and tries to construct an incentive-compatible mechanism to make the agents truthfully report the observed state.
% This is in stark constrast to 


% \citet{alonso2014resource} study the delegation mechanism design without money with multiple agents, but their model is significantly

% Several works are devoted to the delegation mechanism without monetary transfer against multiple agents.

% As our problem conceptually belongs to the signaling model of delegation (we refer to the survey by \citet{bendor2001theories} for more detailed exposition), it seems worthwhile to present several works in a multi-agent version of the signaling model of delegation.
% To the best of our knowledge, the most relevant problem setting would be \emph{legislative game} with asymmetric information by~\citet{gilligan1989asymmetric}, \citet{krishna2001asymmetric}, and \citet{martimort2008informational}.
% They study a problem in which two self-interested agents with information advantage observe a state of nature and independently send a private signal in an interval $I$, i.e. the solution space. 
% A legislator (principal) should then select a solution from the solution space, however, she suffers an adverse selection such that she does not observe the state of nature.
% Instead, she updates her belief on the state of nature from the agents' signals, and finally chooses the solution based on it.
% The legislator's utility depends on the state of nature, thus she aims to extract much information on the state of nature through the mechanism.
% Different from it, the information asymmetry in our setup arises from \emph{moral hazard}, as per~\citet{ulbricht2016optimal}, such that the principal cannot directly observe all the searched solutions, but not from \emph{adverse selection} regarding the information asymmetry on the state of nature.
% \citet{ulbricht2016optimal} study delegation mechanisms by considering both the moral hazard and adverse selection but with a monetary transfer, thus we will not discuss more in detail.
% While there exists a line of literature dealing with contract-based delegated search (\citet{lewis2012theory}, \citet{krishna2008contracting}), we do not discuss it in detail since the problem setup is largely different from ours.

Finally, there is an increasing attention in the Computer Science community regarding an algorithm design with a delegated decision.
\citet{bechtel2020delegated} considers a stochastic probing problem when the principal delegates the role of probing to a self-interested agent. They quantify the loss of delegation similar to \citet{kleinberg2018delegated} by revealing a connection between delegated stochastic probing and generalized prophet inequalities.
\citet{bechtel2022delegated} generalizes the second model of \citet{kleinberg2018delegated}, namely Weitzman's box problem which deals with a costly sampling of the agent, by considering a combinatorial constraint.
% \citet{braun2022delegated} study online version of delegated search in which the agent observes a sequence of samples in an online manner and irrevocably decides whether or not to propose to the principal.

==> Delegating to Multiple Agents (1)/remaining_proofs.tex <==


\section{Proofs}\label{sec:rem_proofs}
\subsection{Proof of Theorem \ref{thm:multiagent_revel}}\label{pf_thm:multiagent_revel}
\begin{proof}
Let $R_i$ be the set of all the solutions belonging to agent $i$ that can be selected by the mechanism $M$, over any feasible $\omb \in \Omega^*$ and corresponding equilibrium strategies, and any random bits of the mechanism.
Given a set of observed solutions by the agents $\omb = \cup_{i \in [n]} \omb_i \in \Omega^*$ and corresponding equilibrium strategy $\sigma$, consider any  $\omega_M \in F_{M,\sigma}(\omb)$.

Suppose that $\om_M$ belongs to agent $i$.
Obviously, $\om_M \in R_i$ holds due to our construction.
Furthermore, in terms of agent $j\neq i$, there exists no solution $\om' \in \omb_j$ such that $x(\om) > x(\om_M)$ since if so, agent $j$ will be selected in $M$ by playing $\om$, \ie for any $\om' \in \omb \setminus \omb_i$,
\begin{align}
x(\om_M) \ge x(\om').	\label{ineq:12051649}
\end{align}
Furthermore, if there exists another $\om \in \omb_i$ such that $x(\om) \ge x(\om')$ for all $\om' \in \omb \setminus \omb_i$ and $y_i(\om) > y_i(\om_M)$, then agent $i$'s utility becomes larger by playing $\om$, which contradicts the assumption that $\sigma_i = \om_M$ is an equilibrium strategy.
Hence, we conclude that whenever such $\om$ exists,
\begin{align}
y_i(\om_M) \ge y_i(\om). \label{ineq:12051650}
\end{align}

Consider a MSPM with an arbitrary tie-breaking rule and eligible sets $R_i$ for each agent $i$.
Let this mechanism $M'$.
% Given $\omb$, let $f$ be the winner under the MSPM and suppose that agent $i$ owns $f$.
% Then, it is straightforward to check that $\sigma_i = f$ and $\sigma_j = \perp$ is an equilibrium strategy.
% Hence, there exists at least one equilibrium.
Let $\sigma'$ be arbitrary equilibrium strategies under $M'$.
Let $\om_{M'}$ be the winner of $M'$.
% Consider Pareto-optimal strategies $\sigma'$
%  in $M'$, i.e. if an agent has two solutions $\om$ and $\om'$ such that $x(\om ) \ge x(\om')$, $y(\om) \ge y(\om')$ and at least one of these inequalities are strict, then the agent does not play strategy $\sigma_i = \om'$.
We now consider two cases (i) when $\om_{M'} \in \omb_i$ and (ii) $\om_{M'} \in \omb_j$ for some $j \neq i$.

Firstly, assume that $\om_{M'}$ belongs to agent $i$.
This means that $\sigma'_i = \om_{M'}$.
Since $\sigma'_i$ is an equilibrium strategy, there exists no solution $\om' \in \omb \setminus \omb_i$ such that $x(\om')>x(\sigma'_i)$ since if so, the agent who owns $\om$ will be selected in $M'$ by playing $\om'$ which contradicts that $\sigma'_i$ is an equilibrium strategy.
Hence, we have $x(\sigma'_i) \ge x(\om')$ for any $\om' \in \omb \setminus \omb_i$.
By~\eqref{ineq:12051650}, this implies that $y_i(\om_M) \ge y_i(\sigma'_i) = y_i(\om_{M'})$.
By our assumption of Pareto optimal play, we further have
\begin{align*}
	x(\sigma'_i) = x(\om_{M'})  \ge x(\om_M).
\end{align*}

Otherwise, suppose that $\om_{M'}$ belongs to agent $j \neq i$.
In this case, suppose that $x(\om_{M'}) < x(\om_{M})$.
Then, agent $i$ is strictly better off by playing $\om_M$.
Hence, this is not equilibrium, and it completes the proof.
% In this case, due to \eqref{ineq:12051649}, if $\sigma'_i \neq \om_M$, agent $i$  is strictly better off by playing $\om_M$.
% Hence we have $\sigma'_i = \om_M$.
% If $x(\om_M) > x(\om_{M'})$, then $M'$ does not select $\om_{M'}$ since $M'$ selects the best solution in terms of the principal's utility.
% Hence, we have $x(\om_{M'}) \ge x(\om_M)$.
% Since the above two cases hold for any $\om_{M'} \in F_{M',\sigma'}(\omb)$ and we consider any $\om_M \in F_{M,\sigma}(\omb)$, we finish the proof.
\end{proof}

\subsection{Proof of Theorem \ref{theorem:multi-agent-unlimited-budget}}\label{pf_theorem:multi-agent-unlimited-budget}

\begin{proof}
We mainly prove that
the expected payoff of randomized single-proposal mechanism $M$
is at least
$$\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.$$

We find a lower bound on the principal's utility in an arbitrary Nash equilibrium. 
%We consider two cases based on whether there exist eligible solutions or not.
Let $\omb = \cup_{i \in [n]}\omb_i$ be the entire set of solutions observed by the agents and $\sigma = (\sigma_1,\ldots, \sigma_n)$ be arbitrary Nash equilibrium.
We separately consider two cases (i) for any $\om \in \omb$, $\om \notin R$ and (ii) there exists $\om \in \omb$ such that $\om \in R$.

{\em Case (i).} 
% \note{In general $R_i$, version, we can similarly argue this case to be $\om \notin R_i$ for any $\om \in \omb_i$?.}
In this case, the utility of all agents is $0$,
and there does not exist a winner. 
Recall that for any Nash equilibrium,
there exists no incentive for any agent to deviate from equilibrium strategies.
We claim that $X_{(1)} < \tau$, where it concludes that the principal's utility is simply zero in this case.
Suppose not, \ie $X_{(1)} \geq \tau$. 
Denote by $\om^*$ one of the candidates which
corresponds to the utility of $X_{(1)}$, and observed by agent $t$.
If agent $t$ proposes $\om^*$, his utility strictly increases from $0$ to $y(\om^*)$,
which contradicts that the agents have played equilibrium strategies.
Hence we conclude that $X_{(1)} < \tau$, and the principal's utility is $0$.

{\em Case (ii).} 
We assume that agents play mixed strategies, \ie
they decide on a probability distribution over the observed solutions.
Formally, let $p_{i, j}$ be the probability that agent $i$ proposes $\omega_{i, j}$.
These probability distributions form a mixed Nash equilibrium.
As agents play mixed strategies, for each $i \in \left[n\right]$ we have $\sum_{j=1}^{k_i} p_{i, j} = 1$.
Define $S_i = \{\omega_{i, j}: p_{i, j} > 0\}$.
For each agent $i$, let $b_i$ be his worst candidate in terms of principal utility, \ie
$b_i = \argmin_{\omega \in S_i}x(\omega)$.
If there are multiple candidates with the worst utility, arbitrarily choose one.
We now proceed with the following claim.
\begin{claim}
    Denote the set of agents who have non-zero utility by $A$, then $|A| = 1$.
\end{claim}
\begin{proof}[Proof of the claim]
    Suppose not.
% Let $t \in A$ be the agent with the worst $b_t$, and least preferred by mechanism among ties.
Let $t$ be an agent $t \in A$ such that for each agent $i \in A-\{t\}$, either
\begin{itemize}
	\item $x(b_t) < x(b_i)$
	\item $x(b_t) = x(b_i)$, and principal prefers agent $i$ over agent $t$ using tie-breaking rule $\rho$,
\end{itemize}
\ie $t$ is the agent with the worst $b_t$ who is least preferred according to the tie-breaking rule.
Since agent $t \in A$ has non-zero utility and $b_t \in S_t$, proposing $b_t$ also gives a non-zero utility to agent $t$.
Let $\omega_{i, j} \in S_i$ be the proposed candidate by arbitrary agent $i \in A-\{t\}$.
This is because if there exists a solution with zero utility in $S_t$, then just removing $b_t$ from $S_t$ and distributing its assigned probability arbitrarily to other solutions will give a strictly higher utility for agent $t$.
For any $i \in A \setminus \{t\}$ and $\om_{i,j} \in S_i$, we observe that $x(\omega_{i, j}) \geq x(b_i)$.
In addition, we have either $x(b_t) < x(\omega_{i, j})$,
or $x(b_t) = x(b_i) = x(\omega_{i, j})$.
Since the principal prefers $i$ over $t$ according to the tie-breaking rule $\rho$, the candidate proposed by agent $t$, \ie $b_t$, is dominated by the candidate proposed by agent $i$, \ie $\omega_{i, j}$.
This implies that the principal never selects $b_t$ as the winner, and it contradicts the fact that agent $t$ has non-zero utility when proposing $b_t$.
Therefore, we can conclude that $|A| = 1$.
\end{proof}


Suppose that agent $i^* \in A$ is the only agent with non-zero utility.
In this case, all agents except agent $i^*$ have a utility of zero. 
% Due to the definition of Nash equilibrium, for any agent $i \neq i^*$, there is no incentive for the agent to propose his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$. 
Due to the definition of Nash equilibrium, for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y_i(f_{M,(\sigma_i,\sigma_{-i})}) = 0$.
%\suho{I understand these sentences, but it would be more formal if we can mathematically represent them, not by english. For example in the above sentence, we can say that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y(\sigma_i) = 0$. I think the reason that Mohammad commented on our previous version to be less formal is that it argues too much with words.}
% Since the agents are playing equilibrium strategies $\sigma$,
% the winner should not be changed with respect to agent $i$'s strategy.
This means that the principal never selects $\om \in \omb_i$ for agent $i \neq i^*$.
Hence, for all $i \neq i^*, \omega_{i^*, j} \in S_{i^*}$,  we have
\begin{align*}
    x(\omega_{i^*, j}) \geq \max_{\om \in \omb_i} x(\om) = X_{i, (1)}
\end{align*}
%
%As a result, if he proposes his best-observed solution, that solution is not selected as the winner, which shows that the current winner gives a higher utility to the principal, i.e. $x(c^*) \geq X_{i, (1)}$. 
%\suho{same as above}
%>>>>>>> Stashed changes
Furthermore, for all $\omega_{i^*, j} \in S_{i^*}$ we have $x(\omega_{i^*, j}) \leq X_{i^*, (1)}$.
Since for $n-1$ agents $i$ ($i \neq i^*$) we have $X_{i, (1)} \leq x(\omega_{i^*, j})$, and $x(\omega_{i^*, j}) \leq X_{i^*, (1)}$
using the definition of $X_{(r)}$, for all $\omega_{i^*, j} \in S_{i^*}$ we get
$$
X_{(n)} \leq X_{(n-1)} \leq ... \leq X_{(2)} \leq x(\omega_{i^*, j}) \leq X_{(1)}.
$$
Also, in this case, all candidates in $S_{i^*}$ should be eligible as they give non-zero utility to agent $i^*$.
% \note{Argue that, if not, by removing the candidate with zero utility, agent can get higher utility?}
This further implies that for all $\omega_{i^*, j} \in S_{i^*}$, $\tau \leq x(\omega_{i^*, j}) \leq X_{(1)}$, and we have
$$\max\left(X_{(2)}, \tau\right) \leq x(\omega_{i^*, j}) \leq X_{(1)}.$$
% \note{In general $R_i$ version, if $X_{(2)} \in R_{(2)}$, then bound by $X_{(2)}$. If $X_{(2)} \notin R_{(2)}$ but $X_{(1)} \in R_{(1)}$, then bound by $x$ of the solution that maximizes $(1)$'s utility $y()$ (due to pareto optimal play). Maybe we need a notation for those solutions.}
This inequality shows that
\begin{itemize}
    \item if $X_{(2)} \geq \tau$ then $x(\omega_{i^*, j}) \geq X_{(2)}$.
	Hence, in this case, the principal's expected utility is at least $X_{(2)}$ as
	$\Ex{f_{M, \sigma}(\omb)} = \sum_{j\in [k_{i^*}], \om_{i^*,j} \in S_{i^*}} p_{i^*, j} x(\omega_{i^*, j}) \geq \sum_{j\in [k_{i^*}], \om_{i^*,j} \in S_{i^*}} p_{i^*, j} X_{(2)} = X_{(2)}$.
    \item if $X_{(1)} \geq \tau \geq X_{(2)}$ then $x(\omega_{i^*, j}) \geq \tau$.
	Hence, in this case, the principal's expected utility is at least $\tau$ as
	$\Ex{f_{M, \sigma}(\omb)} = \sum_{j\in [k_{i^*}], \om_{i^*,j} \in S_{i^*}} p_{i^*, j} x(\omega_{i^*, j}) \geq \sum_{j\in [k_{i^*}], \om_{i^*,j} \in S_{i^*}} p_{i^*, j} \tau = \tau$.
\end{itemize}

Therefore, by combining the results of case (i) and case (ii) the expected utility of the principal is at least
\begin{align}
	\Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
	\Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.\label{ineq:infbud_tau}
\end{align}


% The proof mainly follows from the following lemma.


% \begin{lemma}
% In multi-agent setting with unlimited budget, the payoff of randomized single-proposal mechanism $M$ is at least $\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}$.
% \begin{proof}[Proof Sketch of Lemma]
% Since there is an unlimited budget for examination, we can assume that the principal takes the best candidate with respect to her own utility.
% There are two cases here:
% \begin{itemize}
%     \item If the best candidate does not satisfy the principal requirements, i.e. none of the proposed candidates are in eligible set $T_\tau$, i.e. $X_{\max} < \tau$; then the principal utility will be $0$.
%     \item If there is at least one candidate which satisfies the principal requirements; then we have $f_{M, \sigma}(\omb) = \argmax_i x(\sigma_i(\om_i))$. If $i^*$ is the agent who owns the winner, then all other agents have a utility of $0$. Consider a Nash equilibrium case where the utility of agents does not increase if they change their candidates (i.e. $\sigma_i(\om_i)$). Since the utility of all agents except agent $i^*$ is $0$, it implies that other agents do not have any strategies to get a positive utility. Since we are considering a Nash equilibrium, if agent $i \left(i \neq i^*\right)$ proposes his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$, then he still gets utility of $0$, which implies that the winner selected by the principal has utility at least $\max_{i \neq i^*} X_{i, (1)}$.
% Therefore, we can conclude that $i^*$ is the agent whose rank is $1$, thus what he proposes should give the principal higher utility than the best proposal of other agents:
% $$
% x(\sigma_{i^*}(\om_{i^*})) \geq X_{(2)} \geq X_{(3)} \geq ... \geq X_{(n)}.
% $$
% Also, if $X_{(2)} < \tau$ then we can have a better bound on the winner since $\sigma_{i^*}(\om_{i^*})$ is eligible then $x(\sigma_{i^*}(\om_{i^*}) \geq \tau$ thus in this case we have:
% $$
% x(\sigma_{i^*}(\om_{i^*})) \geq \tau > X_{(2)} \geq X_{(3)} \geq ... \geq X_{(n)}.
% $$
% \end{itemize}

% Therefore, we can conclude that the utility is bounded by 
% $$
% \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
% \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}
% $$
% \end{proof}
% \end{lemma}
\end{proof}


\subsection{Proof of Theorem \ref{thm:recover}}\label{pf_thm:recover}
\begin{proof}
%	By Theorem 4 of \citet{kleinberg2018delegated}, there exist corresponding SPMs under the single-agent setting such that the three results presented in the theorem statement hold.
%	Hence, it suffices to show that for each case, there exists an MSPM under the multi-agent setting which outperforms the SPM under the single-agent setting.
%	To this end, we will show that for each agent $i$, we can define a proper eligible set $R_i$ so that the principal's expected utility from agent $i$'s candidate satisfies the guarantees provided in \citet{kleinberg2018delegated}.
%	That is, under the MSPM with proper eligible sets, we will show that for each agent's candidate $\sigma_i$ satisfy $\Ex{x(\om_i)} \ge \rho \Ex{X_{i,(1)}}$ for each one of three cases presented in the theorem statement where $\rho$ refers to the corresponding approximation ratio.
	Given the multi-agent delegation problem, we construct a single-agent instance and
    then use guarantees on the single-agent setting to prove our theorem. 
    Consider a problem instance of multi-agent delegation where $n$ agents propose solutions.
	In order to find solutions, agent $i$ samples a solution from each of his $k_i$ distributions $\{D_{i, j}\}_{j=1}^{k_i}$.
    Note that all solutions lie in $\Omega$.
	We construct a single-agent problem instance
	where we denote the only agent by $s$.
    In the single-agent instance, for all $i \in [n]$, agent $s$ samples $k_i$ solutions,
    one from each of distributions $\{D_{i, j}\}_{j=1}^{k_i}$,
    hence $\sum_{i=1}^{n} k_i$ samples on aggregate.
    
    Let $\om$ be a solution that agent $s$ observes from the distributions that belong to agent $i$.
    We represent this solution in single-agent instance with a pair $\left(\om, i\right)$.
    Importantly, we define the solution space $\Omega'$ in single-agent instance by $\Omega' := \Omega \times \left[n\right]$.
    In the constructed instance, the principal's utility of the solutions, \ie the function $x(.)$, does not change.
    Precisely, $x(\left(\omega, i)\right) := x(\omega)$.
    However, we define $y(\left(\omega, i)\right)$, \ie
    agent $s$ utility for $\om$ when observed by distributions of agent $i$, to be $y(\left(\omega, i)\right) := y_i(\om)$.
 
	According to \citet{kleinberg2018delegated}, there exists an SPM with proper eligible set $R$ under the constructed instance such that
	principal's expected utility is at least $\frac{1}{2}\Ex{X_{(1)}}$.
	We use eligible sets $R_i = R$ for all agents in the multi-agent instance.
	We claim that for any realization of solutions $\omb = \cup_{i=1}^{n} \omb_i$,
	the principal's utility in the multi-agent setting is at least that of the single-agent setting.
    This further implies that
	using eligible sets $R_i = R$, principal's expected utility in multi-agent settings is at least $\frac{1}{2}\Ex{X_{(1)}}$.
	
	Consider a realization of solutions $\omb$. Let $(\omega, i)$ be the winner in the single-agent setting.
	If $(\omega, i) = \perp$, then all observed solutions are not eligible.
	Formally, for all $i$ in $\left[n\right]$, and $j$ in $\left[k_{i}\right]$:
	$\omega_{i, j} \notin R$. In this case, there is no eligible solution in the multi-agent setting which
	indicates that the principal's utility in both settings is zero.
	
    On the other hand, if $(\omega, i) \neq \perp$, let $\omega^*$ be the winner in the multi-agent instance, we claim that $x(\omega^*) \geq x(\omega)$.
	Note that $(\omega, i)$ is the winner of the single-agent instance so $\om$ is the eligible solution that
    maximizes agent $s$ utility by giving her the utility of $y\left((\om, i)\right) = y_i(\om)$.
 
    Denote by $\sigma_i$ the solution proposed by agent $i$ in the multi-agent instance. 
    As both $\sigma_i, \omega \in R$, and $\omega$ is the eligible solution that maximizes $y_i$, then 
	$y_i(\omega) \geq y_i(\sigma_i)$.
    As a result, according to Assumption~\ref{as:pareto}, $x(\sigma_i) \geq x(\omega)$.
	There are two cases

	\begin{itemize}
		\item
		$\omega^*$ is sampled by $i$, \ie $\omega^* = \sigma_i$. As shown above $x(\omega^*) = x(\sigma_i) \geq x(\omega)$.
		\item
		$\omega^*$ is sampled by another agent $j \neq i$.
		As the principal selects the best candidates among all agents, $x(\omega^*) \geq x(\sigma_i)$.
		Using the inequality $x(\sigma_i) \geq x(\omega)$ we further conclude that $x(\omega^*) \geq x(\omega)$.
	\end{itemize}

	This finishes the proof.

        Finally, consider a correspondence between the multi-agent and single-agent setting such that the entire solutions in the multi-agent setting is sampled by the agent in the single-agent setting (as we did in the proof).
        Then, our proof in fact shows that the multi-agent problem can always bring higher (or equal) principal's utility than the single-agent problem equipped with any possible mechanism without money.
        This is because any mechanism in the single-agent setting can be reduced to the single-proposal mechanism by Lemma 1 in \citet{kleinberg2018delegated}, and we prove that our construction of the mechanism above yields a higher (or equal) utility for the principal than the single-proposal mechanism in the single-agent setting.

	% OLD PROOF
	% \todo{Rewrite the entire proof}
	% First, we focus on proving (1) and we will argue that the proof naturally transfers to the other settings as well.
	% Consider a problem instance of the multi-agent setting.
	% Restrict our attention to agent $i$, and consider a corresponding problem instance of the single-agent setting so that it is equivalent to the problem instance in which the principal delegates to only agent $i$ in the multi-agent setting.
	% Then, by \citet{kleinberg2018delegated}, there exists an SPM under the constructed single-agent setting such that the principal's expected utility is at least $\frac{1}{2}\Ex{X_{i,(1)}}$.
	% Denote this mechanism by $M'_i$ and let its eligible set be $R_i$.
	% We can define such $R_i$ for each agent $i \in [n]$.
	% Given the observed solution $\omb_i$ of agent $i$, let the agent's strategy be $\sigma'_i$ under the single-agent setting with $M_i'$.
	
	% Now, under the multi-agent setting, consider an MSPM with eligible sets $R_i$ and a deterministic tie-breaking rule $\rho$ with transitivity.
	% Suppose that the solutions are realized to be $\omb = (\omb_1, \ldots, \omb_n)$.
	% Let agent $i$'s strategy be $\sigma_i$ for $i \in [n]$ given the observed solutions.
	% Define $i^*$ the agent w.r.t. the tie-breaking rule with best candidate $\om^*$ such that $x(\om^*) \ge x(\om)$ for any $\om \in \omb$.
	% If there are multiple agents with the highest $x(\om)$, then choose the one that is the most preferred by the tie-breaking rule $\rho$.
	% Note that we can always specify such a single agent due to the transitivity of deterministic $\rho$.
	% Due to the arguments observed in the proof of Theorem~\ref{theorem:multi-agent-unlimited-budget}, we have $x(\sigma_i) \ge X_{i,(1)}$ for $i \neq i^*$.
	% For $i^*$, its strategy $\sigma_{i^*}$ satisfies (1) $\sigma_{i^*} \in R_{i^*}$ and $y(\sigma_{i^*}) \ge y(\om')$ for any $\om' \in \omb_{i^*}$.
	% Overall, this concludes that $x(\sigma_i) \ge x(\sigma'_i)$ for any $i \in [n]$ and for any $\omb_i \in \Omega^{k_i}$, given the other agents' observed solutions $\omb_{-i}$.
	% Fix an agent $i$ and its observed solution $\omb_i$, by marginalizing over the randomness of $\omb_{-i}$, we have
	% \begin{align*}
	% 	\Exu{\omb}{x(\sigma_i)}
	% 	= 
	% 	\Exu{\omb_i}{\Exu{\omb_{-i}}{x(\sigma_i)\given \omb_{-i}}}
	% 	\ge \Exu{\omb_i}{x(\sigma'_i)} \ge \frac{1}{2}\Ex{X_{i,(1)}}.
	% \end{align*}
	% Since $M$ selects the final candidate that maximizes the principal's utility, we conclude that the principal's expected utility is at least
	% \begin{align*}
	% 	\Exu{\omb}{\max_{i \in [n]}x(\sigma_i)} \ge \frac{1}{2}\Ex{\max_{i \in [n]}X_{i,(1)}} = \frac{1}{2}\Ex{X_{\max}},
	% \end{align*}
	% and this implies that our mechanism is $(2,0)$-approximate mechanism.
	% Since we can argue similarly for cases (2) and (3), we finish the proof.
\end{proof}

\subsection{Proof of Theorem \ref{thm:lowerbound_comp_worst}}\label{pf_thm:lowerbound_comp_worst}
\begin{proof}
	Consider a multi-agent instance where $n$ agents propose solutions.
	If there exists an agent whose sampled solutions are always better than others agents' solutions,
	we call that agent a~\emph{super}~agent. Formally, we say that agent $i$ is super~agent
	if for each $j \in \left[k_i\right]$, each $i' \in \left[n\right] \setminus \{i\}$,
	and each $j' \in \left[k_{i'}\right]$ when $\omega_{i, j} \sim D_{i, j}, \omega_{i', j'} \sim D_{i', j'}$
	we have $x(\omega_{i, j}) \geq x(\omega_{i', j'})$.

	When a multi-agent delegation problem instance has a super agent,
	then whatever the super agent proposes is taken as the winner as all other agents' proposed solutions
    are dominated by any solution of the super agent.
	As a result, the multi-agent instance reduces to a single-agent instance where
	only agent $i$ exists as the single agent.

	We now show that $(2,0)$-approximation is tight for Bayesian mechanisms.
	We use the notion of a super agent and construct a multi-agent delegation problem where
	there exists a super agent so that only his sampled solutions are important.
	We note that $X_{(1)}$ here corresponds to the solution observed by the super agent as other agents will never sample the best solution.

	Assume this agent samples two solutions from distributions $D_1$, and $D_2$.
    \begin{itemize}
        \item 
        $D_1$ always gives the same solution $\omega_1$ to the agent such that $x(\omega_1) = 1, y(\omega_1) = 10$.
        \item 
        $D_2$ gives the agent solution $\omega_{21}$ such that $x(\omega_{21}) = \frac{1}{\alpha}, y(\omega_{21}) = 5$
    	with probability of $\alpha$ while with probability of $1-\alpha$,
    	it gives solution $\omega_{22}$ to the agent such that $x(\omega_{22}) = \frac{\alpha}{1-\alpha}, y(\omega_{22}) = 5$.
        Note that $\alpha$ is a very small positive number.
    \end{itemize}
	There are two possibilities for sampled solutions by this agent
	either it is $\{\omega_{1}, \omega_{21}\}$, or it is $\{\omega_{1}, \omega_{22}\}$.
	We first consider $\Ex{X_{(1)}}$
	\begin{align*}
		\Ex{X_{(1)}} = \alpha \parans{\frac{1}{\alpha}} + \parans{1 - \alpha}\parans{1} = 2-\alpha.
	\end{align*}
	
	Now we consider the principal's policy. There are two cases
	\begin{itemize}
		\item
		principal accepts $\omega_{1}$, \ie $\omega_{1} \in R$ then as $y(\omega_{1}) > y(\omega_{21}) = y(\omega_{22})$,
		agent proposes $\omega_{1}$ no matter what he samples from $D_2$. In this case, the principal's utility is $1$.
		\item
		principal rejects $\omega_{1}$, \ie $\omega_{1} \notin R$. In this case, the principal accepts the other solution as it gives a non-zero utility to her.
		With probability of $\alpha$, $\omega_{21}$ is sampled by the agent which gives the utility of $\frac{1}{\alpha}$ to the principal,
		however, $\omega_{22}$ is sampled with probability of $1-\alpha$ which gives the utility of $\frac{\alpha}{1-\alpha}$ to the principal.
		Therefore, prinicpal's expected utility using this policy is $\alpha \parans{\frac{1}{\alpha}} + \parans{1-\alpha}\parans{\frac{\alpha}{1-\alpha}}= 1 + \alpha$.
	\end{itemize}
        % \suho{multiplicative approximation factor!}
	Denote by $ALG$ the principal's utility using her policy. In both cases, the principal's expected utility $\Ex{ALG} \le 1 + \alpha$. By putting $\alpha := \frac{\eps}{3-\eps}$, we have
	\begin{align*}
		(2-\eps)\Ex{ALG} \le (2-\eps)(1 + \alpha) =
        (2-\eps)\left(1 + \frac{\epsilon}{3-\epsilon}\right) = 2 - \frac{\eps}{3-\eps} = 2 - \alpha = \Ex{X_{(1)}}.
	\end{align*}
    Therefore, $(2-\eps)\Ex{ALG} \le \Ex{X_{(1)}}$. This indicates that the multiplicative approximation factor is at least $2-\eps$, which finishes the proof.
\end{proof}

\subsection{Proof of Theorem \ref{thm:informed}}\label{pf_thm:informed}
\begin{proof}
	Define $R_i = R = \{\om : x(\om) \ge r(n,k)\}$.
	Suppose that we run MSPM with the eligible set $R$.
	Due to Theorem~\ref{theorem:multi-agent-unlimited-budget}, the principal's expected utility is at least
	\begin{align}
		\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau \IND[X_{(1)} \ge \tau > X_{(2)}]}
		&\ge
		\Ex{\tau \IND[X_{(1)} \ge \tau]}
		\\
		&\ge
		\Pr{\exists i : X_{i,(1)} \ge r(n,k)}r(n,k)
		\nonumber
		\\
		&=
		\parans{1 - F(r(n,k))^{nk}}r(n,k)
		\nonumber
		\\
		&\ge
		\parans{1 - \parans{r(n,k)^{\alpha}}^{nk}}r(n,k)
		\nonumber
		\\
		&=
		r(n,k) - r(n,k)^{\alpha nk+1},
		\label{ineq:01041212}
	\end{align}
	where the second inequality comes from our assumption on $F(x) \le x^{\alpha}$.
	Plugging $r(n,k) = \parans{\frac{1}{\alpha nk + 1}}^{\frac{1}{\alpha nk}}$,\footnote{Note that this choice of $r(n,k)$ comes from derivating \eqref{ineq:01041212} w.r.t. $r(n,k)$ by considering it as a function of $\alpha nk$.} we can further obtain
	\begin{align*}
		\parans{\frac{\alpha nk}{\alpha nk +1}}^{\frac{1}{\alpha nk}},
	\end{align*}
	which yields the multiplicative approximation ratio of $\parans{\frac{\alpha nk}{\alpha nk +1}}^{\frac{-1}{\alpha nk}}$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:comp_obl_neg}}\label{pf_thm:comp_obl_neg}
\begin{proof}
        % \suho{I think we also need to borrow the MSPM reduction result in here as well. I don't even remember what I mean by this...}
        In order to prove this theorem,
	we reuse the idea of super agent defined in the proof of   Theorem~\ref{thm:lowerbound_comp_worst}.
        Before that, we claim that the principal cannot announce an eligible set other than $\Omega$.
        The proof is based on straightforward arguments but we provide it to make it self-contained.
        \begin{claim}\label{cl:3}
            If $R_i \neq \Omega$ for some $i \in [n]$, then the additive price of anarchy can be arbitrarily close to $L$, \ie for any $\eps>0$ there exists a problem instance such that $\pos_a \ge L - \eps$.
        \end{claim}
        \begin{proof}[Proof of the claim]
            Since $R_i \neq \Omega$, there must be an element $\om \in \Omega$ such that the principal does not admit.
            Assume that $x(\om) = L-\eps/2$, and agent $i$'s distribution is a point mass on $\om$.
            Further, assume that other agents $j \neq i$ have distributions such that the principal's utility is at most $\eps/2$ for any point in their support.
            Then, our MSPM with the given eligible sets only accepts some solutions from $j \neq i$, which results in the principal's utility of at most $\eps/2$.
            Meanwhile, the optimal utility will be to select agent $i$'s solution $\om$ under which the principal can obtain $L-\eps$.
            Hence, the additive approximation factor is $L-\eps/2 - \eps/2 = L-\eps$, and it completes the proof.
        \end{proof}
        Due to the claim above, the principal should announce no eligible set in order to derive a nontrivial approximation ratio.
	Consider a multi-agent instance such that there exists a super agent. 
	Because the principal does not have any information regarding the distribution of agents,
	she cannot announce any eligible sets
	% \keivan{is it true? if so, we should emphasize on this fact in the definition of oblivious case}\suho{see claim}
	which implies that she accepts all solutions
	and takes the best one among the proposed solutions. 
	As a result, whatever the super agent proposes is selected by the principal.
	Assume the super agent samples two solutions from distributions $D_1$ and $D_2$.
	$D_1$ always gives the same solution $\omega_1$ to the agent such that $x(\omega_1) = L - \eps/2, y(\omega_1) = 5$.
	$D_2$ always gives the agent solution $\omega_{2}$ such that $x(\omega_{2}) = \eps/2, y(\omega_{2}) = 10$.
	We obtain
	\begin{align*}
		\Ex{X_{(1)}} = \Ex{\max\{\eps/2, L - \eps/2\}} = L -\eps/2.
	\end{align*}
	The super agent proposes $\omega_2$ as it will not be rejected by the principal
	and gives a higher utility to him, which means that the principal's utility is $x(\omega_2) = \eps/2$.
	Therefore, the additive approximation factor of this mechanism is $\Ex{X_{(1)}} - x(\omega_2) = L-\eps$. This finishes the proof.
\end{proof}

\subsection{Proof of Theorem \ref{thm:comp_sym_general}}\label{pf_thm:comp_sym_general}
\begin{proof}
        For ease of presentation, assume that $L=1$.
	By our assumption on symmetry and since each agent independently samples solutions, $X_{i,(1)}$ for $i \in [n]$ are identical and independent.
	Then, the result directly follows from the following theorem.
	\begin{lemma}[\citet{lopez2011upper}]\label{lm:lopez}
		Let $X_1,\ldots, X_n$ be i.i.d. random variables supported on $[0,1]$. Given an integer $s$ such that $1 \le s \le n-1$, let $Y_s$ and $Y_{s+1}$ be $s$-th and $s+1$-th order statistics of $X_1,\ldots, X_n$. Then, the following holds.
		\begin{align*}
			\Ex{Y_{s+1} - Y_s} \le \binom{n}{s}\left(\frac{s}{n}\right)^s \left(1-\frac{s}{n}\right)^{n-s}.
		\end{align*}
	\end{lemma}
	Plugging $s = n-1$ yields the desired result for $L=1$.
    By scaling the random variables, we can easily obtain the general of upper bound $L(1-\nicefrac{1}{n})^{n-1}$.

    To prove that this upper bound is tight upper bound for $\Ex{X_{(1)} - X_{(2)}}$, consider a symmetric problem instance equipped with a Bernoulli distribution with parameter $p$, \ie $X_{i,j} \sim \text{Bernoulli}(p)$.
	In this case, $X_{i,(1)}$ is also a Bernoulli distribution with parameter $q = 1-(1-p)^k$.
	Furthermore, we have
	\begin{align*}
		\Ex{X_{(1)} - X_{(2)}}
		&=
            \binom{n}{n-1}(1-q)^{n-1}q.
	\end{align*}
	If we set $q = 1-(1-p)^k = \frac{1}{n}$, which is equivalent to $p = 1 - (1-1/n)^{1/k}$, then we have the tight bound of $(1-1/n)^{n-1}$.
    By scaling this problem instance, we finish the proof.

    % To obtain the tightness, suppose that $X_{i,j}$ is r.v. such that $X_{i,j}= L - \eps/2$ with probability $p>0$ and is $\eps/2$ otherwise, for $i \in [n]$ and $j \in [k_i]$.
    % Denote the former solution (with $X_{i,j}=L-\eps/2$) by type 1, and the latter by type 2.
    % Consider arbitrary mechanism $M$.
    % Given $M$, define $q_i$ be the probability that agent $i$ is selected when all the agents submit type 2 solution.
    % Let $A$ be the set of agents satisfying $q_i > 0$.
    % Assume that the utility of the principal and the agent is correlated so that if $X_{i,j} =L - \eps/2$ then $Y_{i,j} = \delta q + \delta$ and if $X_{i,j} = \eps/2$ then $Y_{i,j} = 1$, where $\delta$ is sufficiently small quantity will be defined later.
    % Define $A_i$ be the event of agent $i$'s solutions $\omb_i$ such that all the solutions are type 2.
    % Let $B_i$ be the event of agent $i$'s solutions $\omb_i$ in which there exists $j_1$ and $j_2$ such that $j_1$ is type 1 solution and $j_2$ is type 2 solution for $j_1 \neq j_2 \in [k_i]$.

    % Consider the following event for $i \in [n]$,
    % \begin{align*}
    %     E_i = \paranm{\omb_i: \{\omb_i \in B_i \} \cap \{\omb_{i'} \in A_{i'} \forall i' \neq i, i' \in [n]\}}.
    % \end{align*}
    % Further define $F = \cup_{i\in A}E_i$.
    % % Further define $F_i$ for $i \in [n]$ as follows.
    % % \begin{align*}
    % %     F_i = \paranm{\omb_i: X_{i,j} = \eps/2, \forall j \in [k_i]}.
    % % \end{align*}
    % % % Finally define $G = \cup_{i \in [n]} G_i$.
    % % % If $G$ happens, $X_{\max} = 1$ due to agent $i$ with $E_i$.
    % Denote the principal's expected utility under the mechanism $M$ by $X_M$.
    % \begin{claim}
    %     $X_{(1)} - X_M \neq 0$ if and only if $F$ happens.
    % \end{claim}
    % \begin{proof}
    %     Suppose that $X_{(1)} - X_M \neq 0$.
    %     Then, this quantity can be only $L - \eps/2 - \eps/2 = L-\eps$.
    %     This implies that some agents sample at least one type 1 solution, but everyone proposes type 2 solutions.
    %     In order for this to be happened, there must be only one agent who samples type 1 solution.
    %     This is true because otherwise, both agents will submit type 1 solutions.
    %     Moreover, this unique agent with type 1 solution also needs to sample at least one type 2 solution, as all the agents propose type 2 solutions.
    %     This concludes that this event of $X_{(1)} - X_M \neq 0$ implies $F$.

    %     Now suppose that $F$ happens.
    %     As $E_i$ are disjoint for $i \in A$, there exists $s \in A$ such that $E_s$ happens.
    %     Then, $X_{\max} = L-\eps/2$ since agent $i$ has both the type 1 and 2 solutions.
    %     By proposing type 1 solution, agent $s$ gets $\delta q_s + \delta$.
    %     On the other hand, if he submits type 2 solution, due to the tie-breaking rule, he gets $q_s \cdot 1 > 0.5q_s > \delta q_s + \delta$ (we can take arbitrarily small $\delta$ to make it true).
    %     Hence, agent $s$'s best-response is to submit type 2 solution.
    %     This means that the principal's utility under the mechanism is $\eps/2$, while $X_{\max} = L-\eps/2$. This finishes the proof.
    % \end{proof}
    
    % Now we compute the probability that the event $Es$ happens.
    % By independence of the solution finding process, we obtain
    % \begin{align*}
    %     \Pr{E_s} := f(n) = \parans{1 - (p^k + (1-p)^k)} \cdot \parans{(1-p)^k)^{n-1}},
    % \end{align*}
    % which further implies $\Pr{F} = Af(n)$.
    % Hence, we have
    % \begin{align*}
    %     \Ex{X_{(1)} - X_M} = (L-\eps)Af(n)
    % \end{align*}
    
    
\end{proof}

\subsection{Proof of Lemma \ref{lm:order_stat_diff}}\label{pf_lm:order_stat_diff}
\begin{proof}
		We separately prove two statements using similar techniques.
		Let $F$ and $f$ be the c.d.f. and p.d.f. of $D$, respectively.
		
		
		\paragraph{Part (1)}
		Rearranging $\Delta_{k,n} \le \Delta_{k,n-1}$, we need to show that
		\begin{align*}
			\Ex{X_{n-k+1:n} - X_{n-k:n-1}} \le \Ex{X_{n-k:n} - X_{n-k-1:n-1}}.
		\end{align*}
		Due to \citet{david1997augmented}, LHS and RHS can be represented as follows.
		\begin{align*}
			\Ex{X_{n-k+1:n} - X_{n-k:n-1}}
			&= 
			\binom{n-1}{n-k}\int_{-\infty}^{\infty}F^{n-k}(x)(1-F(x))^{k}dx.
			\\
			\Ex{X_{n-k:n} - X_{n-k-1:n-1}}
			&= 
			\binom{n-1}{n-k-1}\int_{-\infty}^{\infty}F^{n-k-1}(x)(1-F(x))^{k+1}dx.
		\end{align*}
		Plugging into the inequality and rearranging it, we need to show that
  
		\begin{align}
			\binom{n-1}{n-k-1}
			\parans{
			\int_{-\infty}^{\infty} F^{n-k-1}(x)(1-F(x))^k \left(\frac{n}{n-k}F(x) - 1\right)dx} \le 0.\label{ineq:12232248_new}
		\end{align}
		Define $G(t) = \int_{-\infty}^{t} F^{n-k-1}(x)(1-F(x))^{k-1} \left( \frac{n-1}{n-k}F(x) - 1\right)f(x)dx$.
		Obviously, $\frac{n-1}{n-k}F(x) - 1$ inside the integrand becomes positive for $x > x_0$ and negative otherwise for some $x_0 \in \R$.
		This implies that $G(t) \le G(\infty)$ for any $t \in \R$.
		Let $u = F(x)$ and by change of variables, we have
		\begin{align*}
			G(\infty)
			&=
			\int_{-\infty}^{\infty} u^{n-k-1}(1-u)^{k-1} \left( \frac{n}{n-k}u - 1\right)du
			\\
			&= 
			\frac{n}{n-k}B(n-k+1,k) - B(n-k,k)
			\\
			&=
			\frac{n}{n-k}\frac{(n-k)!(k-1)!}{n!} - \frac{(n-k-1)!(k-1)!}{(n-1)!}
			=0
		\end{align*}
		where $B(\cdot,\cdot)$ denotes the beta function.
		Hence, we have $G(t) \le 0$ for any $t \in \R$.
		Now we use the following lemma.
		\begin{lemma}[\citet{barlow1975statistical}]\label{lm:barlow}
			Given two functions $g:\R \mapsto [a,b]$ and $h:\R \mapsto [a,b]$ and $h$ is nonnegative, then the following holds.
			\begin{enumerate}
				\item If $\int_{-\infty}^t g(x)dx \le 0$ for any $t \in \R$, then for any nonincreasing function $h:\R \mapsto \R$, we have $\int_{-\infty}^t g(x)h(x)dx \le 0$ for any $t \in \R$.
				\item If $\int_{-\infty}^t g(x)dx \ge 0$ for any $t \in \R$, then for any nondecreasing function $h:\R \mapsto \R$, we have $\int_{-\infty}^t g(x)h(x)dx \ge 0$ for any $t \in \R$.
			\end{enumerate}
		\end{lemma}
		Plugging $g(x)$ to be the integrand of $G(x)$ and $h(x) = (\frac{f(x)}{1-F(x)})^{-1}$ to the first part of the above lemma, we conclude that ~\eqref{ineq:12232248_new} holds since $h(t)$ is nonincreasing due to the assumption on MHR.
		This completes the first part of the lemma.
		
		\paragraph{Part (2)}
		Now consider the MRHR distribution case.
		Rearranging $\delta_{k,n} \le \delta_{k,n-1}$, we need to show that
		\begin{align*}
			\Ex{X_{k+1:n} - X_{k+1:n-1}} \le \Ex{X_{k:n} - X_{k:n-1}}.	
		\end{align*}
		Again due to \cite{david1997augmented}, we have
		\begin{align*}
			\Ex{X_{k+1:n} - X_{k+1:n-1}}
			&=
			-\binom{n-1}{k}\int_{-\infty}^{\infty}F^{k+1}(x)(1-F(x))^{n-k-1}dx.
			\\
			\Ex{X_{k:n} - X_{k:n-1}}
			&=
			-\binom{n-1}{k-1}\int_{-\infty}^{\infty}F^{k}(x)(1-F(x))^{n-k}dx.	
		\end{align*}
		Plugging into the inequality and rearranging it, it suffices to show that
		\begin{align*}
			\frac{(n-1)!}{(k-1)!(n-k)!}\int_{-\infty}^{\infty}F^k(x)(1-F(x))^{n-k-1}\parans{\frac{n}{k}F(x) - 1}dx \ge 0.
		\end{align*}
		Define $G'(t) = \int_{t}^{\infty} F^{k-1}(x)(1-F(x))^{n-k-1}\parans{\frac{n}{k}F(x) - 1} f(x) dx$.
		Observe that $\parans{\frac{n}{k}}F(x) - 1$ becomes positive for $x > x_0$ and negative otherwise for some $x_0 \in \R$.
		Hence, $G'(t) \ge G'(-\infty)$.
		Now we show that $G'(-\infty) \ge 0$.
		Using change of variable with $F(x) = u$, we have
		\begin{align*}
			G'(-\infty)
			&=
			\int_{-\infty}^{\infty}u^{k-1}(1-u)^{n-k-1}\parans{\frac{n}{k}u - 1}du
			\\
			&=
			\frac{n}{k}B(k+1, n-k) - B(k, n-k)
			\\
			&=
			\frac{n}{k}\frac{k!(n-k-1)!}{n!} - \frac{(k-1)!(n-k-1)!}{(n-1)!}= 0,
		\end{align*}
		and it concludes that $G'(t) \ge 0$ for any $t \in \R$.
		Now, plugging $g(x)$ to be the integrand of $G'(x)$ and $h(x) = (\frac{f(x)}{F(x)})^{-1}$ to the second part of Lemma \ref{lm:barlow}, we conclude that ~\eqref{ineq:12232248_new} holds since $h(t)$ is nondecreasing due to the assumption on MRHR.
		This completes the first part of the lemma.

\end{proof}

\subsection{Proof of Lemma \ref{lm:mhr_preserving}}\label{pf_lm:mhr_preserving}
\begin{proof}
		Let $f(x)$ and $F(x)$ be p.d.f. and c.d.f. of the distribution $X_i \sim D$, and let $g(x)$ and $G(x)$ be that of $r$-th order statistics, respectively.
		Then, we have
		\begin{align*}
			1-G(x)
			&=
			\sum_{j=0}^{r-1}\binom{n}{j}F(x)^j(1-F(x))^{n-j}
			\\
			g(x)
			&=
			\frac{n!}{(r-1)!(n-r)!}f(x)F(x)^{r-1}(1-F(x))^{n-r}.
		\end{align*}
		Hence, its hazard rate can be obtained as
		\begin{align*}
			h(x)
			&=
			\frac{\frac{n!}{(r-1)!(n-r)!}f(x)F(x)^{r-1}(1-F(x))^{n-r}}{\sum_{j=0}^{r-1}\binom{n}{j}F(x)^j(1-F(x))^{n-j}}
			\\
			&= \frac{n!}{(r-1)!(n-r)!} \frac{f(x)}{1-F(x)}
			\frac{F(x)^{r-1}(1-F(x))^{n-r+1}}{\sum_{j=0}^{r-1}\binom{n}{j}F(x)^j(1-F(x))^{n-j}}
			\\
			&= \frac{n!}{(r-1)!(n-r)!} \frac{f(x)}{1-F(x)}
			\frac{1}{\sum_{j=0}^{r-1}\binom{n}{j}\left(\frac{1-F(x)}{F(x)}\right)^{r-j-1}}.
		\end{align*}
		Since $f(x)/(1-F(x))$ is nondecreasing by MHR property of $D$ and $1-F(x)/F(x)$ is nonincreasing function of $x$, we conclude that $h(x)$ is nondecreasing function of $x$.
\end{proof}

\subsection{Proof of Theorem \ref{thm:mhr_upperbound}}\label{pf_thm:mhr_upperbound}
\begin{proof}
	Recall that the additive approximation factor is upper bounded by $\Ex{X_{(1)} - X_{(2)}}$ by Corollary \ref{cor:infbud_notau}.
	As we discussed, the proof mainly follows from Lemma \ref{lm:order_stat_diff} on the expected difference between two consecutive order statistics.	
	First, by Lemma \ref{lm:mhr_preserving},  $X_{i,(1)}$ has MHR distribution for $i \in [n]$.
	Now, denote by $\Ex{X_{(1):n} - X_{(2):n}}$ the additive approximation factor in the problem setting when there exists $n$ agents.
	By repeating Lemma \ref{lm:order_stat_diff} with $k=1$, we can obtain the following inequalities.
	\begin{align*}
		\Ex{X_{(1):n} - X_{(2):n}} 
		\le
		\Ex{X_{(1):2} - X_{(2):2}}
		=
		\Ex{|A-B|},
	\end{align*}
	where $A$ and $B$ are two i.i.d. random variables of which the endowed distribution is equivalent to that of $X_{i, (1)}$.
	We now use the following inequality.\footnote{Weaker bound of $\Ex{|A-B|} \le \sqrt{\var(a)}$ can be obtained by simply rewriting it as $\Ex{\sqrt{(A-B)^2}}$ and applying Jensen's inequality.}
	\begin{lemma}[Theorem 5 in \cite{cerone2005bounds}]
		Let $A,B$ be i.i.d. random variables with mean $\mu$ and variance $\sigma^2$.
		For any $p,q$ such that $p>1$ and $\frac{1}{p} + \frac{1}{q} = 1$, suppose that $\Ex{|A - \mu|^{p}} < \infty$.
		Then, the following inequality holds.
		\begin{align*}
			\Ex{|A-B|} \le \frac{2}{(q+1)^{1/q}}\Ex{|A - \mu|^{p}}^{1/p}.
		\end{align*}
	\end{lemma}
	Plugging $p=q=2$ into the lemma, we obtain
	\begin{align*}
		\Ex{|A-B|} \le \sqrt{\frac{4\var(A)}{3}}.
	\end{align*}
	In case of uniform distribution $U[0,1]$, it is widely known that $X_{i,(1)} \sim Beta(k,1)$.
	Hence, we conclude that the additive approximation factor is bounded above by
	\begin{align*}
		\sqrt{\frac{4k}{3(k+1)^2(k+2)}} \approx \frac{1.155}{k}.
	\end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lm:order_stat_diff_restricted}}
\begin{proof}
		We separately prove two cases.
		
		\paragraph{Part (1)}
		Rearrange $(n+1)\Delta_{k,n} = \Delta_{k,n}  + n\Delta_{k,n} \le n\Delta_{k,n-1}$ and divide it by $n-1$,, we need to show that
		\begin{align*}
			\frac{\Delta_{k,n}}{n}  + \Ex{X_{n-k+1:n} - X_{n-k:n-1}} \le \Ex{X_{n-k:n} - X_{n-k-1:n-1}}.
		\end{align*}
		Again to \citet{david1997augmented}, each term can be represented as follows.
		\begin{align*}
			\frac{\Delta_{k,n}}{n}
			&=
			\frac{1}{n}\binom{n}{k}\int_{-\infty}^{\infty}F^{n-k}(x)(1-F(x))^{k} dx
			\\
			\Ex{X_{n-k+1:n} - X_{n-k:n-1}}
			&= 
			\binom{n-1}{n-k}\int_{-\infty}^{\infty}F^{n-k}(x)(1-F(x))^{k}dx.
			\\
			\Ex{X_{n-k:n} - X_{n-k-1:n-1}}
			&= 
			\binom{n-1}{n-k-1}\int_{-\infty}^{\infty}F^{n-k-1}(x)(1-F(x))^{k+1}dx.
		\end{align*}
		Plugging into the inequality and rearranging it, we need to show that
  
		\begin{align*}
			\binom{n-1}{n-k-1}
			\parans{
			\frac{1}{n-k}\int_{-\infty}^{\infty}F^{n-k}(x)(1-F(x))^{k}dx  + 
			\int_{-\infty}^{\infty} F^{n-k-1}(x)(1-F(x))^k \left( \frac{n}{n-k}F(x) - 1\right)dx} \le 0.
		\end{align*}
		We can further expand it to be
		\begin{align}
			\binom{n-1}{n-k-1}
			\parans{
			\int_{-\infty}^{\infty} F^{n-k-1}(x)(1-F(x))^k \left( \frac{n+1}{n-k}F(x) - 1\right)dx} \le 0.
			\label{ineq:01011741}
		\end{align}
		Define 
		\begin{align*}
			G(t)
			= 
			\int_{-\infty}^{t} F^{n-k-1}(x)(1-F(x))^k \left( \frac{n+1}{n-k}F(x) - 1\right)f(x) dx
		\end{align*}
		Obviously, $\frac{n+1}{n-k}F(x) - 1$ inside the integrand becomes positive for $x > x_0$ and negative otherwise for some $x_0 \in \R$.
		This implies that $G(t) \le G(\infty)$ for any $t \in \R$.
		Let $u = F(x)$ and by change of variables, we have
		\begin{align*}
			G(\infty)
			&=
			\int_{-\infty}^{\infty} u^{n-k-1}(1-u)^{k} \left( \frac{n+1}{n-k}u - 1\right)du
			\\
			&= 
			\frac{n+1}{n-k}B(n-k+1,k+1) - B(n-k,k+1)
			\\
			&=
			\frac{n+1}{n-k}\frac{(n-k)!k!}{(n+1)!} - \frac{(n-k-1)!k!}{n!} = 0
		\end{align*}
		where $B(\cdot,\cdot)$ denotes the beta function.
		Hence, we have $G(t) \le 0$ for any $t \in \R$.
		Plugging $g(x)$ to be the integrand of $G(x)$ and $h(x) = 1/f(x)$ to the first part of Lemma~\ref{lm:barlow}, we conclude that ~\eqref{ineq:01011741} holds since $h(t)$ is nonincreasing due to the assumption on $f(x)$.		
		This completes the first part of the lemma.
		
		\paragraph{Part (2)}
		Rearranging $(n+1)\delta_{k,n} \le n\delta_{k,n-1}$, we need to show that
		\begin{align*}
			\frac{1}{n}\Ex{X_{k+1:n} - X_{k:n}} + \Ex{X_{k+1:n} - X_{k+1:n-1}} \le \Ex{X_{k:n} - X_{k:n-1}}.	
		\end{align*}
		Due to \citet{david1997augmented}, we obtain the following equations.
		\begin{align*}
			\frac{1}{n}\Ex{X_{k+1:n} - X_{k:n}}
			&=
			\frac{1}{n}\binom{n}{n-k}\int_{-\infty}^{\infty}F^{k}(x)(1-F(x))^{n-k}dx
			\\
			\Ex{X_{k+1:n} - X_{k+1:n-1}}
			&=
			-\binom{n-1}{k}\int_{-\infty}^{\infty}F^{k+1}(x)(1-F(x))^{n-k-1}dx
			\\
			\Ex{X_{k:n} - X_{k:n-1}}
			&=
			-\binom{n-1}{k-1}\int_{-\infty}^{\infty}F^{k}(x)(1-F(x))^{n-k}dx
		\end{align*}
		Plugging into the inequality and rearranging it, we need to show that
		\begin{align*}
			\frac{(n-1)!}{(k-1)!(n-k)!}\parans{-\frac{1}{k}\int_{-\infty}^{\infty}F^k(x)(1-F(x))^{n-k}dx + \int_{-\infty}^{\infty}F^k(x)(1-F(x))^{n-k-1}\parans{\frac{n}{k}F(x) - 1}} \ge 0,
		\end{align*}
		which is equivalent to
		\begin{align*}
			\frac{(n-1)!}{(k-1)!(n-k)!}\parans{\int_{-\infty}^{\infty}F^k(x)(1-F(x))^{n-k-1}\parans{\frac{n+1}{k}F(x) - \frac{k+1}{k}}} \ge 0.
		\end{align*}
		Define $G'(t) = \int_{t}^{\infty}F^{k-1}(x)(1-F(x))^{n-k-1}\parans{\frac{n+1}{k}F(x) - \frac{k+1}{k}}f(x)dx$.
		Observe that $\frac{n+1}{k}F(x) - \frac{k+1}{k}$ becomes positive for $x > x_0$ and nonpositive otherwise for some $x_0 \in \R$.
		Hence, $G'(t) \ge G'(-\infty)$.
		Now we show that $G'(-\infty) \ge 0$.
		Using change of variable with $F(x) = u$, we have
		\begin{align*}
			G'(-\infty)
			&=
			\int_{-\infty}^{\infty}u^{k-1}(1-u)^{n-k-1}\parans{\frac{n+1}{k}u  - \frac{k+1}{k}}	du
			\\
			&=
			\frac{n+1}{k}B(k+1,n-k) - \frac{k+1}{k}B(
			k,n-k)
			\\
			&=
			\frac{n+1}{k}\frac{k!(n-k-1)!}{n!} - \frac{k+1}{k}\frac{(k-1)!(n-k-1)!}{(n-1)!}
			\\
			&=
			\frac{(k-1)!(n-k-1)!}{(n-1)!}\parans{\frac{n+1}{n} - \frac{k+1}{k}} \le 0,
		\end{align*}
		where the last inequality follows from $k \le n-1$.
		Hence we conclude that $G'(t) \ge 0$ for any $t \in \R$.
		Now, plugging in $g(x)$ to be the integrand of $G'(x)$ and $h(x) = f(x)^{-1}$ to the second part of Lemma \ref{lm:barlow}, we finish the proof.
\end{proof}

\subsection{Proof of Lemma \ref{lm:id_preserving}}\label{pf_lm:id_preserving}
\begin{proof}
		We separately prove the following two cases.
  
		\paragraph{Part (1)}
		Let $f(x)$ and $F(x)$ be p.d.f. and c.d.f. of the distribution $X_i \sim D$, and let $g(x)$ be p.d.f. of $n$-th order statistics, respectively.
		Then, we have
		\begin{align*}
			g(x)
			&=
			\frac{n!}{(n-1)!(n-n)!}f(x)F^{n-1}(x)(1-F(x))^{n-n} = nf(x)F(x)^{n-1}.
		\end{align*}
		Since both $f(x)$ and $F(x)$ are nondecreasing on $x$, we finish the proof.
		
		\paragraph{Part (2)}
		Let $g(x)$ be p.d.f. of first order statistics.
		Then, we have
		\begin{align*}
			g(x) = \frac{n!}{(1-1)!(n-1)!}f(x)F^{1-1}(x)(1-F(x))^{n-1} = nf(x)(1-F(x))^{n-1}.
		\end{align*}
		Since both $1-F(x)$ and $f(x)$ are nonincreasing on $x$, we finish the proof.
\end{proof}

\subsection{Proof of Theorem \ref{thm:decaying_upperbound}}\label{pf_thm:decaying_upperbound}
\begin{proof}
Recall that the additive approximation factor is upper bounded by $\Ex{X_{(1)} - X_{(2)}}$ by Corollary \ref{cor:infbud_notau}.
	As we discussed above, the proof mainly follows from Lemma \ref{lm:order_stat_diff_restricted} on the expected difference between two consecutive order statistics.
	By Lemma \ref{lm:id_preserving}, we know that $X_{i,(1)}$ has p.d.f. which is nondecreasing on $x$.
	Now, denote by $\Ex{X_{(1):n} - X_{(2):n}}$ the additive approximation factor in the problem setting when there exists $n$ agents.
	By repeating Lemma \ref{lm:order_stat_diff_restricted} with $k=1$, we have the following series of inequalities.
	\begin{align*}
		(n+1)\Ex{X_{(1):n} - X_{(2):n}} 
		&\le
		n \Ex{X_{(1):n-1} - X_{(2):n-1}}
		\\
		n\Ex{X_{(1):n-1} - X_{(2):n-1}} 
		&\le
		(n-1)\Ex{X_{(1):n-2} - X_{(2):n-2}}
		\\
		&\vdots
		\\
		4\Ex{X_{(1):3} - X_{(2):3}} 
		&\le
		3\Ex{X_{(1):2} - X_{(2):2}}.
	\end{align*}
	By multiplying the inequalities, we obtain
	\begin{align*}
		\Ex{X_{(1):n} - X_{(2):n}} \le \frac{3}{n+1}\Ex{|A-B|},
	\end{align*}
	where $A$ and $B$ are two i.i.d. random variables of which the endowed distribution is equivalent to that of $X_{i, (1)}$.
	Similarly from the proof of Theorem~\ref{thm:mhr_upperbound}, we can further obtain
	\begin{align*}
		\Ex{|A-B|} 
		\le
		\sqrt{\frac{4}{3}\var(A)},
	\end{align*}
	and it completes the proof.
	In case of uniform distribution $U[0,1]$, it is widely known that $X_{i,(1)} \sim Beta(k, 1)$.
	Hence, we conclude that the additive approximation factor is upper bounded by
	\begin{align*}
		\frac{3}{n+1}\sqrt{\frac{4k}{3(k+1)^2(k+2)}} \approx \frac{3.464}{k(n+1)}.
	\end{align*}

\end{proof}

\subsection{Proof of Theorem \ref{thm:pim_neg_incomp}}\label{pf_thm:pim_neg_incomp}
\begin{proof}
The proof consists of two parts.
First, we prove that there exists a problem instance such that proposing a solution that minimizes the principal's utility constructs an equilibrium, which leads to the principal's utility of $\Ex{\max_{i \in [n]}X_{i,(k)}}$.
Next, we analyze the bound on this quantity under the uniform distribution.

\paragraph{Worst-case instance}
Consider $n$ symmetric agents that find solutions $\omega$ such that
	$x(\omega) = x_0$ is sampled from a continuous distribution with c.d.f. of $F(x_0)$.
    Each agent samples $k$ solutions.
    For example, agent $i$ samples $\omega_{i, 1}, \omega_{i, 2}, ..., \omega_{i, k}$.
For an observed solution $\om_{i, j}$, define agents' utility function $y$ as a function of $x(\om_{i,j})$ as follows
\begin{align*}
		y(\omega_{i, j}) = \parans{1 - \parans{\parans{1 - F(x(\omega_{i, j}))}^k}^{n-1}}^{-2}.
\end{align*}
Under this setting, we claim that there exists a BNE such that each agent,
among all of his sampled solutions, proposes the solution which minimizes the principal's utility.
In order to show this claim, we prove that assuming other agents propose solutions with the lowest principal's utility,
best-response for agent $i$ is also to submit the solution which minimizes the principal's utility. Denote others' strategy by $\sigma_{-i}$.
\begin{align*}
    \Ex{u_i(\omega, \sigma_{-i}) | x(\omega) = x_0} = \Pr{\omega \text{ is winner} | \sigma_{-i}, x(\omega)=x_0} y(\omega)
\end{align*}
As all other agents propose solutions with the lowest principal's utility, the probability that $\omega$ is chosen as the winner is the probability that all agents observe at least one solution $\omega'$ such that $x(\omega') \le x(\omega) = x_0$.
Note that tie does not happen as $F$ is a continuous function.
Formally, 
\begin{align*}
	\Pr{\omega \text{ is winner} | \sigma_{-i}, x(\omega)=x_0} = \parans{1 - \parans{1 - F(x_0)}^k}^{n-1}.
\end{align*}
Plugging in the above equation, we have
\begin{align*}
	\Ex{u_i(\omega, \sigma_{-i}) | x(\omega) = x_0} = \parans{1 - \parans{1 - F(x_0)}^k}^{n-1} y(\omega) = \frac{1}{\parans{1 - \parans{1 - F(x_0)}^k}^{n-1}}
\end{align*}
This indicates that agent utility is a decreasing function of $x_0$ which further implies that agent $i$ best response is to propose solution $\omega$ such that $\omega = \argmin_{\omega \in \omb_i} x(\omega)$.
We prove that agent $i$ best-response is to propose the solution with the lowest principal's utility, which concludes that this set of strategies forms a BNE.
% This example shows that incomplete prior-independent setting is different from complete prior-independent case and by finding a proper function $y$, it is possible to motivate agents prosposing their worst solutions in terms of principal's utility, i.e. agent $i$ proposes solution which gives the utility of $X_{i, (k)}$ to the principal.
Hence in this case, the expected utility of the principal is $\Ex{\max_{i \in [n]} X_{i,(k)}}$.

\paragraph{Computing lower bound of $\poa_a$ for uniform distribution}
Now we derive an upper bound for this quantity on the uniform distribution $U[0,1]$ setting, \ie
$X_{i, j} \sim U[0, 1]$.
Note that $X_{i,(k)}$ follows the beta distribution with parameter $(1,k)$.
By Jensen's inequality,
\begin{align}
    e^{t\parans{\Ex{\max_{i \in [n]} X_{i,(k)}} - 1/(k+1)}}
    \le
    \Ex{e^{t \cdot \parans{\max_{i \in [n]} X_{i,(k)} -1/(k+1)}}}
    \le
    \sum_{i=1}^n \Ex{e^{t(X_{i,(k)} - 1/(k+1))}}.\label{ineq:01152042}
\end{align}
Now we use the fact that beta distribution is subgaussian with certain choices of parameters.
\begin{theorem}[Theorem 4 in \cite{elder2016bayesian}]
    The beta distribution with parameter $\alpha, \beta$ is $\frac{1}{4(\alpha+\beta) + 2}$-subgaussian.
\end{theorem}
Plugging $\alpha =1$ and $\beta=k$, we obtain that $X_{i,(k)}$ is $\frac{1}{4k+6}$-subgaussian.
Due to the definition of subgaussianity, we have
\begin{align*}
    \Ex{e^{t(X_{i,(k)})}} 
    \le e^{t^2/(8k+12)}.
\end{align*}
Plugging back to \eqref{ineq:01152042} and rearranging, we obtain
\begin{align*}
    \Ex{\max_{i \in [n]} X_{i,(k)}}
    \le
    \frac{1}{k+1} + \inf_{t > 0 } \frac{1}{t} \log \parans{n \cdot e^{t^2/(8k+12)}}
    =
    \frac{1}{k+1}  + \sqrt{\frac{\log n}{2k+3}}.
\end{align*}
Since $\Ex{X_{\max}} = \frac{nk}{nk+1}$, we conclude that the additive approximation factor is at least
\begin{align*}
    \poa_a \ge \frac{nk}{nk+1} - \frac{1}{k+1} - \sqrt{\frac{\log n}{2k+3}} \ge \frac{k-1}{k+1} - \sqrt{\frac{\log n}{2k+3}}.
\end{align*}
This concludes that there exists no mechanism such that $\poa_a < \frac{k-1}{k+1} - \sqrt{\frac{\log n}{2k+3}}$.
We note that by fixing $n$ and increasing $k$ sufficiently, we can make this bound arbitrarily close to $1$, and we finish the proof.
% \keivan{I didn't check technical details but the bound worked when I ran simulation. current lowerbound is correct and I verified it with expermients.}
% \begin{corollary}
% 	Consider $n$ symmetric agents such that
% 	$x(\omega)$ is sampled from uniform distribution over $\left[0, 1\right]$.
% 	We define utility function $y$ based on \ref{exm:exm1}.
% 	According to BNE found in \ref{exm:exm1},
% 	agent $i$ proposes solution that corresponds to $X_{i, (k)}$. 
% 	So delegation gap is
% 	\begin{align*}
% 		\Ex{X_{(1)}} - \Ex{\max_i X_{i, (k)}}.
% 	\end{align*}
% 	Accoring to uniform distribution order statistics\cite{gentle2012springer},
% 	\keivan{How should I reference this?} we know that $X_{i, (k)} \sim Beta(1, k)$. \keivan{quanity delegation gap.}
%     \suho{ see: https://math.stackexchange.com/questions/2212309/maximum-of-independent-beta-random-variables}
% \end{corollary}
\end{proof}


\subsection{Proof of Theorem \ref{thm:bayes_oblivious}}\label{pf_thm:bayes_oblivious}
\begin{proof}
The proof consists of two main parts.
First, we construct an event $E$ such that there exists an $\Pr{E^c}$-approximate BNE which yields the optimal principal's utility.
Then, we analyze the probability of the event $E$ happening.

\paragraph{Existence of approximate BNE}
	Consider an MSPM with no eligible sets and a deterministic tie-breaking rule $\rho$.
	Define an event $E_i(\cdot)$ as follows.
	\begin{align*}
		E_i(\{x(\om), y(\om)\}_{\om \in \omb_i})
		=
		\paranm{\omb_i : \argmax_{\om \in \omb_i} x(\om)^{k(n-1)}y(\om) = \argmax_{\om \in \omb_i} x(\om)}.
	\end{align*}
	For notational simplicity, let $x(A) = \{x(\om)\}_{\om \in A}$ and similarly for $y(A)$.
        We often overwrite $E_i(\{x(\om), y(\om)\}_{\om \in \omb_i})$ by $E_i$ or $E_i(\omb_i)$. 
	Define 
	\begin{align}
		E(\omb) = E(x(\omb), y(\omb)) = \cap_{i \in [n]} E_i(x(\omb_i)).\label{ineq:01231307}
	\end{align}
        We also write $E(\omb)$ to denote $E$.
        Now, we will prove that given $E(x(\omb), y(\omb))$ and the other's strategies, proposing a solution that maximizes $x$ will be approximately best-response.
	Let's restrict our attention to the case in which $E$ happens given $\omb$.
	Suppose that agent $j \neq i$ proposes a candidate to maximize $x(\cdot)$, \ie $\sigma_{j} = \argmax_{\om \in \omb_j}x(\om)$.
	Then, conditioned on $E$, agent $i$'s expected payoff of proposing $\om \in \omb_i$ can be obtained as
	\begin{align*}
		u_i(\om, \sigma_{-i}|E(\omb))
		&=
		\Pr{\om \text{ is winner} \given E(\omb)}\cdot y(\om)
		\\
		&=
		\Pr{x(\om) \ge x(\om'), \forall\om' \in \omb_{-i}\given E(\omb)}\cdot y(\om)
		\\
		&= x(\om)^{k(n-1)}y(\om).
	\end{align*}
	Since we conditioned on $E(\omb)$, for agent $i$, the solution that maximizes $x(\om)^{k(n-1)}y(\om)$ is exactly the same to the solution that maximizes $x(\om)$.
	This verifies that conditioned on $E(\omb)$ and assuming that the other agent $j \neq i$ proposes a candidate that maximizes $x(\cdot)$, also maximizing $x(\cdot)$ is agent $i$'s best response.
	Let $\sigma_i^x$ be a strategy to propose a solution that maximizes $x(\cdot)$ for agent $i$.
 
	Given that all the other agents $j$ playing $\sigma_j^x$ for $j \neq i$, we can further obtain the following regarding agent $i$'s utility
	\begin{align*}
		u_i(\sigma_i^x, \sigma_{-i})
		&=
		\Ex{u_i(\sigma_i^x, \sigma_{-i})\given E}\Pr{E} + \Ex{u_i(\sigma_i^x, \sigma_{-i})\given E^c}\Pr{E^c}
		\\
		&\ge
		\Ex{u_i(\sigma_i^x, \sigma_{-i})\given E}\Pr{E}
		\\
		&\ge
		\Ex{u_i(\sigma'_i, \sigma_{-i})\given E}\Pr{E}
		\\
		&=
		\Ex{u_i(\sigma'_i, \sigma_{-i})} - \Ex{u_i(\sigma_i',\sigma_{-i}|E^c)}\Pr{E^c}
		\\
		&\ge
		\Ex{u_i(\sigma'_i, \sigma_{-i})} - \Pr{E^c},
	\end{align*}
	where the second inequality follows from the fact that given $E$, playing $\sigma_i^x$ is weakly dominant over any other strategy $\sigma'_i$ for agent $i$.
	This implies that if we characterize a good lower bound $\alpha$ such that $\Pr{E} \ge \alpha$, we have
	\begin{align*}
		u_i(\sigma_i^x, \sigma_{-i})
		\ge
		u_i(\sigma_i', \sigma_{-i}) - 1 + \alpha,
	\end{align*}
	which implies that $\sigma_i^x$ is $(1-\alpha)$-approximate BNE.

\paragraph{Analyzing the lower bound on $\Pr{E}$}
	Now, we compute the lower bound on $\Pr{E}$.
	Due to the independence of the utility distributions, we have
	\begin{align}
		\Pr{E(\omb)}
		= 
		\prod_{i \in [n]}
		\Pr{E_i(\omb_i)}.\label{ineq:01222241}
	\end{align}
We start with the following claim.
\begin{claim}\label{cl:4}
    $\Pr{E_i(\omb_i)} = \Ex{\prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}}}$, where $A_{i,j} = \parans{\frac{X_{i,(j)}}{X_{i,(1)}}}^{k(n-1)}$ for $j \in [k]$.
\end{claim}
\begin{proof}[Proof of the claim]

 Note that each probability can be computed as the following.
	\begin{align*}
		\Pr{E_i(\omb_i)} 
		= 
		\int_{x(\omb_i)} \Pr{E_i(\omb_i) \given x(\omb_i)}f_x(x(\omb_i))dx(\omb_i).
	\end{align*}
	Given $x(\omb_i)$, we can further compute
	\begin{align*}
		\Pr{E_i(\omb_i) \given x(\omb_i)}
		&=
		\int_{y(\omb_i)}
		\Pr{E_i(x(\omb_i)) \given x(\omb_i), y(\omb_i)}f_y(y(\omb_i))dy(\omb_i)
		\\
		&=
		\Pr{\frac{y(\om^*_i)}{ y(\om)} \ge \parans{\frac{x(\om)}{x(\om_i^*)}}^{k(n-1)},\forall \om \in \omb_i \given x(\omb_i)}
		\\
		&=
		\Pr{\frac{Y_{i,(1)}}{Y_{i,(j)}} \ge \parans{\frac{X_{i,(j)}}{X_{i,(1)}}}^{k(n-1)}, \forall j \in [k] \given X_{i,j}, \forall j \in [k]}.
	\end{align*}
	Note that this probability is $1$ when $j=1$.
	% For each $j \in [k]$, define $A_{i,j} = \parans{\frac{X_{i,(j)}}{X_{i,(1)}}}^{k(n-1)}$.
	Conditioned on the event $Y_{i,(1)} = t$, this probability can be further expanded as
	\begin{align*}
		\Pr{t\parans{\frac{X_{i,(1)}}{X_{i,(j)}}}^{k(n-1)}\ge Y_{i,(j)} \given X_{i,j},\forall j \in [k],Y_{i,(1)} = t}
		&=
		\min\parans{1, t\parans{\frac{1}{A_{i,j}}}}.
	\end{align*}
	Since each solution is i.i.d. sample, we have 
	\begin{align}
		\Pr{\frac{Y_{i,(1)}}{Y_{i,(j)}} \ge \frac{X_{i,(j)}}{X_{i,(1)}}, \forall j \in [k] \given X_{i,j}, \forall j \in [k]}
		&=
		\prod_{j=2}^k\parans{\int_{t=0}^{A_{i,j}}t\parans{\frac{1}{A_{i,j}}}dt + \int_{t=A_{i,j}}^1 1 dt}
		\nonumber
		\\
		&=
		\prod_{j=2}^k\parans{1-\frac{A_{i,j}}{2}}
		\label{ineq:01061949}
	\end{align}
	Hence we have
	\begin{align*}
		\Pr{E_i(\omb_i)} =
		\Pr{\frac{Y_{i,(1)}}{Y_{i,(j)}} \ge \frac{X_{i,(j)}}{X_{i,(1)}}, \forall j \in [k]}
		&=
		\Pr{\frac{Y_{i,(1)}}{Y_{i,(j)}} \ge \frac{X_{i,(j)}}{X_{i,(1)}}, \forall j \in [k] \given X_{i,j}, \forall j \in [k]}\Pr{X_{i,j},\forall j \in [k]}
		\\
		&=
		\int_{X_i} \prod_{j=2}^k\parans{1-\frac{A_{i,j}}{2}} dX_i
		\\
		&=
		\Ex{\prod_{j=2}^k\parans{1-\frac{A_{i,j}}{2}}}
	\end{align*}
\end{proof}
 

%	Finally, we have
%	\begin{align}
%		\Pr{E}
%		&=
%		\prod_{i=1}^n
%		\int_{X_{i}}2\prod_{j=1}^k\parans{1-\frac{1}{2}\parans{\frac{X_{i,j}}{X_{i,(1)}}}^{k(n-1)}} dX_i. \note{These notations needs to be made more formal.}
%		\\
%		&=
%		\prod_{i=1}^n
%		\Ex{2\prod_{j=1}^k\parans{1-\frac{1}{2}\parans{\frac{X_{i,j}}{X_{i,(1)}}}^{k(n-1)}}}.
%	\end{align}
	
%	Define $B_{i,j} = \parans{\frac{X_{i,(j)}}{X_{i,(1)}}}^{k(n-1)}$.
%	Then, since $B_{i,j}$ has
%	
%	Using $1-x \ge e^{-x/(1-x)}$, we have
%	\begin{align*}
%		\Pr{E}
%		&\ge
%		\prod_{i=1}^n
%		\Ex{e^{-\sum_{j=2}^k \frac{B_{i,j}}{2-B_{i,j}}}}. \note{**loose point**}
%	\end{align*}
%	Now we argue that $1-\frac{A_{i,j}}{2}$	for $j=2,\ldots, k$ are independent.
%	It suffices to show that $\frac{X_{i,(j)}}{X_{i,(1)}}$ for $j=2,\ldots, k$ are independent.
%	Note that pdf of $\frac{X_{i,(j)}}{X_{i,(1)}}$ can be computed as follows.
%	\begin{align*}
%		f_{\frac{X_{i,(2)}}{X_{i,(1)}},\ldots,\frac{X_{i,(j)}}{X_{i,(k)}}}(a_{i,2},\ldots, a_{i,k})
%		&= \int_{X_{i,(1)} = t}f_{X_{i,(2)} ,\ldots, X_{i,(n)}}(ta_{i,2},\ldots, ta_{i,k})f_{X_{i,(1)}}(t) dt
%		\\
%		&= \int_{X_{i,(1)} = t} f_{X_{i,(1)}, \ldots, X_{i,(k)}}(t,ta_{i,2}, \ldots, ta_{i,k})dt
%		\\
%		&= \int_{X_{i,(1)} = t} k! dt,
%	\end{align*}
%	where the last inequality follows from the fact that joint density of all the order statistics is simply $k!$.
%	For each p.d.f. of $A_{i,j}$, observe that for $j=2,\ldots, k$,
%	\begin{align*}
%		f_{A_{i,j}}(a_{i,j})
%		&=
%		\int_{X_{i,(1)}=t} f_{X_{i,(1)},X_{i,(j)}}(t,ta_{i,j}) dt
%		\\
%		&=
%		\int_{X_{i,(1)}=t} f_{U_{k-j+1},U_{k}}(ta_{i,j}, t) dt
%		\\
%		&=
%		\int_{X_{i,(1)}=t} k! \frac{(ta_{i,j})^{k-j}}{(k-j)!}\frac{(t-ta_{i,j})^{j-2}}{(j-2)!}dt
%		\\
%		&=
%		\int_{X_{i,(1)}=t} \frac{k!}{(k-j)!(j-2)!} t^{k-2}a_{i,j}^{k-j}(1-a_{i,j})^{j-2}dt
%		\\
%		&=
%	\end{align*}
%	where $U_{(i)}$ denotes $i$-th order statistics given $k$ i.i.d. random variables from $U[0,1]$.

Now we prove that we can decompose the product inside the expectation as follows.
\begin{claim}\label{cl:5}
    $\Ex{\prod_{j=2}^k\parans{1-\frac{A_{i,j}}{2}}} \ge \int_{t=0}^1\prod_{j=2}^k\parans{\Ex{1-\frac{1}{2}\parans{\frac{X_{i,(j)}}{t}}^{k(n-1)} \given X_{i,(1)}= t}}\Pr{X_{i,(1)} =t}dt$.
\end{claim}
\begin{proof}[Proof of the claim]

	
	Given $X_{i,(1)} = t$, we note that $1-\frac{A_{i,j}}{2}$ for $j=2,\ldots,k$ is nonincreasing function over  $(X_{i,(2)},\ldots, X_{i,(k)})$.
	Now, we use the following correlation inequality called as \emph{Fortuin-Kasteleyn-Ginibre} (FKG) inequality.
	\begin{lemma}[\cite{alon2016probabilistic}]\label{lm:FKG}
		Let $\nu_1,\ldots, \nu_n$ be a probability measure on $\R$.
		If functions $f,g:\R^n \mapsto [0,1]$ are monotone increasing functions, then $\Exu{\nu}{f\cdot g} \ge \Exu{\nu}{f} \cdot \Exu{\nu}{g}$, where $\nu$ is a product measure over $\nu_1,\ldots, \nu_n$.
		The same inequality holds when both $f,g$ are monotone decreasing functions.
	\end{lemma}
        For given $i$, we have $f_j = 1-\frac{A_{i,j}}{2}$ for $j=2,3,\ldots, k$, each of which is a nonincreasing function over $X_{i,(j)}$.\footnote{Note in fact that we cannot directly plug in $f_j = 1-A_{i,j}/2$ in the inequality due to the correlation between the order statistics. That said, by rewriting the expression to be over the original random variables instead of order statistics, we can easily see that the same result follows, since the expectation remains for either of expressions.}
        Hence, by applying FKG inequality, we can further expand it as follows.
	% \kvdelete{we need to elaborate more here, what is each of our functions and how we use FKG.
	% I guess we have functions $f_2, f_3, .., f_{k-1}$ each of which is a function of $X_{i, (j)}$
	% then we need to mention the fact that they are decreasing and then using FKG.
	% }
	\begin{align}
		\Ex{\prod_{j=2}^k \parans{1-\frac{A_{i,j}}{2}}}
		&=
		\int_{t=0}^1\Ex{\prod_{j=2}^k \paranl{1-\frac{1}{2}\parans{\frac{X_{i,(j)}}{t}}^{k(n-1)}} \given X_{i,(1)} = t}\Pr{X_{i,(1)} = t}dt
		\nonumber
		\\
		&\ge
		\int_{t=0}^1\prod_{j=2}^k\parans{\Ex{1-\frac{1}{2}\parans{\frac{X_{i,(j)}}{t}}^{k(n-1)} \given X_{i,(1)}= t}}\Pr{X_{i,(1)} =t}dt,
		\label{ineq:01022357}
	\end{align}
        and it completes the proof.
\end{proof}

Now we show that we can derive a constant lower bound that depends only on $k,n$ and $j$ on the quantity inside the expectation as follows.
\begin{claim}\label{cl:6}
    For $j =2,3,\ldots, k$, define $g_j(t)$ as follows.
    \begin{align*}
        g_j(t) = 	\Ex{1-\frac{1}{2}\parans{\frac{X_{i,(j)}}{t}}^{k(n-1)}\given X_{i,(1)} = t}.
    \end{align*}
    Then, we have the following lower bound on $g_j(t)$.
    \begin{align*}
        g_j(t) \ge 1 - \frac{1}{2}\parans{\frac{k-1}{kn-1}}^{j-1}.
    \end{align*}
\end{claim}
\begin{proof}[Proof of the claim]
We remark that $g_j(t)$ is a lower bound on the probability that $E_i(\omb_i)$ happens conditioned on $X_{i,(1)}=t$.
	Rewrite $g_j(t)$ as
	\begin{align*}
		\int_{x=0}^t \parans{1-\frac{1}{2}\parans{\frac{x}{t}}^{k(n-1)}}f_{X_{i,(j)} | X_{i,(1)}=t}(x)dx
	\end{align*}
	Now, the joint density function of $X_{i,(j)},X_{i,(1)}$ can be computed as
	\begin{align*}
		f_{X_{i,(j)},X_{i,(1)}}(x,t)
		&=
		f_{U_{(k-j+1)}, U_{(k)}}(x,t)
		\\
		&=
		k!\frac{x^{k-j}}{(k-j)!}\frac{(t-x)^{j-2}}{(j-2)!},
	\end{align*}
	where $U_{(j)}$ denotes $j$-th order statistics from $k$ i.i.d. random variables with $U[0,1]$.
	
	The density function of $X_{i,(1)}$ is p.d.f. of $Beta(k,1)$, which is $t^{k-1}/B(k,1)$ where $B(\cdot,\cdot)$ is the beta function.
	This implies that
	\begin{align*}
		f_{X_{i,(j)}|X_{i,(1)}=t}(x) = 	k!\frac{x^{k-j}}{(k-j)!}\frac{(t-x)^{j-2}}{(j-2)!}\frac{B(k,1)}{t^{k-1}}
	\end{align*}

	Hence, we have
	\begin{align*}
		g_j(t)
		=
		\int_{x=0}^t \parans{1-\frac{1}{2}\parans{\frac{x}{t}}^{k(n-1)}}\frac{k!}{(k-j)!(j-2)!}\frac{B(k,1)}{t^{k-1}}x^{k-j}(t-x)^{j-2}dx.
	\end{align*}
	By change of variables with $x = ty$, and we have
	\begin{align}
		g_j(t)
		&=
		\int_{y=0}^1 \parans{1-\frac{y^{k(n-1)}}{2}}
		\frac{k!}{(k-j)!(j-2)!}\frac{B(k,1)}{t^{k-1}}(ty)^{k-j}(t-ty)^{j-2}tdy
		\nonumber
            \\
		&=
		\frac{k!B(k,1)}{(k-j)!(j-2)!}
		\int_{y=0}^1
		\parans{1-\frac{y^{k(n-1)}}{2}}y^{k-j}(1-y)^{j-2}dy,
		\nonumber
	\end{align}
    where we use the fact that $B(x,y) = \frac{(x-1)!(y-1)!}{(x+y-1)!}$ for positive integers $x,y$,
    Rewriting the RHS using the definition of beta function, we can further expand
    \begin{align}
            g_j(t)=
		\frac{(k-1)!}{(k-j)!(j-2)!}\parans{B(k-j+1,j-1) - \frac{B(kn-j+1,j-1)}{2}}
		&=
		1 - \frac{1}{2} \frac{(kn-j)!(k-1)!}{(kn-1)!(k-j)!}
		\nonumber
            \\
		&=
		1 - \frac{1}{2} \frac{(k-j+1)\ldots (k-1)}{(kn-j+1)\ldots(kn-1)}
		\nonumber
            \\
		&\ge
		1-\frac{1}{2}\parans{\frac{k-1}{kn-1}}^{j-1},\label{ineq:01212139}
    \end{align}
where we use that $B(x,y) = \int_{t=0}^1 t^{x-1}(1-t)^{y-1}dt$ for any real $x,y$.
For the inequality, we use $\frac{k-j+1}{kn-j+1} \le \frac{k-1}{kn-1}$ for any $j =2,3,\ldots, k$.
This completes the proof.
\end{proof}

Due to the claims above (Claim~\ref{cl:4},\ref{cl:5} and \ref{cl:6}) and by \eqref{ineq:01222241}, we obtain the following lower bound on the event $E_i$.
	\begin{align*}
            \Pr{E_i}
            &=
            \Ex{\prod_{j=2}^k \parans{1-\frac{A_{i,j}}{2}}}
            \\
            &\overset{(a)}{\ge}
            \int_{t=0}^1\parans{\prod_{j=2}^k g_j(t)}\Pr{X_{i,(1)} =t}dt
            \\
		&\overset{(b)}{\ge}
		\int_{t=0}^1  \parans{\prod_{j=2}^k 1-\frac{1}{2}\parans{\frac{k-1}{kn-1}}^{j-1}}\Pr{X_{i,(1)}=t}dt
		\\
		&=
		 \prod_{j=2}^k \parans{1-\frac{1}{2}\parans{\frac{k-1}{kn-1}}^{j-1}}
		\\
		&\ge
		 \prod_{j=2}^k \parans{1-\frac{1}{2}\parans{\frac{1}{n}}^{j-1}},
	\end{align*}
        where $(a)$ holds by Claim~\ref{cl:5}  and $(b)$ follows from Claim~\ref{cl:6}.
	
 Using $1-x \ge e^{-x/(1-x)}$ for $x \in (0,1)$, we finally have 
	\begin{align}
		\Pr{E(\omb_i)}
		&\ge
		\exp\parans{-\sum_{j=2}^k \frac{\parans{\frac{1}{n}}^{j-1}}{2-\parans{\frac{1}{n}}^{j-1}}}.\label{ineq:05031951}
	\end{align}
        Now we proceed with the following series of algebraic manipulation.
        \begin{align*}
            \eqref{ineq:05031951}
            &\ge
		\exp \parans{-\sum_{j=2}^k \frac{1}{2n^{j-1}-1}}
		\\
		&\ge
		\exp \parans{-\sum_{j=2}^k \frac{1}{2}\frac{1}{n^{j-1}-1}}
		\\
		&=
		\exp \parans{-\frac{1}{2(n-1)}\sum_{j=2}^k \frac{1}{n^{j-2}+n^{j-3}+\ldots +1}}
		\\
		&\ge
		\exp \parans{-\frac{1}{2(n-1)}\sum_{j=2}^k \frac{1}{n^{j-2}}}
		\\
		&=
		\exp \parans{-\frac{1}{2(n-1)} \frac{1-\parans{\frac{1}{n}}^{k-1}}{1-\frac{1}{n}}}
		\\
		&\ge
		\exp\parans{-\frac{n}{2(n-1)^2}}.
        \end{align*}
	Multiplying it over $i \in [n]$, we have
	\begin{align}
		\Pr{E} \ge \exp\parans{-\frac{n^2}{2(n-1)^2}},
		\label{ineq:01062049}
	\end{align}
	where it converges to $1/\sqrt{e} \approx 0.6065...$ as $n$ increases.
	Hence, we conclude that playing $\sigma_i^x$ is $(1 - e^{-n^2/2(n-1)^2})$-approximate BNE, and as the principal's utility is $X_{\max}$ for any observation of solutions under this equilibrium, we complete the proof. 
\end{proof}

\subsection{Proof of Theorem \ref{theorem:multi-agent-limited-budget}}
\label{pf_theorem:multi-agent-limited-budget}
\begin{proof}
Due to our definition of RSPM, $B$ of proposed candidates will be randomly chosen by the principal and the best candidate among them will be selected as the winner.
Let $E$ be the set of agents who have at least one eligible solution to propose, and $E'$ be the set of other agents. 
Denote the size of sets $E$ and $E'$ by $e$ and $e'$ respectively so that $e + e' = n$.
Let $\omb = \cup_{i \in [n]}\omb_i$ be the entire set of solutions observed by the agents and $\sigma = (\sigma_1,\ldots, \sigma_n)$ be arbitrary equilibrium strategy.
For $i \in E'$,  since agent $i$ does not have eligible solutions,
even his best-observed solution which gives the utility of $X_{i, (1)}$ to the principal is not eligible.
%\suho{This notion of best observed solution is used a lot. How about formally define it in model section and reuse them?}
This implies that $X_{i, (1)} < \tau$. 
On the other hand, for $i \in E$, agent $i$ has at least one eligible observed solution to propose which
implies that his best-observed solution is also eligible as well, \ie $X_{i, (1)} \geq \tau$.
These arguments further imply that $X_{(e)} \geq \tau > X_{(e + 1)}$.
% Due to our definition of rank, we can further conclude that for any $i \in [e]$, the agent with rank $i$ is partitioned to $E$ and for any $j \in [n] \setminus [e]$, the agent with rank $j$ is partitioned to $E'$. 
We consider two cases (i) when $e \le B$ and (ii) when $e > B$, and prove the theorem separately. 

{Case (i): $e \leq B$.} 
In this case, the number of agents who have eligible solutions is at most $B$, which implies that $X_{(B+1)} < \tau$. 
In this case, there exist at most $B$ proposed candidates thus the principal can examine all of them and take the best one. 
As a result, this case is equivalent to the unlimited budget we had in Theorem \ref{theorem:multi-agent-unlimited-budget},
and hence from the same argument, the principal's expected utility is at least
\begin{align*}
    \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau > X_{(B+1)}\right]} + 
    \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}
    .
\end{align*}

%<<<<<<< Updated upstream
%{\em Case (ii): $e > B$.} 
%We define set $L \subseteq E$ of size $B - 1$ of agents whose candidates give the lowest utility to the principal so for each pair of agents $(i, j)$ where $i \in E - L, j \in L$, we have $x(c_i) > x(c_j)$. 
%We call the agents in set $L$ as \textit{losers}. 
%The principal randomly examines $B$ candidates proposed by agents. 
%This implies that loser agents are never selected as the winner because there always exists a candidate from a non-loser agent in the set of candidates that the principal examines, and that candidate gives a better utility to the principal thus a proposed candidate by a loser agent is not selected as the winner. 
%\suho{I think it suffices to emphasize when it first appears.}
%\suho{As I said above, maybe we can argue this sentence more formally by doing some math on it?}
%As a result, the utility of loser agents is $0$. 
%For all non-loser agents such as agent $i$, there is a chance that his candidate is selected as the winner because if the principal examines $B - 1$ candidates proposed by loser agents, and also examines agent $i$'s candidate, then in this case agent $i$'s candidate is selected as the winner. 
%=======

{Case (ii): $e > B$.} 
We follow the proof steps of Theorem~\ref{theorem:multi-agent-unlimited-budget}. Assume that agents play mixed strategies, \ie they construct a probability distribution over the observed solutions.
Formally, given the solutions $\omb$, denote by $p_{i, j}$, the probability that agent $i$ submits $\omega_{i, j}$ as his candidate.
These probability distributions shape a mixed Nash equilibrium.

For each $i \in [n]$ we have $\sum_{j=1}^{k_i} p_{i, j} = 1$.
Define $S_i = \{\omega_{i, j} : p_{i, j} > 0\}$ as the multi-set of solutions that agent $i$ proposes with positive probability.
For each agent $i$, let $b_i$ be the candidate which gives the worst utility to the principal, \ie $b_i = \argmin_{\omega \in S_i} x(\omega$).
If there are multiple candidates with the worst utility, we arbitrarily choose one.
We use $A$ to denote the set of agents who have non-zero utility.

We proceed with the following claim.
\begin{claim}
    $|A| \le e-B+1$.
\end{claim}
\begin{proof}[Proof of the claim]
Suppose not, then $|A| \ge e-B+2$.
Let $t \in A$ be an agent such that for each agent $i \in A \setminus \{t\}$, either
\begin{itemize}
    \item $x(b_t) < x(b_i)$
    \item $x(b_t) = x(b_i)$, and mechanism prefers agent $i$ over agent $t$ using tie-breaking rule $\rho$,
\end{itemize}
\ie agent $t$ is the agent with non-zero utility having worst $b_t$ and least preferred using $\rho$.
As he has non-zero utility and $b_t \in S_i$, proposing $b_t$ gives him non-zero utility as well.

According to the definition of $b_t$,
when $t$ proposes $b_t$, no matter what agents in $A \setminus \{t\}$ propose,
their candidates are dominant, \ie
the mechanism prefers candidate submitted by any agent in $A \setminus \{t\}$ over $b_t$. 

% \suho{please parse the sentence, as it's hard to follow.}
There are $e$ candidates in total and as $|A \setminus \{t\}| \ge e-B+1$, any random choice of $B$ candidates includes at least one candidate of agents in $A \setminus \{t\}$.
This implies that $b_t$ is never selected as the winner,
which is a contradiction with the fact that proposing $b_t$ gives non-zero utility to agent $t$.
So, we conclude that $|A| \le e - B + 1$.
\end{proof}

Now, we focus on agents in $E \setminus A$.
Let $t' \in E \setminus A$ be an agent such that for any agent $j \in E \setminus (A \cup \{t'\})$, either
\begin{itemize}
    \item $X_{t', (1)} > X_{j, (1)}$
    \item $X_{t', (1)} = X_{j, (1)}$, and mechanism prefers agent $t'$ over agent $j$ using tie-breaking rule $\rho$,
\end{itemize}
\ie agent $t'$ has the first-best solution among agents in $E \setminus A$ and
mostly preferred by tie-breaking rule $\rho$.
Note that we proved $|A| \le e - B + 1$ so $|E \setminus A| \ge B - 1$.
Now we claim $X_{t', (1)} \le x(b_t)$ as follows.
\begin{claim}
    $X_{t', (1)} \le x(b_t)$.
\end{claim}
\begin{proof}[Proof of the claim]
Suppose not and let $x(b_t) < X_{t', (1)}$.
We know that under Nash equilibrium, agent $t'$ gets zero utility thus given the strategies of others, no matter what his strategy is, he gets zero utility. 
As a result, even if he proposes his first-best solution that gives the utility of $X_{t', (1)}$ to the principal, his solution is never selected.
However, according to the definition of $t'$, this solution is always preferred to
all candidates proposed by agents in $E \setminus \left(A \cup \{t'\}\right)$ which are at least $B - 2$ candidates. It is also dominant over $b_t$.
Hence due to the randomness of the mechanism,
there exists a non-zero probability that the principal takes these $B - 1$ candidates
and the candidate proposed by $t'$ so that $t'$ becomes the winner and gets non-zero utility.
This is a contradiction to the fact that $t'$ has zero utility and thus $X_{t', (1)} \le x(b_t)$.
\end{proof}

Let $\omega^*$ be the winner. $\omega^*$ belongs to agents in $A$ and according to definition of $b_t$, $x(b_t) \le x(\omega^*)$.
We also proved that $X_{t', (1)} \le x(b_t)$ so principal's utility is at least $X_{t', (1)}$. 
We recall that
\begin{itemize}
    \item 
    According to definitions of $E$ and $E'$,
    $X_{t', (1)} \ge \tau > X_{i, (1)}$ for all $i \in E'$. 
    \item
    According to the definition of $t'$, we have
    $X_{t', (1)} \ge X_{j, (1)}$ for each $j \in E \setminus \left(A \cup \{t'\}\right)$.
\end{itemize}
 
Hence $X_{t', (1)}$ is at least as large as the first-best solutions of $|E'| + |E \setminus \left(A \cup \{t'\}\right)| \geq n - e + B - 2$ agents.
Therefore, we can conclude that $X_{t', (1)} \geq X_{(e - B + 2)}$.
So, in this case where $X_{(e)} \geq \tau > X_{(e+1)}$, we obtain a lower bound on principal's utility as
\begin{align*}
\Ex{X_{(e-B+2)}\IND\left[X_{(e)} \geq \tau > X_{(e+1)}\right]}.
\end{align*}

Now by iterating over all values for $e > B$, we state that the expected utility is at least
\begin{align*}
\sum_{e=B+1}^{n} \Ex{X_{(e-B+2)}\IND\left[X_{(e)} \geq \tau > X_{(e+1)}\right]},
\end{align*}
where we write $X_{(n + 1)} := -\infty$. 
By combining the result of case (i), and case (ii), we can infer that the principal's expected utility is at least
\begin{align*}
\Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau > X_{(B+1)}\right]} +  \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}
+
\sum_{e=B+1}^{n} \Ex{X_{(e-B+2)}\IND\left[X_{(e)} \geq \tau > X_{(e+1)}\right]},
\end{align*}
which shows that the additive approximation factor is at most
\begin{align*}
\Ex{X_{(1)}}
-
\Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau > X_{(B+1)}\right]} -  \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]} \\
-
\sum_{e=B+1}^{n} \Ex{X_{(e-B+2)}\IND\left[X_{(e)} \geq \tau > X_{(e+1)}\right]}
\end{align*}
which finishes the proof.


% The proof mainly follows from the following lemma.
% \begin{lemma}
% Given an examination budget $2 \leq B \le n-1$, the delegation gap of single-proposal mechanism is at least $\sum_{k=B+1}^{n} \Ex{X_{(k-B+2)}\IND\left[X_{(k)} \geq \tau > X_{(k+1)}\right]} $.
% \end{lemma}
% \begin{proof}[Proof Sketch of Lemma]
% Consider the set of proposed candidates. Since the examination budget is $B$ then $B$ of proposed candidates will be randomly chosen by the principal and the best candidate among them will be selected as the final outcome. Assume that $E$ is the set of agents who have at least one eligible solution to propose, and $E'$ is the set of other agents. We can see that $X_{(i)} < \tau\ (\forall_{i \in E'})$ so if there are $e'$ agents in set $E'$, then $E'$ is the set of agents whose ranks are higher than $n - e'$. Based on the number of agents who proposed a candidate we have two cases: 
% \begin{itemize}
%     \item if $|E| \leq B$: this case is equivalent to the unlimited budget we had in Lemma 1 since the principal can examine all proposed candidates. Therefore with the same argument, the principal's utility will be at least:
%     $$
%     \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
%     \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}
%     $$
%     \item if $|E| > B$: 
%     we define set $L \subseteq E$ of size $B - 1$ of agents whose candidates give the lowest utility to the principal. Since the principal randomly examines $B$ candidates proposed by agents, it is guaranteed that the agents' candidates in set $L$ are never selected by the principal. As a result, the utility of agents in $L$ is $0$. For all other agents $i \in E - L$, there is a chance that their candidates are selected by the principal because if the principal examines $B - 1$ candidates proposed by agents in $L$ and agent $i$'s candidate, then in this case agent $i$'s candidate will be selected as the final outcome since by the definition of $L$ we have:
% $x(\sigma_i(\omega_i)) > \max_{j \in L} \sigma_j(\omega_j)$. So, agent $i \in E-L$ has a positive utility in expectation with respect to the randomness of selection; and all agents $j \in L$ have the utility of $0$.
% Consider agent $j \in L$, in a Nash equilibrium if he changes his strategy, he still does not have positive utility, which implies that even if he proposes his best-observed solution which gives the utility of $X_{(j)}$ to the principal, then he is still in set $L$ with the utility of $0$. As a result, we can infer that:
% \begin{align*}
%   x(\sigma_i(\omega_i)) \geq X_{j, (1)} (\forall i \in E - L, \forall j \in L ) \rightarrow X_{i, (1)} \geq X_{j, (1)} \left(\forall i \in E - L, \forall j \in L\right). 
% \end{align*}

% So, agents in set $L$ are agents whose rank is in $[n-e'-B+2, n-e']$; and in this case, for principal's utility we have:
% $$
% x(\sigma_i(\omega_i)) \geq X_{(n-e'-B+2)} = X_{(|E| - B + 2)} \left(\forall i \in E - L\right) 
% $$
% Then by iterating over all possible values of $|E| > B$, the principal's utility will be at least:
% \begin{align*}
% % \Ex{X_{(|E|-B+2)}\IND\left[X_{(|E|)} \geq \tau\right]} (\forall |E|) \\
% \sum_{k=B+1}^{n} \Ex{X_{(k-B+2)}\IND\left[X_{(k)} \geq \tau > X_{(k+1)}\right]} \\
% \geq \Ex{X_{(n-B+2)}}
% \end{align*}
% \end{itemize}
% \end{proof}
\end{proof}


\subsection{Proof of Theorem \ref{thm:bce}}\label{pf_thm:bce}
\begin{proof}
        We recommend the readers skim the proof of Theorem~\ref{thm:bayes_oblivious} in Appendix~\ref{pf_thm:bayes_oblivious} before reading this proof.
        Similar to the proof of Theorem~\ref{thm:bayes_oblivious}, we proceed with three main steps.
        First, we construct a Bayes correlated equilibrium with a certain choice of signaling scheme in which we signal the agents whenever some good event $E$ happens.
        Next, we show that the principal's utility given the signal can be decomposed as $\Ex{X_{\max}} \cdot \Pr{E}$.
        Finally, we obtain a lower bound on the probability that $E$ happens.

        \paragraph{Constructing Bayes correlated equilibrium}
	Consider an MSPM with no eligible sets and a deterministic tie-breaking rule $\rho$.
	Denote by $\omb = \cup_{i \in [n]}\omb_i$ the solutions observed by the agents.
	Similar to the proof of Theorem~\ref{thm:bayes_oblivious}, define an event $E_i(\cdot)$ as follows.
	\begin{align*}
		E_i 
		=
		\paranm{x(\omb_i), y(\omb_i) : \argmax_{\om \in \omb_i} x(\om)^{k(n-1)}y(\om) = \argmax_{\om \in \omb_i} x(\om)}.
	\end{align*}
	Let $x(A) = \{x(\om)\}_{\om \in A}$ and similarly for $y(A)$.
	Define $E = \cap_{i \in [n]} E_i$.
	Let $\sigma_i^x$ be a strategy to propose a solution that maximizes $x(\cdot)$ for agent $i$.
	Denote by $u_i(\sigma_i,\sigma_{-i} | A)$ agent $i$'s expected utility conditioned on the event $A$, \ie
	\begin{align*}
		u_i(\sigma_i,\sigma_{-i} | A)
		=
		\Ex{\int_{\omb \in A}y_i(f_{M,(\sigma_i, \sigma_{-i})})f(\omb | A)d\omb},
	\end{align*}
	where we write $f(\omb | A)$ to denote the probability density function of $\omb$ conditioned on $A$.
	Conditioned on $E_i$, agent $i$'s expected payoff of proposing a solution $\om \in \omb_i$ given that others play $\sigma_{-i}^x$ is
	\begin{align*}
		u_i(\om, \sigma_{-i}^x|E_i)
		&=
		\Pr{\om \text{ is winner} \given E}\cdot y(\om)
		\\
		&=
		\Pr{x(\om) \ge x(\om'), \forall\om' \in \omb_{-i}\given E}\cdot y(\om)
		\\
		&= x(\om)^{k(n-1)}y(\om).
	\end{align*}
	This implies that conditioned on $E_i$, agent $i$'s best response given that others play $\sigma_{-i}^x$ is also $\sigma_i^x$.
	Hence, conditioned on $E(\omb)$, playing $\sigma^x = (\sigma_1^x, \ldots, \sigma_n^x)$ is best-response for each agent given the others' strategies.
	
	Observe that due to the Nash's existence theorem, there exists at least one BNE.
	Denote this equilibrium by $\sigma^o= (\sigma^o_1, \ldots, \sigma^o_n)$.
	Now consider a mediator who recommends $\psi_i = \sigma_i^x$ to agent $i \in [n]$ whenever $E(\omb)$ happens, and recommends $\sigma'_i$ otherwise.
	Due to our construction of $E$, we have
	\begin{align*}
		u_i(\psi_i, \sigma_{-i}^x | E)
		\ge 
		u_i(\sigma_i, \sigma_{-i}^x | E),	
	\end{align*}
	for any other strategy $\sigma'_i$ of agent $i$.
	From our definition of $\sigma^o$, we also have
	\begin{align*}
		u_i(\psi_i, \sigma^o_{-i} | \neg E)
		\ge
		u_i(\sigma'_i, \sigma^o_{-i} | \neg E),
	\end{align*}
	for any other strategy $\sigma'_i$ of agent $i$.
	Combining two inequalities above, we can verify that obeying $\psi = (\psi_1, \ldots, \psi_n)$ constructs a BNE as follows
	\begin{align*}
		u_i(\psi_i, \psi_{-i})
		&=
		u_i(\psi_i, \sigma_{-i}^x | E) \Pr{E} + u_i(\psi_i, \sigma_{-i}^o | \neg E) \Pr{\neg E}
		\\
		&=
		u_i(\psi_i, \sigma_{-i}^x | E) \Pr{E} + u_i(\psi_i, \sigma_{-i}^o | \neg E) \Pr{\neg E}
		\\
		&\ge
		u_i(\sigma'_i, \sigma_{-i}^x | E) \Pr{E} + u_i(\sigma'_i, \sigma_{-i}^o | \neg E) \Pr{\neg E}.
	\end{align*}

        \paragraph{Decomposing the principal's utility}
	For notational simplicity, denote by $x(\sigma)$ the principal's expected utility given the strategies $\sigma$, and $x(\sigma | \omb)$ the principal's utility given $\omb$, \ie given all the random variables $x(\omb)$ and $y(\omb)$.
	Denote by $f_x(x(\omb))$ and $f_y(y(\omb))$ the p.d.f. of $x(\omb)$ and $y(\omb)$, respectively.
	Now, under the BCE with $\psi$, suppose that the agents obey the recommended strategies, \ie $\sigma = \psi$.
	The principal's expected utility $x(\sigma)$ can be lower bounded as
	\begin{align}
		&\int_{x(\omb)}\left( \int_{y(\omb)} \Ex{x(\sigma  | \omb) \given x(\omb), y(\omb)} f_y(y(\omb))dy(\omb) \right) f_x(x(\omb))dx(\omb)
		\nonumber
		\\
		&\overset{(a)}{=} 
		\int_{x(\omb)}\left( \int_{y(\omb)} \Ex{x(\sigma  | \omb) \given x(\omb), y(\omb), E}\Pr{E \given x(\omb), y(\omb)}f_y(y(\omb))dy(\omb) \right) 
		\nonumber
		\\
		&+ \left( \int_{y(\omb)} \Ex{x(\sigma  | \omb) \given x(\omb), y(\omb), \neg E} \Pr{\neg E \given x(\omb), y(\omb)}f_y(y(\omb))dy(\omb) \right)  f_x(x(\omb))dx(\omb)
		\nonumber
		\\
		&\overset{(b)}{\ge}
		\int_{x(\omb)}\left( \int_{y(\omb)} \Ex{x(\sigma  | \omb) \given x(\omb), y(\omb), E} \Pr{E \given x(\omb), y(\omb)}f_y(y(\omb))dy(\omb) \right) f_x(x(\omb))dx(\omb),
		\nonumber
	\end{align}
	where $(a)$ holds by the law of total expectation, and $(b)$ follows from ignoring the latter integral, \ie the one conditioned on $\neg E$.
	First, we observe that conditioned on the event $E$, the principal's utility $x(\sigma | \omb)$ is simply $X_{\max}$.
	This is because conditioned on $E$, each agent $i$ submits $\sigma_i^x$, and the principal finally chooses the one that maximizes her own utility.
	By the independence of $X_{\max}$ over the random variables $y(\cdot)$, we can further obtain
	\begin{align}
		x(\sigma )
		&\ge
		\int_{x(\omb)}\left( \int_{y(\omb)}\Pr{E \given x(\omb), y(\omb)}f_y(y(\omb))dy(\omb) \right)   X_{\max} f_x(x(\omb))dx(\omb).
		\\
		&=
		\int_{x(\omb)}\prod_{i=1}^n\left(\int_{y_i(\omb_i)}\Pr{E \given x(\omb), y_i(\omb)}f_{y_i}(y_i(\omb))dy_i(\omb) \right)   X_{\max} f_x(x(\omb))dx(\omb),
		\label{ineq:12251801}
	\end{align}
	where the last equality follows from the independence of the solutions between the agents.
	Defining $A_{i,j} = \parans{\frac{X_{i,(j)}}{X_{i,(1)}}}^{k(n-1)}$, due to \eqref{ineq:01061949}, we can rewrite \eqref{ineq:12251801} as
	\begin{align}
		\int_{x(\omb)}\parans{\prod_{i=1}^n\prod_{j=2}^k\parans{1 - \frac{A_{i,j}}{2}}}  X_{\max} f_x(x(\omb))dx(\omb)
		&=
		\Ex{X_{\max} \prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}}}
		\nonumber
		\\
		&=
		\Ex{ \Ex{t\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}} \given X_{\max} = t} }.
		\\
		&=
		\int_{t=0}^{1}\Ex{\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}} \given X_{\max} = t}t \Pr{X_{\max} = t}dt
		\label{ineq:01062038}
	\end{align}
	Now we prove the following claim.
	\begin{claim}
		$g(t) = \Ex{\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}} \given X_{\max} = t}$ is an increasing function on $t$.
	\end{claim}
	\begin{proof}[Proof of the claim]
		We can write $g(t)$ as
		\begin{align*}
			\sum_{s=1}^n\Ex{\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}} \given X_{s,(1)} = t, \argmax_{i \in [n]} X_{i,(1)} = s}\Pr{\argmax_{i \in [n]} X_{i,(1)} = s \given X_{\max} = t}.
		\end{align*}
		Due to symmetry, we know $\Pr{\argmax_{i \in [n]} X_{i,(1)} = s \given X_{\max} = t}$ is exactly equal for $s \in [n]$, and it does not change with respect to $t$.
		In addition, given $X_{s,(1)} = t $ and $\argmax_{i \in [n]} X_{i,(1)} = s$, in $\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}}$, only the terms $\prod_{j=2}^k\parans{1 - \frac{A_{s,j}}{2}}$ changes with respect to $t$.
		Given $X_{s,(1)} = t $, we can rewrite it as
		\begin{align*}
			\prod_{j=2}^k\parans{1 - \frac{A_{s,j}}{2}} = \prod_{j=2}^k \parans{1- \parans{\frac{X_{s,(j)}}{t}}^{k(n-1)}},
		\end{align*}
		and it is obviously an increasing function with respect to $t$.
		Combining the results, we conclude that $g(t)$ is an increasing function on $t$.
	\end{proof}
        Rewriting the expectation based on $X_{i,j}$ and applying FKG inequality similar to the proof of Theorem~\ref{thm:bayes_oblivious}, we obtain
	\begin{align*}
		\eqref{ineq:01062038}
		&\ge
		\parans{\int_{t=0}^1 \Ex{\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}} \given X_{\max} = t} \Pr{X_{\max} = t} t} \cdot \parans{ \int_{t=0}^1 t \Pr{X_{\max} = t} dt}
		\\
		&=
		\Ex{\prod_{i=1}^n \prod_{j=2}^k \parans{1 - \frac{A_{i,j}}{2}}} \Ex{X_{\max}}
		\\
		&=
		\Pr{E}\cdot \Ex{X_{\max}}.
	\end{align*}

        \paragraph{Obtaining a lower bound on $\Pr{E}$}
        Now it remains to lower bound the probability $\Pr{E}$, which is already given in \eqref{ineq:01062049}.
	Hence, we conclude that the principal's expected utility under this BCE is at least
	\begin{align*}
		\exp\parans{- \frac{n^2}{2(n-1)^2}}\Ex{X_{\max}},
	\end{align*}
	and it completes the proof.
\end{proof}


\subsection{Proof of Theorem \ref{theorem:multi-agent-correspondence}}\label{pf_theorem:multi-agent-correspondence}
\begin{proof}
We start by presenting the following lemma from~\citet{kleinberg2018delegated}.
\begin{lemma}[\citet{kleinberg2018delegated}]\label{thm:singleagent_revel}
In the single-agent setting, for any mechanism $M$ and corresponding dominant strategies $\sigma$, there exists a MSPM such that for any equilibrium strategies $\sigma'$, we have $x(f_{M,\sigma}(\omb)) = x(f_{SPM,\sigma'}(\omb))$ for any $\omb \in \Omega^*$.
\end{lemma}
% This corresponds to a celebrated revelation principal~(cite) in mechanism design literature.
% It is important to note that any SPM requires an examination budget of $1$, since it only evaluates a single candidate from a single agent.
% This implies that there is no merit in having a large examination budget against single-agent.
% This is fairly intuitive because, in a single-agent setting, the agent does not have any incentive to signal more than two candidates since he knows that only one of them would be eventually selected.
By the lemma, it suffices to consider the case when $M$ is a SPM.
Let the realized solutions in $P$ be $\omb = \{\om_1, \om_2,\ldots, \ldots \om_k\}$. Consider a partition of $\omb$ as follows
\begin{align*}
	\omb_{1} &= \{\om_1,\ldots, \om_{k_1}\}
	\\
	\omb_{2} &= \{\om_{k_1+1},\ldots, \om_{k_1+k_2}\}
	\\
	&\vdots
	\\
	\omb_{n} &= \{\om_{k_1+\ldots+k_{n-1}+1},\ldots, \om_{k_1+\ldots + k_n=k}\}.
\end{align*}
Suppose that agent $i$'s realization of solutions in $P'$ is $\omb_{i}$ so that the outcomes of $P$ and $P'$ are coupled. 
This coupling is indeed possible because the probability that agent $i$'s solutions are realized to be $\omb_i = \{\om_{i_1},\ldots, \om_{i_{k_i}}\}$ is exactly equal to the marginal probability that $\om$'s $i$-th partition is realized to be $\omb_i = \{\om_{i_1},\ldots, \om_{i_{k_i}}\}$.

Consider a SPM with an eligible set $R$ under $P$, and corresponding equilibrium strategies $\sigma$.
Denote by $x$ and $y$ the principal and the agent's utility function under $P$ respectively.
Given the solutions realized as above, SPM will select the solution which maximizes $y(\om_j)$ for $j \in [k]$ such that $\om_j \in R$, \ie $\om_1^* = \argmax_{j \in [n], \om_j \in R} y(\om_j)$.
Let this solution be $\om_1^*$.
Now consider a MSPM with arbitrary tie-breaking rule and the same eligible set $R$ under $P'$, and suppose that the agents play equilibrium strategies $\sigma'$.
Let $\om_2^*$ be the corresponding winner in this case.
% Let $A$ be a set of solutions that can be selected as a winner in the MSPM under $P'$.
% Note that $A$ might include multiple solutions since the examination process is randomized in RSPM.
% For any $\om_2^* \in A$, 

We want to show that $x(\om_2^*) \ge x(\om_1^*)$  for any realization of solutions $\omb$.
Suppose not.
It is obvious that both $x(\om_1^*)$ and $x(\om_2^*)$ belong to the eligible set $R$.
If $\om_1^*$ and $\om_2^*$ belongs to the same partition $\omb_i$, it means that agent $i$ has both the solutions $\om_1^*$ and $\om_2^*$.
By our definition on $\om_1^*$ such that $\om_1^* = \argmax_{j \in [n], \om_j \in R} y(\om_j)$, submitting $\om_1^*$ is gives the better or the same utility for agent $i$.
If $y(\om_1^*) > y(\om_2^*)$, then simply submitting $\om_1^*$ gives a strictly better utility for agent $i$, and it contradicts that $\sigma'$ is equilibrium strategy.
If $y(\om_1^*) = y(\om_2^*)$, then $x(\om_1^*) \le x(\om_2^*)$ by Assumption~\ref{as:pareto}.
Hence, $x(\om_1^*) \le x(\om_2^*)$ in both cases.

Now suppose that $\om_1^*$ and $\om_2^*$ belongs to the different partitions $\omb_i$ and $\omb_j$.
Suppose that agent $i$'s equilibrium strategy satisfies $\sigma'_i \neq \om_1^*$.
If playing $\omb_i$ is strictly better for agent $i$, it contradicts that $\sigma'_i$ is an equilibrium strategy.
Hence $y(\om_1^*) = y(\sigma_i')$. Again by Assumption~\ref{as:pareto}, since agent $i$ plays $\sigma_i'$, we have $x(\sigma'_i) \ge x(\om_1^*)$.
Note that the principal should observe both $\sigma_i'$ and $\om_2^*$, and commits to $\om_2^*$.
This implies that $x(\om_2^*) \ge x(\sigma_i') \ge x(\om_1^*)$, and we finish the proof.
\end{proof}

==> Delegating to Multiple Agents (1)/setup.tex <==
% !TEX root =  main.tex
\section{Problem setup}
\label{sec:setup}
\vspace{-2mm}\xhdr{Multi-agent delegation.}
Consider a \emph{principal} who designs a delegation mechanism and a~set of $n$ \emph{agents} who perform the task and decide solutions.
Let $\Omega$ be a set of potential solutions.
% , i.e.
% any solutions found by any agent belong to this set.
Each agent is equipped with a number of solutions $k_i \in \N$, and each solution $j$ for $j \in [k_i]$ is sampled from a probability distribution $D_{i,j}$ supported on $\Omega$.
We assume that $k_i \ge 2$ for $i \in [n]$ to avoid trivial regime.
% and finds $k_i$ solutions by independently sampling from $k_i$ probability distributions $D_{i, 1}, D_{i, 2}, ..., D_{i, k_i}$ supported on $\Omega$.
Each distribution $D_{i,j}$ may refer to
the potential quality of the $j$th solution of agent $i$, and the number of solutions $k_i$ can be interpreted as the agent's willingness-to-pay in terms of his effort, both of which are exogenous to the mechanism.
% The number $k_i$ can be interpreted as
% the agent's willingness-to-pay in terms of his effort, i.e.
% if $k_i$ is large he exerts high effort on the task and
% finds a large number of solutions, and vice versa.
% We assume that both $k_i$ and $\{D_{i, j}\}_{j \in [k_i]}$ are exogenous parameters for each $i \in [n]$, and thus are not affected by the mechanism.
% Note that we use $[n]$ to denote $\{1,2,\ldots, n\}$ throughout the paper.
We denote by $\om_{i,j} \in \Omega$ the agent $i$'s $j$-th solution for $i \in [n],j \in [k_i]$, and $\omb_i$ the agent $i$'s multi-set of all solutions.
We further use  $\omb = \cup_{i \in [n]}\omb_i \in \Omega^*$ to denote the multi-set of all the solutions sampled by the agents.
After agent $i$ observes his own solutions $\omb_i$, he sends a signal to the principal, and then the principal finally adopts one of the solutions based on the agents' signals.
%We provide tangible examples for what can possibly considered as a reasonable mechanism and corresponding signaling strategies in Discussion~\ref{disc:beyondmspm}.

%Each agent $i$ tries to seek a solution in $\Omega$, but he cannot find arbitrary number of solutions as much as he wants, since this procedure requires him to exert efforts on it.
%Instead, he has an exogenous parameter of willingness-to-pay in terms of his effort, and this translates to a unique number of solutions $k_i$ that the agent can find.
%These solutions are independently and identically sampled from a distribution $D_i$ supported on $\Omega$, which can be translated as the agent's skill since it denotes how the solutions found by agents are distributed.

For notational consistency, let \emph{solution} denote an outcome observed by an agent, \emph{candidates} to denote the set of solutions that the mechanism can access given the agents' signals, \emph{winner} to denote the final solution adopted by the principal.
We further say our problem to be \emph{single-agent} problem if $n=1$, and \emph{multi-agent} problem if $n \ge 2$.

\paragraph{Mechanism}
A \emph{mechanism} $M = (\Sigma, f, S)$ is specified by a set of signals $\Sigma = \Sigma_1 \times \ldots \times \Sigma_n$ of which the $i$-th coordinate $\Sigma_i$ corresponds to the signal from agent $i$, a set of possible random bits $S$ of the mechanism, and an allocation function $f: \Sigma \times S \mapsto \Omega$ which denotes the winner selected by the principal given the signals by agents and the random bits.
If the mechanism is deterministic, we overwrite the domain of the allocation as $f: \Sigma \mapsto \Omega$.
We mostly deal with a deterministic mechanism but introduce a general definition for completeness.
For some given random bits $s \in S$, we denote by $M_s$ the mechanism in which its random bits are fixed to be $s$. 
Note that we use a generalized notion of signal to denote any possible interaction from the agents to the principal.
For example, agent $i$ may simply propose a subset of his observed solutions as candidates, or he may exploit a mixed strategy of proposing solutions randomly.
Throughout the paper, we use $\Omega^*$ to denote a family of all finite multi-set over $\Omega$.
% , e.g. $\{\om\} \in \Omega^*,\forall \om \in \Omega$ and $\{\om, \om'\} \in \Omega^*,\forall \om,\om' \in \Omega$ and so on so forth.
% Due to our use of the multi-set, even if the same solution $\om$ is observed by more than one agent, we distinguish each solution and its owner.



% Same Distribution for all samples of an agent
% \suho{For now, just define $\Sigma_i$ be a family of sequence of samples from $\Omega^*$.}
% \paragraph{Agent's strategy}
% Each agent $i$ selects such a signal based on a strategy $\sigma_i:\Omega^* \mapsto \Sigma_i$, which can be interpreted as for each agent $i$, given a set of multi-set of the $k_i$ solutions $\omb_i = \{\om_{i,1},\ldots, \omega_{i,k_i}\}$ sampled from $D_i$, he sends a signal, i.e. strategy, $\sigma(\omb_i)$ to the principal.
% \suho{Mention that $\Sigma$ can be $\Delta(\Omega)$, i.e. a distribution over the observed solutions, so that he plays a mixed strategy}
% We assume that there exists no coalition between the agents.
% If the winner $\om$ belongs to some agent $i$'s solutions $\omb_i$, then the principal's utility is $x(\om)$, agent $i$'s utility is $y_i(\om)$, and the other agent $j$'s utility is $0$.
% As defined above, in case of a null outcome, i.e. if all the outcomes are rejected, then all the players' utilities are $0$.
% If the winner $\om$ does not belong to $\cup_{i \in [n]} \omb_i \cup\{\perp\}$, then the principal receives utility $0$ and all the agents have utility $-1$.
% This restricts the winner to be selected within the solutions $\cup_{i \in [n]} \omb_i \cup\{\perp\}$, which is consistent with our assumption that the principal has no ability to directly sample from distributions $D_i$, thus delegates this task to the agents and selects among their candidates.
%Let $\omega^*  = \cup_{i \in [n]} \omega^*_i$ be a set of solutions probed by the agents, and let $\set{F}$ be a family of feasible sequence of realized samples so that $\omega^* \in \set{F}$.

\paragraph{Agent's strategy} 
% \keivan{we must mention that agent strategy is not only a function of his observations, but also a function of other knowledge he has regarding others' dist/solutions}
Each agent $i$ selects a certain signal based on a \emph{strategy} $\sigma_i:\Omega^* \mapsto \Sigma_i$.
More formally, given a multi-set of the $k_i$ solutions $\omb_i = \{\om_{i,1},\ldots, \omega_{i,k_i}\}$, agent $i$ sends a signal $\sigma(\omb_i)$ to the principal.
Importantly, agent $i$ determines the strategy based on the information regarding the others' solutions as well as his own solutions.
We elaborate more in the subsequent paragraph.
The principal has a utility function $x:\Omega \mapsto \R_{> 0}$ and
each agent $i$ for $i \in [n]$ has a utility function $y_i:\Omega\mapsto \R_{> 0 }$.
If solution $\omega \in \omb$ is selected as the winner and $\om$ belongs to agent $i$, then the principal and agent $i$ realize utilities of $x(\omega)$ and $y_i(\omega)$ respectively.
The other agents $j\neq i$ realize their utility to be zero.
Note that we restrict the winner to be within $\omb$ so that the principal cannot commit to a solution beyond the observed set of solutions.
We further assume that $\Omega$ includes a null outcome $\perp$.
If the principal selects $\perp$ as the winner, this represents that no solution is adopted by the principal and the realized utility is zero, \ie $x(\perp) = y_i(\perp) = 0$ for $i \in [n]$.
% \keivan{Fix prophet lower bound to delta}
% Otherwise, we assume that both the principal and agents have positive utility, i.e. $x(\om),y_i(\om) > 0$ for any $\om \in \Omega \setminus \{\perp\}$ for any $i \in [n]$.

% If the winner $\om$ belongs to agent $i$'s solutions $\omb_i$, then the principal's utility is $x(\om)$, agent $i$'s utility is $y_i(\om)$, and the other agent $j$'s utility is zero.
% Note that all the players' utilities are zero if the principal does not adopt any solution.
% For the completeness of the model, we assume that
% If the winner $\om$ does not belong to $\cup_{i \in [n]} \omb_i \cup\{\perp\}$, then the principal receives utility $0$ and all the agents have utility $-1$.
% This restricts the winner to be selected within the solutions $\cup_{i \in [n]} \omb_i \cup\{\perp\}$,
% which is consistent with our assumption that the principal has no ability to directly sample from distributions $\{D_{i, j}\}_{j \in [k_i]}$,
% thus delegates the task to the agents.

% Define $x_{i,(j)}$ and $y_{i,(j)}$ denote hte index of $j$-th highest solutions of agent $i$ in terms of $x_i$ and $y$, respectively.
%In addition, let $x_{i | \tau}$ be the index of smallest solution of agent $i$ satisfying $X_{i,j} \ge \tau$, and define $y_{i| \tau}$ similarly.

\paragraph{Information structure}
In terms of the principal's information for agents' distributions of solutions, we consider the following two types of mechanism.
\begin{definition}[Bayesian and prior-independent mechanism]
	We say that mechanism $M$ is \Emph{prior-independent mechanism} (PIM), if it does not have any information on the distributions from which the solutions are drawn.
	If it priorly knows the distribution from which the quantity $x(\cdot)$ over the solutions are drawn for each agent,
%	\footnote{This is in contrast to \citet{kleinberg2018delegated}, where they often assume that the principal is aware of the distributions for both $x(\cdot)$ and $y(\cdot)$} 
	we denote by \Emph{Bayesian mechanism} (BM).
\end{definition}
Importantly, as noticed in the definition, PIM has significant informational gain over BM.
It does not require any process of acquiring information on the distribution of solutions.
Indeed, in practice, it is difficult or even impossible to estimate the distribution of each agent in advance.
Even if it's possible, it usually entails a costly procedure to acquire such information, and thus PIM is more broadly applicable.

Regarding the principal's information on the agents' solutions, we consider an information asymmetry arises from \emph{moral hazard} such that the principal has no information on the realized set of solutions since she delegates the search (choice) to the self-interested agents.
Instead, she can only access a subset of solutions based on the signals provided by the agents.

To model the agent's information structure, we basically assume that the agents know the principal's utility function.
Furthermore, we consider two cases of complete information and incomplete information based on the agent's information with respect to the others.
In the \Emph{complete information} setting, all the observed solutions are revealed to each other, thereby each agent determines his own strategy after observing all the solutions.
In the \Emph{incomplete information} setting, only the distributions of the solutions are publicly available to the agents but not the exact observed solutions, and thus each agent determines his own strategy based on the given knowledge of the others' distributions.
% Note that the incomplete information setting corresponds to the Bayesian game which entails an intrinsic challenge in analyzing mechanisms and equilibriums.
% Nevertheless, we provide several positive results in this setting in Section~\ref{section:no_cost_incomp} as well as in the complete information setting Section \ref{section:no_cost}.


\paragraph{Allocation function and overall mechanism}
We first define an interim allocation function which represents the winner adopted by the mechanism given the observed set of solutions.
\begin{definition}[Interim allocation function]
$f_{M,\sigma}: \Sigma \mapsto \Omega$ is an (interim) allocation function given mechanism $M$ and strategy $\sigma$.
That is, given $\omb = \cup_{i \in [n]}\omb_i$, the mechanism $M$ selects $f_{M,\sigma} (\omb)$ as the winner when each agent $i$ plays $\sigma_i$.
In case of randomized mechanism,  we use $f_{M_s, \sigma}$ to denote the allocation function given the random bits $s$, and $F_{M,\sigma}$ to denote the set of possible winners $\cup_s f_{M_s, \sigma}$.
\end{definition}
% Note that we can compute the principal's and agent $i$'s expected utility by $\Ex{x(f_{M,\sigma})}$ and $\Ex{y_i(f_{M,\sigma})}$ for each $i \in [n]$, where the expectation is taken over the randomness in the solutions and the mechanism.
% Same distribution for all samples of an agent
% Overall, the mechanism proceeds as follows.\note{put a figure instead of it}
% \begin{enumerate}
% \item The principal commits to a mechanism $M$.
% \item Each agent $i$ observes $k_i$ solutions $\omb_i$ from distributions $D_i$.
% \item Each agent $i$ strategically send a private signal $\sigma_i$ based on $M$ given $\om = \cup_{i \in [n]}\omb_i$.
% \item The principal selects the winner $f_{M,\sigma}$.
% \end{enumerate}
Overall, the mechanism proceeds as follows: (1) the principal commits to a mechanism $M$, (2) each agent $i$ observes solutions $\omb_i$, (3) each agent $i$ strategically sends a private signal $\sigma_i$, and (4) the principal selects the winner $f_{M,\sigma}$ (or $f_{M_s, \sigma}$).
% \begin{enumerate}
% \item The principal commits to a mechanism $M$.
% \item Each agent $i$ observes solutions $\omb_i$.
% \item Each agent $i$ strategically sends a private signal $\sigma_i$.
% \item The principal selects the winner $f_{M,\sigma}$ (or $f_{M_s, \sigma}$).
% \end{enumerate}

\subsection{Further preliminaries}
We here present further notations that will be broadly used throughout the paper.
\begin{definition}[Nash equilibrium]
	Given a mechanism $M$, a set of strategies $\sigma = (\sigma_1,\sigma_2,\ldots, \sigma_n)$ is called a \emph{Nash equilibrium}, if $\sigma_i$ yields
	\begin{align}
		y_i(\sigma_i, \sigma_{-i})
		\ge
		y_i(\sigma_i', \sigma_{-i}),\label{ineq:01251707}
	\end{align}
	for agent $i$'s any other strategy $\sigma'_{i}$ given the others' strategy $\sigma_{-i}$.
	We call each $\sigma_i$ an equilibrium strategy of agent $i$. We often abuse equilibria or equilibrium to denote Nash equilibrium.
    Whenever the mechanism is randomized, we take expectation over the utility in~\eqref{ineq:01251707}.
\end{definition}

%\begin{definition}[Dominant strategy equilibrium]
%\suho{We may not need to define it}
%Given a mechanism $M$, we say that agent $i$ has dominant strategy $\sigma_i$ if $\sigma_i$ yields
%\[
%y_i(f_{M, (\sigma_i,\sigma_{-i})}) \ge y_i(f_{M, (\sigma'_i, \sigma_{-i})}),
%\]
%for agent $i$'s any other strategy $\sigma'_i$ regardless of the other's strategy $\sigma_{-i}$.
%If there exists a dominant strategy $\sigma_i$ for every agent $i \in [n]$, we call it a dominant strategy equilibrium.
%\end{definition}
%In a dominant strategy equilibrium, each player has no incentive to deviate regardless of the other's strategy $\sigma_{-i}$, however in a Nash equilibrium, it has no incentive to deviate assuming that the others play equilibrium strategies $\sigma_{-i}$.
%Note that a dominant strategy equilibrium implies a Nash equilibrium.

% Now we define a notion of examination cost and budget of delegation mechanism.
%
%\begin{definition}[Price of anarchy]
%Price of anarchy $PoA$ of mechanism $M$ denotes the worst-case ratio between the principal's expected payoff under the standard multi-agent setting and that under the case in which the set of agents cooperates with unlimited communication.
%\end{definition}
%Price of anarchy larger than $1$ means that there exists a loss 
For sake of exposition, we define $X_{i,j} = x(\om_{i,j})$  and $Y_{i,j} = y_i(\om_{i,j})$ for each $j \in [k_i]$ and $i \in [n]$. 
Furthermore, we denote by $X_{i,(j)}$ the $j$-th highest solution in $\om_i$ in terms of $x(\cdot)$ so that $X_{i,(1)} \ge X_{i,(2)} \ge \ldots \ge X_{i,(k_i)}$ and 
define $Y_{i,(j)}$ the agent $i$'s utility for the solution that corresponds to $X_{i,(j)}$.
We often overwrite $X_{i,(1)}$ by the \emph{first-best solution} of agent $i$, and the agent who has $X_{(i)}$ by \emph{$i$-th best agent}.
Note that $X_{i,j}$ and $Y_{i,j}$ for each $j \in [k_i]$ and $i \in [n]$ are random variables such that $X_{i,j}$ and $Y_{i,j}$ are correlated with respect to $\om_{i,j}$.
%In addition, we define a rank of an agent as follows.
%\begin{definition}[Agent's rank]
%\keivan{do we still need Rank? we need $X_{(i)}$ btw, which is already presented in Section 2.} \suho{I don't think so. Let's remove it after confirm. This section needs to be self-contained, but we can cherry-pick some def of notations from contribution section.}
%Given $X_{1,(1)}, \ldots, X_{n,(1)}$, let $\phi$ be a permutation on $[n]$ such that $X_{\phi(1),(1)} \ge X_{\phi(2), (1)} \ge \ldots \ge  X_{\phi(n),(1)}$.
%We say that agent $i$ has rank $r$ if $i = \phi^{-1}(r)$ for $i \in [n]$, and denote this agent by $r$-th best agent.
%\end{definition}

We measure the principal's utility by comparing it to a strong benchmark $\opt$ given a realized set of solutions $\omb$, defined formally as follows.
\begin{align*}
\opt= \Ex{\max_{\om \in \omb} x(\omega)} = \Ex{\max_{i \in [n]} \max_{j \in [k_i]} X_{i,j}}.
\end{align*}
We often abuse $X_{\max} = X_{(1)} = \max_{i \in [n]} \max_{j \in [k_i]} X_{i,j}$.
Note that $\opt$ denotes the principal's utility when she can access all the solutions sampled by the agents, and select the best solution by herself.

In terms of the approximation ratio of the mechanism, we consider both the additive and multiplicative approximation factors, defined as follows.
\begin{definition}
    \label{def:apx-mech}
	Mechanism $M$ and corresponding strategies $\sigma$ are $(\rho,\gamma)$-approximate if
	\begin{align*}
		\rho\Ex{f_{M,\sigma(\omb)}} + \gamma
		\ge
		\opt.
	\end{align*}
\end{definition}
% Note that $\rho$ and $\eps$ correspond to the multiplicative and additive approximation factors, respectively.
% We say that a mechanism has a \emph{delegation gap} of $\gamma$ if it is $(1,\gamma)$-approximate.
Note that the expectation in LHS is taken over the randomness in $M$ as well as that in solutions.

Since we deal with the approximation factor of the mechanism in its equilibrium, we further define the notion of the price of anarchy and the price of stability as follows.
\begin{definition}[Price of anarchy/stability]
    \label{def:poa-pos}
    Mechanism $M$ has multiplicative \emph{price of anarchy} ($\poa_m$) of $\rho$ if it is $(\rho,0)$-approximate under any equilibrium.
    It has multiplicative \emph{price of stability} ($\pos_m$) of $\rho$ if there exists an equilibrium such that $M$ is $(\rho,0)$-approximate.
    We similarly define $\poa_a$ and $\pos_a$ to denote the price of anarchy/stability for the additive approximation factor $(1,\gamma)$.
\end{definition}

% Since the expected payoff of the principal depends on the order in which the candidates are examined, we consider a worst-case payoff of the principal such that the principal's payoff is computed against an adversarial order of examining the candidates.
% For example, the mechanism can specify an ordering between the agents and inspect each items randomly within the agent based on the ordering.
% On the other hand, the mechanism may just randomly permute all the items

% \begin{definition}[Delegation gap]
% \todo{change terminologies as needed}
% We say that a mechanism $M$ has $c$-delegation gap, if under any Nash equilibrium $\sigma$, the principal's expected utility is at least $1/c$ times the expected utility of the case in which the principal herself selects an outcome from the entire set of realized samples.
% Formally, $M$ has $c$-delegation gap, if for any Nash equilibrium $\sigma$ we have
% \begin{align*}
% \Ex{f_{M,\sigma}(\omb)} \ge 1/c \cdot \textsc{Opt},
% \end{align*}
% and there exists at least one Nash equilibrium.
% \end{definition}

%\begin{definition}[Delegation gap]
%	We say that a mechanism $M$ has delegation gap of $G$,
%	if under some strategies $\sigma$,
%	the difference between principal's expected utility and and $\opt$ is at most $G$.
%	Formally, $M$ has delegation gap of $G$, if under the strategies $\sigma$ we have
%	\begin{align*}
%	\opt - \Ex{f_{M,\sigma}(\omb)} \le G.
%	\end{align*}
%\end{definition}
%
%On contrary, the expectation in $\opt$ is taken only over the randomness in solutions $\omb$.
%Note that the delegation gap corresponds to the additive approximation factor. 
%In addition to the delegation gap, we often use the multiplicative approximation factor in presenting our several results, mostly when we compare the multi-agent delegation mechanism to the single-agent delegation mechanism of \cite{kleinberg2018delegated}.
%More formally, we say that a mechanism $M$ is $\alpha$-\emph{approximate} if $\alpha \Ex{f_{M,\sigma}(\omb)} \ge \opt$.

For self-containedness, we present the mechanism introduced by \citet{kleinberg2018delegated}.
\begin{definition}[Single-proposal mechanism]
In a single-proposal mechanism (SPM) under the single-agent setting, an eligible set $R \subset \Omega$ is announced by the principal, the agent proposes a~solution $\om$, and the principal accepts it if $\om \in R$, and rejects it otherwise.
\end{definition}

% \begin{theorem}[\cite{kleinberg2018delegated}]
% In the single-agent setting, the following results hold.
% \begin{enumerate}
% 	\item If the principal cannot observe the agent's utility, there exists a SPM with an eligible set that achieves $(2,1)$-approximation.
% 	\item Furthermore, if the principal and agent have independent utilities, each drawn from an atomless distribution, there exists a SPM with an eligible set that achieves $(\frac{e}{e-1},1)$-approximation.
% 	\item In the same setting as (2), but if the principal can observe the agent's utility, there exists a SPM with an eligible set that achieves $(\frac{1}{\alpha - \mO(\log n/n)},1)$-approximation, where $\alpha \approx 0.745$ is a solution of $\int_0^1(y - \ln y + 1 - 1/\alpha)^{-1}dy = 1$  
% \end{enumerate}
% \end{theorem}

% They quantify the approximation ratio of SPM with some eligible sets in various problem settings.
% Their proof mainly relies on the novel connection between the principal's utility in the single-proposal mechanism and the approximation ratio of various stopping rules in continuous-time prophet inequalities.

% \begin{proof}
% For any mechanism $M$ and corresponding dominant strategies $\sigma$, consider a fixed sequence of realized samples $\omega^* \in \set{F}$.
% Let $\set{R}_{\omega^*}$ be the range of $f_{M,\sigma}$ and $y$ be the utility function of the agent.
% Consider a single-proposal mechanism $M'$ with eligible set $R = \cup_{\omega^* \in \set{F}} R_{\omega^*}$.
% Define $\omega$ be a candidate which maximizes the agent's utility among $\set{R}_{\omega^*}$, i.e. $y(\omega) \ge y(\omega')$ for any $\omega' \in \set{R}_{\omega^*}$.
% If there exists $\omega' \in \set{R}_{\omega^*}$ such that $y(\omega') < y(\omega)$, consider a restricted strategy $\sigma'$ in which for any sequence of samples $\omega^*$, whenever $f_{M,\sigma}(\omega^*) = \omega'$, define $\sigma'(\omega^*) = \omega$.
% Then it is obvious that $\sigma'$ has strictly larger payoff, which contradicts the assumption.
% Take a maximal utility candidate in terms of the principal, i.e. $\omega_x = \argmax_{\omega \in \set{R}_{\omega^*}} x(\omega)$, then $y(\omega_x)= y(\omega')$ for any $\omega' \in \set{R}_{\omega^*}$.
% Let $\sigma_x$ be a pure strategy which only submits $\omega_x$. 
% Under $M'$, if there exists dominant strategies $\sigma_{M'}$ such that $\sigma_{M'}$ yields strictly larger payoff than $\sigma_x$, then this strategy also has strictly larger payoff than $\sigma_x$ under $M$.
% Hence $\sigma_x$ is dominant strategies under $M'$, and we also have $x(f_{M',\sigma_x}(\omega^*)) = x(\omega_x) \ge x(f_{M, \sigma_M}(\omega^*))$.
% This completes the proof.
% \end{proof}

In our multi-agent setup, we mainly investigate a variant of the SPM defined as follows.
\begin{definition}[Multi-agent single-proposal mechanism]\label{def:mspm}
In a \emph{multi-agent single-proposal mechanism (MSPM)}, a tie-breaking rule $\rho$ and an eligible set $R_i \subset \Omega$ are announced by the principal for each agent $i$.
Each agent proposes up to one solution, and the principal filters a candidate from agent $i$ if it is not contained in $R_i$.
After filtering, the principal selects the winner by choosing the candidate that maximizes her utility, given the tie-breaking rule $\rho$.
We say that MSPM has a homogeneous eligible set if $R_i = R$ for $i \in [n]$.\footnote{We provide further examples of reasonable mechanisms in Appendix~\ref{sec:fur_fea_mec}.}
\end{definition}
%\begin{discussion}\label{disc:beyondmspm}
%    Another reasonable choice of mechanism will be to require each agent submitting certain number, say two, of solutions, \ie multi-proposal mechanism.
%    Under this mechanism, each agent might select a pair of aggressive solution with large ex-post utility but smaller chance to be selected, and conservative solution with small ex-post utility but larger probability of winning, in order to balance these features of two solutions.\footnote{More abstractly, one may consider a mechanism that requires each agent to signal some statistics of the observed solutions, \eg sample average or the number of eligible solutions, upon the solutions themselves.}
%    As astute readers may have noticed, in the complete information setting, however, the revelation principle style of result allows us to reduce any mechanism to single-proposal mechanism, so such generalization does not help. This is formalized in Theorem~\ref{thm:multiagent_revel}.
%\end{discussion}

\begin{remark}\label{rm:bm_pim_comp}
Importantly, in terms of the principal's information, MSPM can be both BM and PIM depending on the eligible set $R_i$.
If we specify $R_i$ to admit any solution from $\Omega$, then it is PIM as we do not need any kind of prior knowledge on the solution.
However, if we want to specify $R_i$ to accept only a certain type of solution as in SPM by \citet{kleinberg2018delegated}, then we essentially need the prior information regarding the distribution of the solution.
This is indeed true because if we commit to an eligible set that possibly rejects some solutions without knowing the distribution of the solutions, then it is obvious that we can construct a worst-case problem instance in which the mechanism essentially cannot accept any solution, resulting in an arbitrarily bad approximation factor. We refer to Claim~\ref{cl:3} in Appendix~\ref{pf_thm:comp_obl_neg} for a  formal discussion.
\end{remark}

Finally, we pose a (minor) assumption that if an agent is indifferent between two solutions, he selects a solution that induces a higher utility for the principal.
\begin{assumption}[Pareto-optimal play]\label{as:pareto}
If an agent has two solutions $\om$ and $\om'$ such that $x(\om ) \ge x(\om')$, $y(\om) \ge y(\om')$ and at least one of these inequalities are strict, then the agent does not play strategy $\sigma_i = \om'$.
\end{assumption}
\begin{remark}
This assumption is reasonable since there exists no merit in playing such a dominated strategy $\om'$.
Moreover in practice, the agents may also want to behave in favor of the principal as much as possible unless they need to sacrifice their own utilities, for any future interactions.
\end{remark}
Before presenting our main results, we begin with the following observation that any mechanism can be reduced to MSPM with the proper choice of parameters.
\begin{theorem}\label{thm:multiagent_revel}
In the multi-agent setting, for any mechanism $M$ with an arbitrary equilibrium $\sigma$, there exists a MSPM $M'$ such that for any equilibrium $\sigma'$, for any $\om \in F_{M,\sigma}(\omb)$ and any $\om' \in F_{M',\sigma'}(\omb)$, we have $x(\om) \le x(\om')$ for any observed solutions $\omb \in \Omega^*$.
\end{theorem}
The proof is provided in Appendix \ref{pf_thm:multiagent_revel}.
Thanks to the theorem, it suffices to narrow down our scope of interest to the set of MSPMs.
Correspondingly, we focus on analyzing the approximation factor of MSPM in both the complete and incomplete information settings.

% This theorem implies that if all agents believe that the principal has enough power to examine all the submitted candidates, each agent proposes at most one candidate.
% Intuitively, the belief that the principal would thoroughly examine all the candidates induces the agents to behave more truthfully to report a single solution, i.e. propose a single good solution in terms of the principal.

% Moreover, if we assume that the agents behave in favor of the principal whenever they are indifferent between two solutions, then the above theorem holds for any equilibrium of the mechanism.
% \begin{corollary}
% Suppose that if an agent has two solutions $\om$ and $\om'$ such that $x(\om ) \ge x(\om')$, $y(\om) \ge y(\om')$ and at least one of these inequalities are strict, then the agent does not play strategy $\sigma_i = \om'$.
% In this case, Theorem~\ref{thm:multiagent_revel} can be strengthened so that the statement satisfies for any equilibrium strategies in $M$'.
% \end{corollary}
% This assumption is reasonable since each agent knows the principal's utility, and thus does not have any incentive to play such a dominated $\om'$, instead it is practical to assume that the agent will behave to satisfy the principal for any possible economical interaction.





% We recall that in $k$-proposal mechanism, an eligible set $R$ is announced in advance as a threshold to accept the candidates.
% If an agent nevertheless submits a sample outside the eligible set $R$ even though knowing that this will be rejected in anyway, it only increases an examination cost of the mechanism and does not benefit neither the agent and principal.
% Hence, we make an assumption that in proposing candidates, each agent excludes samples which are obvious to be rejected by the principal.
% More formally, we define the following assumption of minimal proposal.
% \suho{This assumption is not necessary. Instead, we can make our theorem statement as "Given $M$, there exists a equilbrium such that $M$ is $(a,b)$-approximation."}
% \begin{assumption}[Minimal proposal]
% Given a mechanism $M$, for any strategy $\sigma_i$ of agent $i$, if there exists a strategy $\sigma'_i$ in which $|\sigma'_i| < |\sigma_i|$, $\sigma_i' \subset \sigma_i$, and $\sigma'_i$ is best response to $M$ regardless of the others' strategy $\sigma_{-i}$, then agent $i$ does not play $\sigma_i$.
% \end{assumption}












==> bck/bayes_recover.tex <==
% \begin{proof}
% 	The overall proof is exactly same as that of Theorem \ref{thm:recover}.
% 	In the proof of Theorem \ref{thm:recover}, we only used Assumption~\ref{as:pareto},
% 	and the fact that principal selects the best proposed solution as the winner.
% 	As both of those asuumptions still hold in incomplete information settings, we can follow the same proof to get the same result.
% 	However, we provide the proof for completeness. \keivan{should we really put the proof here? it is exactly same.}

	% Consider a problem instance of multi-agent settings where $n$ agents propose solutions.
	% In order to find solutions, Agent $i$ samples $k_i$ times from distribution $D_i$.
	% We construct a single-agent problem instance
	% where the only agent samples $k_i$ times from each distribution $D_i$, $\sum_{i=1}^{n} k_i$ samples on aggregate.
	% According to \citet{kleinberg2018delegated}, there exists an SPM with proper eligible set $R$ under the constructed settings such that
	% principal's expected utility is at least $\frac{1}{2}\Ex{X_{(1)}}$.
	% We use the same eligible $R$ in designed SPM for all agents in multi-agent settings.
	% We claim that for any realization of solutions $\omb = \cup_{i=1}^{n} \omb_i$,
	% principal's utility in multi-agent setting is at least that of single-agent setting which further implies that
	% using same eligible set $R$, principal's expected utiltiy in multi-agent settings is at least $\frac{1}{2}\Ex{X_{(1)}}$.
	% \keivan{Should I elaborate on single-agent utility function?}

	% Consider a realization of solutions $\omb$. Let $\omega$ be the winner in single-agent setting.
	% If $\omega = \perp$, then all observed solutions are not eligible.
	% Formally, for all $i$ in $\left[n\right]$, and $j$ in $\left[k_{i}\right]$:
	% $\omega_{i, j} \notin R$. In this case, there is not any eligible solution in multi-agent setting as well which
	% indicates that prinicpal utiltiy in both settings is zero.
	% On the other hand, if $\omega \neq \perp$, let $\omega^*$ be the winner in multi-agent setting, we claim that $x(\omega^*) \geq x(\omega)$.
	% Denote by $i$ the agent who has sampled $\omega$. Denote by $\sigma_i$ the solution proposed by agent $i$ in multi-agent setting.
	% As both $\sigma_i, \omega \in R$, and $\omega$ is the eligible solution which maximizes agent utility in single-agent setting then 
	% $y_i(\omega) \geq y_i(\sigma_i)$. As a result, according to Assumption~\ref{as:pareto}, $x(\sigma_i) \geq x(\omega)$.
	% There are two cases

	% \begin{itemize}
	% 	\item
	% 	$\omega^*$ is sampled by $i$, i.e. $\omega^* = \sigma_i$. As shown above $x(\omega^*) = x(\sigma_i) \geq x(\omega)$.
	% 	\item
	% 	$\omega^*$ is sampled by another agent $j \neq i$.
	% 	As principal selects the best proposed solutions among all agents, $x(\omega^*) \geq x(\sigma_i)$.
	% 	Using the inequality $x(\sigma_i) \geq x(\omega)$ we further conclude that $x(\omega^*) \geq x(\omega)$.
	% \end{itemize}

	% This finishes the proof.

	% OLD PROOF
	% As in the proof of Theorem \ref{thm:recover}, we focus on proving (1) and we will argue that the proof naturally transfers to the other settings as well.
	% Consider a problem instance of the multi-agent setting.
	% Restrict our attention to agent $i$, and consider a problem instance of the single-agent setting such that the principal delegates to only agent $i$.
	% Then, by \citet{kleinberg2018delegated}, there exists an SPM under the constructed single-agent setting such that the principal's expected utility is at least $\frac{1}{2}\Ex{X_{i,(1)}}$.
	% Denote this mechanism by $M'_i$ and let its eligible set be $R_i$.
	% We can define such $R_i$ for each agent $i \in [n]$.
	% Given the observed solution $\omb_i$ of agent $i$, let the agent's strategy be $\sigma'_i \in \Omega^{k_i}$ under the single-agent setting with $M'$.
	
	% Now, under the multi-agent setting, consider an MSPM with eligible sets $R_i$ and a deterministic tie-breaking rule with transitivity.
	% Suppose that the solutions are realized to be $\omb = (\omb_1, \ldots, \omb_n)$ and consider any corresponding equilibrium strategies $\sigma = (\sigma_1,\ldots, \sigma_n)$.
	% We want to show that each agent $i$, given the observed solutions $\omb_i$, play a strategy $\sigma_i$ such that $x(\sigma_i) \ge x(\sigma'_i)$.
	% Suppose not, i.e. $x(\sigma_i)<x(\sigma'_i)$ for some $i \in [n]$.
	% If agent $i$ does not have eligible solutions, it contradicts the fact that $x(\sigma_i) < x(\sigma'_i)$.
	% Hence, agent $i$ has at least one eligible solution $\sigma'_i$.
	% Obviously, $\sigma \in R_i$ since if not the agent's utility in playing $\sigma_i$ is simply zero, and then proposing $\sigma'_i$ would yield a larger utility.
	% Then, by the definition of $\sigma'_i$, $y(\sigma'_i) \ge y(\sigma_i)$ and $x(\sigma'_i) > x(\sigma_i)$.
	% This contradicts Assumption~\ref{as:pareto} since $\sigma'_i$ dominates $\sigma_i$.
	% Therefore we conclude that $x(\sigma_i) \ge x(\sigma'_i)$.
	% Since the principal eventually selects the best candidate that maximizes her utility, we have
	% \begin{align*}
	% 	\Ex{\Ex{\max_{i \in [n]} x(\sigma_i) \given \omb_i}}
	% 	\ge
	% 	\Ex{\Ex{\max_{i \in [n]}x(\sigma'_i) \given \omb_i}}
	% 	\ge
	% 	\frac{1}{2}\Ex{X_{\max}}.
	% \end{align*}
	% Similarly, we can derive the same arguments for (2) and (3), and we finish the proof.
% \end{proof}

% In proving Theorem \ref{thm:recover_bayes}, we only analyze the principal's expected utility given a BNE, but we do not characterize the BNEs at all.
% This is in stark contrast to the complete information setting, since in Theorem~\ref{theorem:multi-agent-unlimited-budget}, we reveal that proposing the solution that maximizes the principal's utility is an equilibrium strategy except for the agent with the best solution, even under the MSPM without any eligible sets.

==> bck/cost_quantify.tex <==

\subsection{Informed mechanism}
\todo{single agent recovery is still possible? - not quite sure for now}

\todo{General lower bound? - when super agent, then regardless of $B$, examining super agent first then prophet lower bound.}


In case of symmetric agents, we observe that Theorem~\ref{thm:informed} still holds even with unit budget.
\begin{corollary}
	Consider symmetric agents endowed with distribution $D$ with support on $[0,1]$ such that its c.d.f. $F(x)$ satisfies $F(x) \le x^{\alpha}$ for any $x \in [0,1]$ for some $\alpha >0$. Then, there exists an oblivious mechanism with arbitrary examination budget such that under any BNE, the delegation gap is at most $1 - \parans{\frac{\alpha nk}{\alpha nk+1}}^{\frac{1}{\alpha nk}}$, which converges to $0$.
\end{corollary}
Noting that the proof of Theorem \ref{thm:informed} can be easily applied to examination cost setting with arbitrary budget, we omit the proof.

\subsection{Oblivious mechanism}
We present several explicit upper bound on the delegation gap for oblivious mechanism.
Our results will be based on the following corollary which is straightforward to obtain from Theorem \ref{theorem:multi-agent-limited-budget}.
\begin{corollary}
If the principal does not define an eligible set, then in the multi-agent setting with budget $2 \leq B \leq n - 1$, the RSPM has a delegation gap of at most
\begin{align*}
\Ex{X_{(1)}} - \Ex{X_{(n-B+2)}}.
\end{align*}
\end{corollary}

\todo{negative results on general setting}

We now consider symmetric agents.
First, in case of arbitrary distribution supported on $[0,1]$, we present the following theorem.
\begin{theorem}
	If agents are symmetric and the domain of their utility function lies in $[0,1]$, then there exists an oblivious mechanism in which the delegation gap is upper bounded by  \todo{Simplify... A figure on this w.r.t. $B$ for several $n$ may help?}.
\end{theorem}
\begin{proof}
	Suppose that we run the RSPM.
	By our assumption on symmetry and since each agent independently samples solutions, $X_{i,(1)}$ for $i \in [n]$ are identical and independent.
	Then, we use the following lemma introduced by \citet{lopez2011upper}.
	\begin{lemma}[\citet{lopez2011upper}]\label{lm:lopez_2}
		Let $X_1,\ldots, X_n$ be i.i.d. random variables supported on $[0,1]$. Given an integer $k$ such that $1 \le l < k \le n-1$, let $Y_k$ and $Y_l$ be $k$-th and $l$-th order statistics of $X_1,\ldots, X_n$. 
		Define
		\begin{align*}
			p_{k,l}= \parans{1 + \parans{\frac{\binom{n-1}{l-1}}{\binom{n-1}{k-1}}}^{\frac{1}{l-k}}}^{-1}.
		\end{align*}
		Then, the following holds.
		\begin{align*}
			\Ex{Y_{l} - Y_{k}} \le np_{k,l}^{k-1}(1-p_{k,l})^{n-l}\parans{\binom{n-1}{k-1}(1-p_{k,l})^{l-k} - \binom{n-1}{l-1}p^{l-k}}
		\end{align*}
	\end{lemma}
	Plugging $l = n$ and $k=B-1$ in the above lemma, we obtain
	\begin{align*}
		\Ex{X_{(1)} - X_{(n-B+2)}}
		\le 	
		\parans{1 + \parans{\frac{1}{\binom{n-1}{B-2}}}^{\frac{1}{n-B+1}}}^{-1},
	\end{align*}
	and it completes the proof.
\end{proof}

\begin{theorem}
	If agents are symmetric and $X_{i,j} \sim D$ such that $D$ has MHR, then there exists an oblivious mechanism in which the delegation gap is upper bounded by $\sqrt{2Var(D_{\max})}$ where $D_{\max}$ is distribution of $X_{i,(1)}$.
	In case of $D = U[0,1]$, we have delegation gap of at most $(n-B+1)\sqrt{2 \cdot \frac{k}{(k+1)^2(k+2)}} \approx \frac{\sqrt{2}(n-B+1)}{k}$.
\end{theorem}
\begin{proof}
	\todo{Elaborate more on}
	Note that
	\begin{align}
		\Ex{X_{(1)} - X_{(n-B+2)}}
		&=
		\Ex{X_{(1)} - X_{(2)}} + \Ex{X_{(2)} - X_{(3)}} + \ldots + \Ex{X_{(n-B+1)} - X_{(n-B+2)}}.\label{ineq:010151137}
	\end{align}
	We now prove that for any $k = 2,\ldots, n-1$,
	\begin{align*}
		\Ex{X_{(k)} - X_{(k+1)}}
		\le 
		\Ex{|A-B|},
	\end{align*}
	where $A$ and $B$ are two i.i.d. random variables of which the endowed distribution is equivalent to that of $X_{i,(1)}$.
	This is indeed true because
	\begin{align*}
		\Ex{X_{n-k+1:n} - X_{n-k:n}}
		&\le
		\Ex{X_{2:n-k+1} - X_{1:n-k+1}}
		\\
		&\le
		\Ex{X_{2:2} - X_{1:2}}
		\\
		&=
		\Ex{|A-B|},
	\end{align*}
	where the first inequality follows from the first part of Lemma~\ref{lm:order_stat_diff}, and the second one follows from the second part.
	Hence, applying Theorem~\ref{thm:mhr_upperbound} in \eqref{ineq:010151137}, we finish the proof.
\end{proof}




\begin{theorem}
	If agents are symmetric and $X_{i,j} \sim D$ such that $D$ has monotone increasing p.d.f. then there exists an oblivious mechanism in which the delegation gap is upper bounded by $\frac{n-B+1}{n+1}\sqrt{2Var(D_{\max})}  +$ where $D_{\max}$ is distribution of $X_{i,(1)}$.
	In case of $D = U[0,1]$, we have delegation gap of at most $\frac{n-B+1}{n+1}\sqrt{2 \cdot \frac{k}{(k+1)^2(k+2)}} \approx \frac{3\sqrt{2}(n-B+1)}{k(n+1)}$.
\end{theorem}
\begin{proof}
	\todo{Similar to the proof above}
\end{proof}




% \subsection{Toward better mechanism}
% Now we study whether there exists a mechanism that outperforms the randomized single-proposal mechanism in the multi-agent case.

% \paragraph{Warm-up: randomized $k$-proposal mechanism}
% We start with a $k$-proposal mechanism, in which the agents can submit up to $k$ candidates, with a simple selection rule: randomly sort the candidates, examine the first $B$ candidates, and then commit to the best candidate.
% This mechanism obviously has an examination cost of $B$.

% Intuitively, this mechanism works very poor as observed by the following conjecture.
% \begin{conjecture}

%In randomized $k$-proposal mechanism with unit budget, the delegation gap can monotonely increase with respect to $k$, and thus is lower bounded by the delegation gap of single-proposal mechanism.

% \keivan{In this case, agent $i$ will propose top $k$ eligible points w.r.t to her own utility $y_i$. Therefore, change in delegation gap depends on whether those top $k$ points give better utility to the principal or not.}

% \suho{Provide a counterexample that this works poorly}
% In a unit-budget randomized $k$-proposal mechanism with arbitrary eligible sets, the delegation gap is monotone increasing with respect to $k$, and thus is lower bounded by the delegation gap of RSPM with the same eligible sets.
% \end{conjecture}
%\begin{proof}[Intuition]
%	The intuition behind this conjecture is that given fixed budget $B$, when $k$ increases then the chance that set of $B$ chosen solutions by principal covers some solutions of a same agent increases. It implies that the agent may rely on the fact that in some cases competition is only over his proposed solutions which motivates him to propose solutions to maximize his own utility instead of principal utility.
%\end{proof}

% \begin{conjecture}
% In a $B$-budget randomized $k$-proposal mechanism with arbitrary eligible sets, the delegation gap can monotony increase with respect to $k$, and thus is lower bounded by the delegation gap of RSPM with the same eligible sets.
% \end{conjecture}

% \keivan{The intuition behind this conjecture is that given fixed budget $B$, when $k$ increases then the chance that set of $B$ chosen solutions by principal covers some solutions of a same agent increases. It implies that the agent may rely on the fact that in some cases competition is only over his proposed solutions which motivates him to propose solutions to maximize his own utility instead of principal utility.}
%\paragraph{Improved mechanism}
%We have some options that we do not fully exploit in our randomized single-proposal mechanism.
%Firstly, we did not customize eligible set for each agent. Secondly, we did not optimize the examination order over the agents.




% \section{Further directions}


% \begin{question}[Improved mechanism - customizing eligible set]
% In our RSPM, the examination set is randomly permuted and then we examine up to $B$ candidates, and we mainly consider a homogeneous eligible set.
% How much can we improve by considering heterogeneous eligible sets for the agents?
% Consider an extreme scenario in which each agent $i$ has a distribution with support on $\{1, 2^i\}$ with probability $1/2$ for both the elements, in terms of the principal's utility, and suppose that both elements have a random utility of $1$ or $2$ for the agent independently from the principal's utility.
% In this case, if we set agent-wise threshold $\tau_i = 2^i$, this seems to work superior to any homogeneous eligible set, though needs to be checked thoroughly.
% As this kind of exploiting agent-wise thresholds seems to be somewhat similar to multiple threshold algorithms in prophet inequality literature, it would be interesting if we can find some relations between general RSPM and multiple thresholds algorithms in the prophet inequalities literature.
% Furthermore, as the principal is allowed to select up to some given multiple candidates, it would be also interesting if we may find some relations between some mechanisms and the multi-unit prophet inequality, though it is not clear at this point.
% \end{question}

% \begin{question}[Improved mechanism - examination order]
% Obviously, the randomized examination is somewhat silly, since if we know that some agents have superior distribution, the principal might be better to examine them first.
% This problem reduces to designing an optimal order of examination for our mechanisms.
% Consider the example we considered in Question 4. 
% In this case, we can further optimize the examination order by examining the agents with large indexes first, as they are always expected to have larger values when the thresholds are set properly.
% Suppose that there exists no eligible set and $k_i = 1$. 
% Under the RSPM each agent essentially proposes only one solution.
% In which order should we examine the candidates in this case?
% More generally, the question of deciding examination order may (or may not) be similar to the problem of deciding optimal ordering in prophet inequalities~\cite{agrawal2020optimal}.
% It would be interesting to explore whether some relations indeed exist, though not seem to be straightforward.
% \end{question}



% \begin{question}[Further possible extensions]
% Further extensions that might be interesting to explore.
% It seems we should definitely think about the incomplete information setting for sake of completeness, but the others might be beyond the scope of this research.
% \begin{enumerate}
%     \item Incomplete information setting
%     \item Multiple distributions for each agent (similarly from~\citet{kleinberg2018delegated}
%     \item binary model with sampling cost model, which corresponds to delegated search on Weitzman's box problem as in~\citet{kleinberg2018delegated}
%     \item Online proposal and examination setting (when agents sequentially propose and the principal should irrevocably decide)
%     \item Learning agents (when each agent does not know the quality of own solutions but rather learns over multiple interaction between the mechanism)
% \end{enumerate}
% \end{question}


% \begin{conjecture}
% For any budget $B$, there exists a mechanism in which the delegation gap is always smaller than randomized single-proposal mechanism.
% Some ideas: use personalized eligible set, use a smarter selection rule
% \end{conjecture}

==> bck/cost_recover.tex <==

\todo{Mention that if $B \ge n$, all the results from the no cost section holds as we consider MSPM with some eligible sets.}
\begin{corollary}
In the multi-agent setting, for any mechanism $M$ with budget $B \ge n$ and corresponding Nash equilibrium $\sigma$, there exists a RSPM $M'$ with budget $n$ such that for any Nash equilibrium strategies $\sigma'$, for any $\om \in F_{M,\sigma}(\omb)$ and any $\om' \in F_{M',\sigma'}(\omb)$, we have $x(\om) \le x(\om')$ for any observed solutions $\omb \in \Omega^*$.\todo{prove for self-containedness}
\end{corollary}

==> bck/randomized_not_working.tex <==
\section{Randomized tie-breaking rule does not work}\label{app_sec:random_tie}
\suho{I think this section will be removed}
We recall that Theorem~\ref{theorem:multi-agent-unlimited-budget} only holds for the \emph{deterministic} tie-breaking rule.
The intuition behind it is that if the principal exploits a randomized tie-breaking rule, it may reduce the power of competition in certain cases since the agents may settle with a bad solution in terms of the principal, as it still gives the agents higher utility with small probability due to the randomized tie-breaking rule, yet another solution which might induce higher probability to be selected by the principal may yield too low utility for the agents. 
However for the deterministic tie-breaking rule, as the principal naturally prefers some agents, less preferred agents tend to submit the candidate more in a competitive manner in order to be selected by the principal, and again, this recursively makes preferred agents behave more in favor of the principal.
More formally, in the following theorem, we prove that the random tie-breaking rule can be arbitrarily bad, which implies that the deterministic tie-breaking rule is essential.
\begin{theorem}
    Consider a MSPM with no eligible sets and a randomized tie-breaking rule that uniform-randomly selects the candidate.
    Then, for any $\alpha \ge 1$, there exists a problem instance such that the mechanism have a bad equilibrium in which the delegation gap can be larger than $\alpha \cdot \Ex{X_{(1)} - X_{(2)}}$.
\end{theorem}
\begin{proof}
    \todo{Fix this w.r.t. i.i.d. sampling}
	Given a solution space $\Omega = \{a,b,c\}$, consider $n=3$ agents with the same utility function $y$ such that $y(a) > 3y(b)$ and $y(b) > y(c)$.
	The principal's utility function is given by $x(\cdot)$ such that $x(a) < x(b) < x(c)$.
	Note that the detailed quantities will be determined later.
	Agent $1$ and $2$ always sample both $a$ and $b$, and agent $3$ also always samples both $a$ and $c$. 
	In this case, although $X_{(1)} - X_{(2)} = x(c) - x(b)$, if all the agents $1$, $2$ and $3$ determine to submit $a$, they can get $y(a)\cdot 1/3 > \max(y(b),y(c))$, and thus this forms an equilibrium.
	In this equilibrium, the delegation gap is $(x(c) - x(a))$, and hence by constructing the function $x(\cdot)$ to satisfy $x(c) - x(a) \ge \alpha (x(c) - x(b))$, we can conclude the proof.
	Note that this is always po ssible since we can take arbitrarily small $x(a) \le \alpha x(b) - (\alpha-1)x(c)$ as RHS is a positive number.
\end{proof}

==> no_cost.tex <==
% !TEX root =  main.tex
\section{Analysis of the multi-agent single-proposal mechanism}\label{section:no_cost}
In this section, we provide a performance guarantee of MSPM.
Note that for the multi-agent delegation problem, it suffices to find a good mechanism over the space of MSPMs, thanks to Theorem~\ref{thm:multiagent_revel}.
We first present the analysis of delegation gap of MSPM, and then present a comparison between the performance of MSPM in the multi-agent setting and the performance of any mechanism in the single-agent setting.

\subsection{Delegation Gap}
We first prove a generic result regarding an arbitrary threshold-based eligible set and further quantify the corresponding delegation gap for some good choices of the parameters of MSPM.

%We mainly argue that a large examination budget gives us a significant amount of gain in terms of principal's utility.

% To elaborate, we first present how the single-proposal mechanism behaves under the single-agent setting in terms of $X_{i,j}$ and $Y_{i,j}$, which will be useful in comparing the results.
% Generally, the threshold $\tau$ is set to be half of the expectation of $X_{\max} =  \max_{j \in [k]} X_{1,j}$ so that $\tau = 1/2\Ex{X_{\max}}$.
% Then, by the dynamics of the single-proposal mechanism, solution with highest $Y_j$ satisfying $X_{j} \ge \tau$ will be selected.
% Define $\set{E} = \{\om \in \omb : x(\om) \ge \tau \}$, i.e. the subset of solutions contained in the eligible set.

% We use $\mec_{SP}$ to denote the expected utility of single-proposal mechanism.
% More, formally,
% \begin{align*}
% \mec_{SP}  = \Ex{TBD}
% \end{align*}

\begin{theorem} \label{theorem:multi-agent-unlimited-budget}
Given any $\tau \ge 0$, let $R$ be an eligible set with threshold $\tau$ such that $R:= \{\omega: x(\omega) \ge \tau, \omega \in \Omega\}$, and $\rho$ be an arbitrary deterministic tie-breaking rule with transitivity.
In the multi-agent setting, MSPM with $\rho$ and a homogeneous eligible set $R$ has a delegation gap of at most
\begin{align*}
\Ex{X_{(1)}} - \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} - 
\Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.
\end{align*}
\end{theorem}
\begin{proof}[Proof]
We mainly prove that the payoff of randomized single-proposal mechanism $M$ is at least $$\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.$$
% We denote by $c_i$ the agent $i$'s proposed candidate. Since there is an unlimited budget for examination, we can assume that the principal examines all candidates and takes the best candidate which maximizes her utility, i.e. winner is $c_{i^*}$ where $i^* = \argmax_{i} x(c_i)$.

We find a lower bound on the principal's utility in an arbitrary Nash equilibrium. 
%We consider two cases based on whether there exist eligible solutions or not.
Let $\omb = \cup_{i \in [n]}\omb_i$ be the entire set of solutions observed by the agents and $\sigma = (\sigma_1,\ldots, \sigma_n)$ be the equilibrium strategies.
We separately consider two cases (i) for any $\om \in \omb$, $\om \notin R$ and (ii) there exists $\om \in \omb$ such that $\om \in R$.

{\em Case (i).} 
In this case, the utility of all agents is $0$,
and there does not exist a winner. 
Recall that for any Nash equilibrium,
there exists no incentive for any agent to deviate from equilibrium strategies.
%We denote the agent with rank $1$ by $t$. 
%<<<<<<< Updated upstream
%We show that in this case $X_{(1)} < \tau$.
%Suppose not, i.e. $X_{(1)} \geq \tau$. 
%Denote by $\om^*$ the candidate which corresponds to the utility of $X_{(1)}$.
%If agent $t$ proposes $\om^*$, his utility strictly increases from $0$ to $y(\om^*)$, which contradicts that the agents have played equilbirium strategies.
%=======
We claim that $X_{(1)} < \tau$, where it concludes that the principal's utility is simply zero in this case.
Suppose not, i.e. $X_{(1)} \geq \tau$. 
Denote by $\om^*$ the candidate which corresponds to the utility of $X_{(1)}$.
If agent $t$ plays $\om^*$, his utility strictly increases from $0$ to $y(\om^*)$, which contradicts that the agents have played equilibrium strategies.
%>>>>>>> Stashed changes
Hence we conclude that $X_{(1)} < \tau$, and the principal's utility is $0$.

{\em Case (ii).} 
Suppose that the winner is the candidate proposed by agent $i^*$. 
In this case, all agents except agent $i^*$ have a utility of $0$. 
Like the previous case, there is no incentive for agents to change their strategies. 
%<<<<<<< Updated upstream
%Consider agent $i \neq i^*$,
%there is no incentive for the agent to propose his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$. 
%This implies that even if agent $i$ proposes that solution, he still gets a utility of $0$. 
%\suho{I understand these sentences, but it would be more formal if we can mathematically represent them, not by english. For example in the above sentence, we can say that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y(\sigma_i) = 0$. I think the reason that Mohammad commented on our previous version to be less formal is that it argues too much with words.}
%As a result, if he proposes his best-observed solution, that solution is not selected as the winner, which shows that the current winner gives a higher utility to the principal, i.e. $x(c^*) \geq X_{i, (1)}$. 
%\suho{same as above}
%=======
Consider agent $i \neq i^*$, there is no incentive for the agent to propose his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$. 
This implies that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y_i(\sigma_i) = 0$.
%\suho{I understand these sentences, but it would be more formal if we can mathematically represent them, not by english. For example in the above sentence, we can say that for any $\sigma_i = \om$ for some $\om \in \omb_i$, $y(\sigma_i) = 0$. I think the reason that Mohammad commented on our previous version to be less formal is that it argues too much with words.}
Since the agents are playing equilibrium strategies $\sigma$, the winner should not be changed with respect to agent $i$'s strategy.
This implies that $x(\sigma_{i^*}) \geq X_{i, (1)}$ for any $i \neq i^*$.
%
%As a result, if he proposes his best-observed solution, that solution is not selected as the winner, which shows that the current winner gives a higher utility to the principal, i.e. $x(c^*) \geq X_{i, (1)}$. 
%\suho{same as above}
%>>>>>>> Stashed changes
Furthermore, we have $x(\sigma_{i^*}) \leq X_{i^*, (1)}$. Since for $n-1$ agents $i$ ($i \neq i^*$) we have $X_{i, (1)} \leq x(\sigma_{i^*})$, and $x(\sigma_{i^*}) \leq X_{i^*, (1)}$ using the definition of $X_{(r)}$ we get
$$
X_{(n)} \leq X_{(n-1)} \leq ... \leq X_{(2)} \leq x(\sigma_{i^*}) \leq X_{(1)}.
$$
Also, in this case, we assume that $\sigma_{i^*}$ is eligible which further implies that $\tau \leq x(\sigma_{i^*}) \leq X_{(1)}$. So we get $\max\left(X_{(2)}, \tau\right) \leq x(\sigma_{i^*}) \leq X_{(1)}$. This inequality shows that
\begin{itemize}
    \item if $X_{(2)} \geq \tau$ then $x(\sigma_{i^*}) \geq X_{(2)}$.
    \item if $X_{(1)} \geq \tau \geq X_{(2)}$ then $x(\sigma_{i^*}) \geq \tau$.
\end{itemize}

Therefore, by combining the results of the case (i), and case (ii) the expected utility of the principal is at least
\begin{align}
	\Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
	\Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}.\label{ineq:infbud_tau}
\end{align}


% The proof mainly follows from the following lemma.


% \begin{lemma}
% In multi-agent setting with unlimited budget, the payoff of randomized single-proposal mechanism $M$ is at least $\Ex{X_{(2)}\IND[X_{(2)} \ge \tau]} + \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}$.
% \begin{proof}[Proof Sketch of Lemma]
% Since there is an unlimited budget for examination, we can assume that the principal takes the best candidate with respect to her own utility.
% There are two cases here:
% \begin{itemize}
%     \item If the best candidate does not satisfy the principal requirements, i.e. none of the proposed candidates are in eligible set $T_\tau$, i.e. $X_{\max} < \tau$; then the principal utility will be $0$.
%     \item If there is at least one candidate which satisfies the principal requirements; then we have $f_{M, \sigma}(\omb) = \argmax_i x(\sigma_i(\om_i))$. If $i^*$ is the agent who owns the winner, then all other agents have a utility of $0$. Consider a Nash equilibrium case where the utility of agents does not increase if they change their candidates (i.e. $\sigma_i(\om_i)$). Since the utility of all agents except agent $i^*$ is $0$, it implies that other agents do not have any strategies to get a positive utility. Since we are considering a Nash equilibrium, if agent $i \left(i \neq i^*\right)$ proposes his best-observed solution, i.e. the solution which gives the principal utility of $X_{i, (1)}$, then he still gets utility of $0$, which implies that the winner selected by the principal has utility at least $\max_{i \neq i^*} X_{i, (1)}$.
% Therefore, we can conclude that $i^*$ is the agent whose rank is $1$, thus what he proposes should give the principal higher utility than the best proposal of other agents:
% $$
% x(\sigma_{i^*}(\om_{i^*})) \geq X_{(2)} \geq X_{(3)} \geq ... \geq X_{(n)}.
% $$
% Also, if $X_{(2)} < \tau$ then we can have a better bound on the winner since $\sigma_{i^*}(\om_{i^*})$ is eligible then $x(\sigma_{i^*}(\om_{i^*}) \geq \tau$ thus in this case we have:
% $$
% x(\sigma_{i^*}(\om_{i^*})) \geq \tau > X_{(2)} \geq X_{(3)} \geq ... \geq X_{(n)}.
% $$
% \end{itemize}

% Therefore, we can conclude that the utility is bounded by 
% $$
% \Ex{X_{(2)}\IND\left[X_{(2)} \geq \tau\right]} + 
% \Ex{\tau\IND\left[X_{(1)} \geq \tau > X_{(2)}\right]}
% $$
% \end{proof}
% \end{lemma}
\end{proof}
The main intuition behind this advantage is that the existence of opponents, whose proposed solutions are examined by the principal, makes agents more competitive in sending signals, thus resulting in submitting more qualified solutions to be selected.


A direct corollary of this result is that we can derive the following upper bound on the delegation gap even without the eligible set.
\begin{corollary}\label{cor:infbud_notau}
MSPM with no eligible set and a deterministic tie-breaking rule with transitivity has a delegation gap of at most
\begin{align}
	\Ex{X_{(1)}} - \Ex{X_{(2)}}\label{ineq:infbud_notau}
\end{align}
\end{corollary}
This implies that even without the eligible set, the multi-agent setting brings some advantages for the principal, which is mainly due to the competitive tension arising between the agents.


We highlight that the theorem only holds for the \emph{deterministic} tie-breaking rule.
The intuition behind it is that if the principal exploits a randomized tie-breaking rule, it may reduce the power of competition in certain cases since the agents may settle with a bad solution in terms of the principal, as it still gives the agents some utility due to the randomized tie-breaking rule and another solution which is more preferred to the principal might yield a low utility for the agents.
However for the deterministic tie-breaking rule, as the principal naturally prefers some agents, the other agents tend to be more competitive in order to be selected by the principal, and this recursively makes those preferred agents to behave more in favor of the principal.
More formally, in the following theorem, we prove that random tie-breaking rule can be arbitrarily bad for some problem instances.
\begin{theorem}
    Consider a MSPM with eligible sets $(R_i)_{i \in [n]}$ and a random tie-breaking rule.
    Then, for any $\eps > 0$, there exists a problem instance such that the mechanism have a bad equilibria in which the delegation gap is at least $1/\eps$.
\end{theorem}
\begin{proof}
\todo{prove it.}
\end{proof}


\todo{Recovering single-agent guarantees.}
% \begin{example}
% Given a solution space $\Omega = \{a,b,c\}$, consider $n=4$ agents with the same utility function $y(a) = 100$, $y(b) = 10$ and $y(c) = 1$ and a principal with utility function $x(a) = 1$, $x(b) = 10$ and $x(c) = 100$.
% Each agent samples two solutions.
% Agents $1,2$ sample $a$ or $c$ with equal probability, and agents $4,5$ sample $b$ or $c$ with equal probability.
% Consider a RSPM with a random tie-breaking rule, eligible sets $R_i$ for $i \in [n]$ and unlimited budget.
% Suppose that the agents' solutions are realized to be $\{a,c\}$,$\{a,c\}$,$\{b,c\}$ and $\{b,c\}$.
% \end{example}




%\note{I couldn't find a good description for Theorem 3.3}
\subsection{Comparing multi-agent and single-agent delegation}
% Furthermore, we find a lower-bound on the expected utility of the principal using RSPM. In Theorem \ref{theorem:multi-agent-unlimited-budget}, we formulate the principal's utiltiy when there is an unlimited examination budget, i.e. principal can examine all candidates. Then in Theorem \ref{theorem:multi-agent-limited-budget}, we consider the case that examination budget is limited, and we find a lower-bound on principal's utilty regarding the examination budget.

%We further ask whether there exists any improvement in the delegation gap in the multi-agent setting compared to single-agent setting despite using of the same mechanism.
%We will elaborate more later on how we compare the multi-agent and the single-agent setting.
%Surprisingly, we find that the delegation gap in multi-agent setting can significantly decrease compared to that of single-agent setting.
%This is mainly due to the competition between agents, which was not there in single-agent setting in which any mechanism with an arbitrary budget can be simply reduced to single-proposal mechanism with unit examination budget.

In this section, we show that the multi-agent delegation indeed brings advantages over the single-agent delegation. we compare the principal's utility when delegating to multiple agents with a situation where a single agent is in charge of finding the solutions. 
We observe that delegating to multiple agents indeed has advantages in terms of the principal's utility.
To this end, we first define a reasonable way to compare the principal's utility in the multi-agent setting with that in the single-agent setting.
%Given a single-agent problem, we present two benchmarks in multi-agent problem as follows.
\begin{definition}[Multi-agent correspondence]
Consider a single-agent problem with a distribution $D$, a number of solutions $k$, the agent's utility function $y$, and the principal's utility function $x$.
Consider a multi-agent problem with $n \ge 2$ agents in which the principal has the same utility function $x$ and each agent $i$ has a distribution $D_i = D$, a number of solutions $k_i$ such that $\sum_{i=1}^nk_i = k$, and the utility function $y_i = y$. We denote this multi-agent problem a \emph{weak} $n$-agent correspondence of the single-agent problem.
%\begin{enumerate}
%	\item there exists an agent $i$ with parameters $k_i = k$, $D_i =D$, and $y_i = y$. We denote this multi-agent problem a \emph{strong} $n$-agent correspondence of the single-agent problem.
%	\item each agent $i$ has a distribution $D_i = D$, a number of solutions $k_i$ such that $\sum_{i=1}^nk_i = k$, and the utility function $y_i = y$. We denote this multi-agent problem a \emph{weak} $n$-agent correspondence of the single-agent problem.
%\end{enumerate}
\end{definition}
%The strong $n$-agent correspondence refers to a strong version of benchmark in which the agent in the single-agent problem becomes one of the agents in the multi-agent problem.
%Intuitively, we expect this strong benchmark to be have better outcome in terms of the principal's utility, since the principal delegates to a strictly better pool of agents.
To see whether delegating to the multi-agent indeed brings advantages, it is fair to compare under the assumption that the agents exert the same total amount of effort in the task in both the single-agent and the multi-agent problem.
Since the number of solutions can be translated as the amount of effort exerted in the task, our definition of the multi-agent correspondence would play a reasonable role in comparing the single-agent and the multi-agent problem.

\begin{theorem}\label{theorem:multi-agent-correspondence}
Given a single-agent problem $P$, denote its multi-agent correspondence $P'$.
For any mechanism $M$ under $P$, there exists a MSPM under $P'$ such that the principal's utility of the MSPM under $P'$ is at least that of  $M$ under $P$.
\end{theorem}
%However in some sense, to see whether delegating to multi-agent indeed brings advantages, it is fair to compare under the assumption that the agents exert the same total amount of effort in the task in both the single-agent and multi-agent problem.
%We first present a result on the strong benchmark.
%\begin{theorem}
%Given a single-agent problem $P$, denote its strong $n$-agent correspondence $P'$.
%For any SPM with an eligible set in $P$, there exists a unit-budget RSPM with a homogeneous eligible set in $P'$ such that the principal's expected utility of the RSPM under any Nash equilibrium in $P'$ is at least that of the $SPM$ in $P$.	
%\end{theorem}
%\begin{theorem}
%Given a single-agent problem $P$, denote its weak $n$-agent correspondence $P'$.
%For any SPM with an eligible set in $P$, there exists a RSPM with a homogeneous eligible set and budget $B=n$ in $P'$ such that the principal's expected utility of the RSPM under any Nash equilibrium in $P'$ is at least that of the $SPM$ in $P$.
%\end{theorem}
\begin{proof}
We start by presenting the following lemma from~\cite{kleinberg2018delegated}.
\begin{lemma}[\cite{kleinberg2018delegated}]\label{thm:singleagent_revel}
In the single-agent setting, for any mechanism $M$ and corresponding dominant strategies $\sigma$, there exists a MSPM such that for any equilibrium strategies $\sigma'$, we have $x(f_{M,\sigma}(\omb)) = x(f_{SPM,\sigma'}(\omb))$ for any $\omb \in \Omega^*$.
\end{lemma}
% This corresponds to a celebrated revelation principal~(cite) in mechanism design literature.
% It is important to note that any SPM requires an examination budget of $1$, since it only evaluates a single candidate from a single agent.
% This implies that there is no merit in having a large examination budget against single-agent.
% This is fairly intuitive because, in a single-agent setting, the agent does not have any incentive to signal more than two candidates since he knows that only one of them would be eventually selected.
By the lemma, it suffices to consider the case when $M$ is a SPM.
Let the realized solutions in $P$ be $\omb = \{\om_1, \om_2,\ldots, \ldots \om_k\}$. Consider a partition of $\omb$ as follows
\begin{align*}
	\omb_{1} &= \{\om_1,\ldots, \om_{k_1}\}
	\\
	\omb_{2} &= \{\om_{k_1+1},\ldots, \om_{k_1+k_2}\}
	\\
	&\vdots
	\\
	\omb_{n} &= \{\om_{k_1+\ldots+k_{n-1}+1},\ldots, \om_{k_1+\ldots + k_n=k}\}.
\end{align*}
Suppose that agent $i$'s realization of solutions in $P'$ is $\omb_{i}$ so that the outcomes of $P$ and $P'$ are coupled. 
This coupling is indeed possible because the probability that agent $i$'s solutions are realized to be $\omb_i = \{\om_{i_1},\ldots, \om_{i_{k_i}}\}$ is exactly equal to the marginal probability that $\om$'s $i$-th partition is realized to be $\omb_i = \{\om_{i_1},\ldots, \om_{i_{k_i}}\}$.
Consider a SPM with an eligible set $R$ under $P$, and corresponding equilibrium strategies $\sigma$.
Denote by $x$ and $y$ the principal and the agent's utility function under $P$ respectively.
Given the solutions realized as above, SPM will select the solution which maximizes $y(\om_j)$ for $j \in [k]$ such that $\om_j \in R$, i.e. $\om_1^* = \argmax_{j \in [n], \om_j \in R} y(\om_j)$.
Let this solution be $\om_1^*$.
Now consider a MSPM with arbitrary tie-breaking rule and the same eligible set $R$ under $P'$, and suppose that the agents play equilibrium strategies $\sigma'$.
Let $\om_2^*$ be the corresponding winner in this case.
% Let $A$ be a set of solutions that can be selected as a winner in the MSPM under $P'$.
% Note that $A$ might include multiple solutions since the examination process is randomized in RSPM.
% For any $\om_2^* \in A$, 
We want to show that $x(\om_2^*) \ge x(\om_1^*)$  for any realization of solutions $\omb$.
Suppose not.
It is obvious that both $x(\om_1^*)$ and $x(\om_2^*)$ belong to the eligible set $R$.
If $\om_1^*$ and $\om_2^*$ belongs to the same partition $\omb_i$, it means that agent $i$ has both the solutions $\om_1^*$ and $\om_2^*$.
By our definition on $\om_1^*$ such that $\om_1^* = \argmax_{j \in [n], \om_j \in R} y(\om_j)$, submitting $\om_1^*$ is gives the better or the same utility for agent $i$.
If $y(\om_1^*) > y(\om_2^*)$, then simply submitting $\om_1^*$ gives a strictly better utility for agent $i$, and it contradicts that $\sigma'$ is equilibrium strategy.
If $y(\om_1^*) = y(\om_2^*)$, then $x(\om_1^*) \le x(\om_2^*)$ by Assumption~\ref{as:pareto}.
Hence, $x(\om_1^*) \le x(\om_2^*)$ in both cases.
Now suppose that $\om_1^*$ and $\om_2^*$ belongs to the different partitions $\omb_i$ and $\omb_j$.
Suppose that agent $i$'s equilibrium strategy satisfies $\sigma'_i \neq \om_1^*$.
If playing $\omb_i$ is strictly better for agent $i$, it contradicts that $\sigma'_i$ is an equilibrium strategy.
Hence $y(\om_1^*) = y(\sigma_i')$. Again by Assumption~\ref{as:pareto}, since agent $i$ plays $\sigma_i'$, we have $x(\sigma'_i) \ge x(\om_1^*)$.
Note that the principal should observe both $\sigma_i'$ and $\om_2^*$, and commits to $\om_2^*$.
This implies that $x(\om_2^*) \ge x(\sigma') \ge x(\om_1^*)$, and we finish the proof.
\end{proof}

A main implication of the theorem is that the principal can actually increase her utility by recruiting more agents with similar utilities to delegate the task and examining only a single solution from each agent.
Although this does not quantify whether the multi-agent delegation largely improves upon the single-agent setting, delegating to multi-agent still has benefits in the sense that it would take much smaller time (or resource) in terms of the agents if we ask $10$ agents to find $10$ solutions and propose at most one solution each, rather than the scenario that we ask a single agent to find $100$ solutions and propose at most $10$ solutions.



% \begin{question}[Quantifying the delegation gap]\label{quest:2}
% Quantify some reasonable upper bounds on \eqref{ineq:infbud_tau} and ~\eqref{ineq:infbud_notau} with respect to distribution $D_i$ and $k_i$ for $i \in [n]$ will be interesting.
% Following the proof technique of prophet inequalities, it seems to be doable to initially prove that we have $2$-approximation.
% Upton this, if we can derive a big improvement over $2$ or $e/(e-1)$ for some regimes, then it will be interesting.
% We may firstly consider a simplistic setting of two agents and $D_i = D$, maybe uniform distribution, and $k_i = k$, and further extend it.
% For example, if $k_i=1$ and $x(D_i) = U[a,b]$ for some positive $a,b > 0$, then it seems to be straightforward to check that the delegation gap is upper bounded by $\mO(1/n)$, using some order statistics (although we do not precisely define $x(D_i)$, we use it to denote the distribution of $x(\om)$).

% Negative results for some characterizations on $k_i,D_i$ might be also interesting. We can say something like if the distributions are something like this, then multi-agent delegation does not improve much, so just better off settling with a single agent.

% Finally, we may try to derive a lower bound on the delegation gap for any mechanism.
% \end{question}

==> note.tex <==

\section{Note}


\subsection{Heterogeneous cost}

\begin{question}[Heterogeneous examination cost]
We suppose that the examination cost of a single solution is fixed at $1$.
Instead, consider a scenario in which each solution has a heterogeneous cost $c(\om)$
If this solution $\omega$ is proposed as a candidate and examined by the principal, it incurs an examination cost of $c(\om)$.
The principal's objective can be (1) maximizing utility given an examination budget $B$ or (2) maximizing utility minus total examination cost.
For (1), the problem formulation seems somewhat to be relevant to the stochastic knapsack (though not exactly the same) but the difference is that the problem parameters are the proposed candidates, and thus strategically determined.
For (2), it seems to be very relevant to Weitzman's box problem, but the difference is that again, the parameters are strategically decided.
However, in order to derive some interesting results, I think it would be reasonable to compare with another benchmark, rather than the strong benchmark of the delegation gap.
This is because, if we still compare with the case in which the principal can just select the optimal solution among the entire solutions, then what we can only say is whether we can recover the results on the no-cost scenario.
Maybe we can consider a benchmark who has more budgets and can access all the solutions, but does not also know the realization of the solutions, and so is sampling probabilistically.
We may further consider a scenario in which the cost is randomly determined, not publicly available to the principal in advance, but only the distribution is informed.
\end{question}


\paragraph{Plan}
\begin{enumerate}
\item Think about better mechanism
\end{enumerate}



\begin{question}
How does this problem setup differs from procurement auction precisely?
Refer: (..)
\end{question}
Common: (i) adverse selection (information asymmetry), (ii) The player with less information designs a mechanism, (iii) the player with more information sends a signal.

Difference: (i) No monetary transfer

\begin{question}
How does this problem setup differs from crowdsourcing contest precisely?
Refer: (Optimal crowdsourcing contests, GEB 19)
\end{question}
Difference: (i) no monetary transfer, (ii) exogenous samples of agents, i.e. they do not strategize over effort (this does not hold for costly sampling box model)

\suho{In order to position this paper properly, take a careful look at (i) Optimal crowdsourcing contests SODA 12 / GEB 19, literature on procurement auction, and literature on signaling game, and legislative game}

\section{Further Possible Extensions}

\paragraph{Complete information setting}
\begin{enumerate}
    \item Multiple distribution for each agent
    \item Binary model with sampling cost (which corresponds to Weitzman's box problem)
\end{enumerate}


\paragraph{Online extension}


\paragraph{Multi-choice extension}


\begin{question}
does revelation principal (lemma 1~\cite{kleinberg2018delegated}) still holds for multi agent case?
My intuition is that this depends on the information assumption.
In complete information case, I think we can reduce any mechanism to single proposal deterministic mechanism.
\end{question}

Then we can ask what is the characterization of the optimal delegation mechanism.
\begin{question}
What is the optimal delegation mechanism?	
\end{question}


Next, we are interested in the characterization of the scenario in which the competition helps
\begin{question}
In which cases the competition helps compared to the case when the task is only delegated to a single agent.
When compared to single best agent (in terms of the principal), then it corresponds to sth like price of stability, and if compared to single worst agent, then it corresponds to sth like the price of anarchy.
\end{question}

\begin{question}
Delegation gap 
If competition helps or harms, how much the delegation gap increases or decreases?	
\end{question}



\begin{question}
In which situation (characterization of realized samples), competition helps/harms? How much it helps/ harms?
\end{question}
i.e. when does the utility of the principal increase / decrease compared to the scenario when a single agent picks all the $n$ samples by herself?
In here, the single agent might be the best agent (in terms of the principal, thus something like price of stability) or the worst agent (in terms of the principal, thus something like price of anarchy).
If it improves the principal's utility, how much the delegation gap improved compared to $1/2$ of \cite{kleinberg2018delegated}?


\subsection{Incomplete Information}

\paragraph{Improved mechanism}\note{Temporary section...just a bunch of ideas below}
\begin{definition}[Score-based single-proposal mechanism]
    In a score-based single-proposal mechanism (S-SPM), eligible set $R_i$ is announced for each agent.
    Each agent submits a single candidate in the eligible set and the candidate that maximizes a pre-commited score function $f:\Omega \mapsto \R$ is selected as the winner.
\end{definition}
We further define a notion of incentive compatibility.
\begin{definition}[Bayesian-Nash incentive compatibility]
	We say that a S-SPM mechanism $M$ is Bayesian-Nash incentive compatible (BNIC) with respect to the score function $f(\cdot)$ if submitting a solution that maximizes $f(\om)$ constructs a Bayesian-Nash equilibrium of the delegation game.
	We simply say that the mechanism is BNIC if it is BNIC w.r.t. score function $f(\om) = x(\om)$.
\end{definition}
If we can find a BNIC mechanism, then it is the best scenario for the principal, as it can naturally achieve the optimal delegation gap as the agents' strategic decisions are fully aligned with the principal's utility.
This indeed can be achieved under a very specific regime of independent and symmetric settings, described as follows.
\begin{proposition}
	Under the independent and symmetric setting, if $y(\cdot)$ is a linear transformation of $x(\cdot)$, then S-SPM mechanism $M$ with score function $f(\om) = x(\om)$ is BNIC.
\end{proposition}

The above example considers a specific scenario in which the principal's and the agents' utilities are fully aligned.


To guarantee a certain ratio of approximation while guaranteeing the incentive compatibility of the S-SPM, the principal has to sacrifice a bit of utility in designing the score function.
At one extreme, the principal can design a BNIC mechanism by sacrificing all the efficiency of the mechanism.
\begin{proposition}
	Under the independent and symmetric setting, consider a S-SPM mechanism $M$ with score function $f(\om) = y(\om)$.
	Then, $M$ is BNIC.
	However, it's delegation gap can be arbitrarily bad.
\end{proposition}
\suho{More work can be done in this direction. Key point is to design a good score function and eligible sets, in order to incentivize the agents to behave in favor of the principal.
For example, consider a score function $f(\om)= y(\om)x(\om)$ and eligible set $R_i = \{\om : x(\om) \ge y(\om)\}$. Although this will not induce a BNIC mechanism, this somehow efficiently balance the principal's utility and agent's utility so that maximizing score function is good for both the agents and the principal.}





\subsection{Learning setting}
Consider a more practical scenario in which each agent $i$ also does not know the exact values of the own samples $\bar{\omega}_i$, and neither does the principal. (and also does not know the distribution sampled from)
\footnote{Another interpretation: at each round, agent $i$ draws a unknown sample from one of unknown $D_i^{(1)},\ldots, D_i^{(l_i)}$}
Each agent correspondingly registers a set of samples at each round and the mechanism specifies which ones to select as the final outcome at the round.
Only the final outcome's reward is revealed at the end of the round.
\footnote{Another variant would be when each agent has a finite budget and decide whether to sample more solutions with costly effort of $c_i$, or commit with current samples $W_i$.}

Since the value of the solutions are not given in hindsight, threshold based mechanisms like single-proposal mechanism does not apply in this case.
Instead, the principal should design a good sequential decision rule, i.e. the bandit algorithm, to incentivize the agents in preferrable manner.

\begin{question}
What happens in single agent setting?
If agent learns well, he will eventually submit a single solution that maximizes own payoff.
Then, if the principal also learns well, he may apply single proposal mechanism to reject agent's solution after some rounds.

\end{question}

\begin{question}
What happens in single agent setting?
\end{question}



One interesting feature in this repeated setting is that the agents might abuse the exploration of the principal's algorithm as in \cite{shin2022multi}.
For example, if the agent becomes certain that his samples are suboptimal to the principal, he may...



\begin{question}
One interesting question in this setting will be even when all the payoffs are aligned, e.g. all $y_i$ are affine transformation of $x$, the agents might 
\end{question}

\subsection{Multiple selection}
When the principal selects multiple outcomes as final solutions?
For example in 





% \subsection{Further questions that we might work on}
% \begin{definition}[Randomized $k$-proposal mechanism]
% In randomized $k$-proposal mechanism, an eligible set $R \subset \Omega$ is announced by the principal, each agent proposes up to $k$ outcomes, and the principal finally uniform randomly chooses an outcome among the proposed candidates.
% \end{definition}

% \begin{conjecture}
% \suho{not proved, but intuitive}
% Randomized $k$-proposal mechanism admits dominant strategy equilibrium.	
% \end{conjecture}


% \begin{conjecture}
% \suho{not proved, but intuitive}
% Any mechanism $M$ with budget $1$ can be reduced to randomized $k$-proposal mechanism.	
% \end{conjecture}


% \begin{conjecture}
% \suho{not proved, but pretty intuitive}
% Randomized $k$-proposal mechanism achieves $(opt,1)$, i.e. it has optimal delegation gap under any mechanism with budget $1$.
% \end{conjecture}




% \begin{conjecture}
% \suho{not proved}
% There exists a online $f(c)$-proposal mechanism which achieves $(opt_c, c)$-approximation for any $c \in \{1,2,\ldots, \sum_{i=1}^n n_i\}$.
% \end{conjecture}



